Singular Value Perturbation and Deep Network Optimization

We develop new theoretical results on matrix perturbation to shed light on the impact of architecture on the performance of a deep network. In particular, we explain analytically what deep learning practitioners have long observed empirically: the parameters of some deep architectures (e.g., residual networks, ResNets, and Dense networks, DenseNets) are easier to optimize than others (e.g., convolutional networks, ConvNets). Building on our earlier work connecting deep networks with continuous piecewise-affine splines, we develop an exact local linear representation of a deep network layer for a family of modern deep networks that includes ConvNets at one end of a spectrum and ResNets, DenseNets, and other networks with skip connections at the other. For regression and classification tasks that optimize the squared-error loss, we show that the optimization loss surface of a modern deep network is piecewise quadratic in the parameters, with local shape governed by the singular values of a matrix that is a function of the local linear representation. We develop new perturbation results for how the singular values of matrices of this sort behave as we add a fraction of the identity and multiply by certain diagonal matrices. A direct application of our perturbation results explains analytically why a network with skip connections (such as a ResNet or DenseNet) is easier to optimize than a ConvNet: thanks to its more stable singular values and smaller condition number, the local loss surface of such a network is less erratic, less eccentric, and features local minima that are more accommodating to gradient-based optimization. Our results also shed new light on the impact of different nonlinear activation functions on a deep network's singular values, regardless of its architecture.

==> content/backups/abstract.tex <==
We develop new theoretical results on matrix perturbation to shed light on the impact of architecture on the performance of a deep network.
%
In particular, we explain analytically what deep learning practitioners have long observed empirically: the parameters of some deep architectures (e.g., residual networks, ResNets, and Dense networks, DenseNets) are easier to optimize than others (e.g., convolutional networks, ConvNets). 
%
Building on our earlier work connecting deep networks with continuous piecewise-affine splines, we develop an exact local linear representation of a deep network layer for a family of modern deep networks that includes ConvNets at one end of a spectrum and ResNets and DenseNets at the other.
%
For regression tasks that optimize the squared-error loss, we show that the optimization loss surface of a modern deep network is piecewise quadratic in the parameters, with local shape governed by the singular values of a matrix that is a function of the local linear representation.
%
We develop novel perturbation results for how the singular values of matrices of this sort behave as we add a fraction of the identity
and multiply by certain diagonal matrices.
\rolf{added "diag"}
%
A direct application of our perturbation results explains analytically why a ResNet is  easier to optimize than a ConvNet: thanks to its more stable singular values and smaller condition number, the local loss surface of a ResNet is less erratic, less eccentric and with wider local minima.
\richb{need to say the right rigorous stuff about the surface}
\rolf{I would say that ``stable'' is an appropriate term in the sense that they do not change as much from region to region (i used the term "erratic" above.) Also I added the term "volatile" in the first part of section 6.3. Not sure which way is more clear ("erratic" or "volative)
...
not sure you want or need to clarify this ... 

other ways to say the same: the pieces of the piecewise ellipsoidic surface vary less for the ResNet when moving from region to region as compared to COnvNets}






\begin{comment}

We develop new theoretical results on matrix perturbation to shed light on the impact of architecture on the performance of a deep network.
%
In particular, we explain analytically what deep learning practitioners have long observed empirically: some deep architectures (e.g., residual networks, ResNets) are easier to optimize than others (e.g., convolutional networks, ConvNets). 
%

Building on our earlier work connecting deep networks with continuous piecewise-affine splines, we develop a local linear representation of a layer for a family of modern deep network parameterized by $\PertVar$, with $\PertVar=0$ corresponding to a ConvNet and $\PertVar=1$ to a ResNet.

%
For regression tasks that optimize the squared-error loss, we show that the optimization loss surface of a deep network is piecewise quadratic, with local shape governed by the singular values of the matrix $Q$ defining the local quadratic term of the loss.

\richb{all this math is just too much for an abstract; i am going to take it out once i think of a clean way}

%
Our approach is to consider $M(\PertVar)D$ with
as the  matrix $W_1$ perturbed by multiplications with diagonal matrices $D_1$ and $D$ representing locally the non-linearities and perturbed by adding a fraction $\PertVar$ of the identity ${\rm Id}$, representing the residual link.
%
We develop novel perturbation results for such scenarios.
%
%Gradient-based optimization depends crucially on the landscape of the loss surface.
%
In both deterministic and random settings, we prove a result that could be of independent interest:  when adding ${\rm Id}$ to any matrix $M$, the square of any of its singular values grows by at most $1+\overline{\tau}$ in general and by at least $1+\underline{\tau}$ under mild conditions.
%
Here, $\overline{\tau}$ and $\underline{\tau}$ denote the largest and smallest eigenvalues of $M+M^T$, respectively.
%
A direct application of our perturbation results explains analytically why a ResNet is  easier to optimize than a ConvNet: thanks to its more stable singular values, the local loss surface of a ResNet is smoother, with wider local minima.



\rolf{I adapted the notation of the following}

We study the singular values of matrices of the form 
$(M_o+\PertVar{\rm Id})D$.
We are interested in understanding the change of the 
singular values under the 
perturbation by adding a fraction $\PertVar$ of the identity ${\rm Id}$ to $M_o$ as well as the multiplicaton with $D$.
%
This scenario is motivated by the need to better understand the impact of architecture on the performance of a deep network.
%
Here, $W_1$ contains the weights of the network layer of interest; $D_1$ and $D$ capture the nonlinearity of network's activation functions; thus,
$M_o=D_1 W_1$ represents locally the action of a layer
of the network. The parameter $\PertVar$ defines a spectrum between two common architectures, with $\PertVar=0$ corresponding to a convolutional network (ConvNet) and $\PertVar=1$ corresponding to a residual network (ResNet).
%
Our perturbation results enable us to explain what deep learning practitioners have long observed empirically: some deep architectures (e.g., ResNets) are easier to optimize than others (e.g., ConvNets). 
%
Gradient-based optimization depends crucially on the landscape of the loss surface.
%
Building on our earlier work in continuous piecewise-affine deep networks, we show that, for regression tasks that optimize the squared error, the optimization loss surface is piecewise-quadratic, with local shape governed by the singular values of the matrix $A$.
%
\richb{need to connect all the discussion about $A$ above with $M$ below}
%
In both deterministic and random settings, we prove a result that could be of independent interest:  when adding ${\rm Id}$ to any matrix $M_o$, the square of any of its singular values grows by at most $1+\overline{\tau}$ in general and by at least $1+\underline{\tau}$ under mild conditions.
%
Here, $\overline{\tau}$ and $\underline{\tau}$ denote the largest and smallest eigenvalues of $M+M^T$, respectively.
%
A direct application of our perturbation results analytically explain why a ResNet is  easier to optimize than a ConvNet: thanks to its larger singular values and its smaller condition number, the local loss surface of a ResNet is less eccentric with wider local minima.







---------
We develop new theoretical results on matrix perturbation to shed light on the impact of architecture on the performance of a deep network.
%
In particular, we explain analytically what deep learning practitioners have long observed empirically: some deep architectures (e.g., residual networks, ResNets) are easier to optimize than others (e.g., convolutional networks, ConvNets). 
%
Building on our earlier work connecting deep networks with continuous piecewise-affine splines, we show that a layer of a modern deep network can be written locally as $M(\PertVar)=D_1 W_1+\PertVar{\rm Id}$.
%
Here, $W_1$ contains the weights of the layer, while $D_1$ captures locally the nonlinearity of the network's activation function. 
%
Through the parameter $\PertVar$, we obtain a spectrum linking two common architectures, with $\PertVar=0$ corresponding to a ConvNet and $\PertVar=1$ to a ResNet.
%
For regression tasks that optimize the squared-error loss, we show that the optimization loss surface of a deep network is piecewise quadratic, with local shape governed by the singular values of the matrix $Q$ defining the local quadratic term of the loss:
$w^T Q w=\|M(\PertVar)D W z \|_2^2$, where  $W$, $D$ represent the trained layer, $z$ its input and $w$ is the flattened version of $W$.
\richb{ok i'm still lost -- you use $D_1, W_1$ just above and now $D,W$. i'm concerned this is too complicated to explain}
%
Our approach is to consider $M(\PertVar)D$ as the  matrix $W_1$ perturbed by multiplications with diagonal matrices $D_1$ and $D$ representing locally the non-linearities and perturbed by adding a fraction $\PertVar$ of the identity ${\rm Id}$, representing the residual link.
%
We develop novel perturbation results for such scenarios.
%
%Gradient-based optimization depends crucially on the landscape of the loss surface.
%
In both deterministic and random settings, we prove a result that could be of independent interest:  when adding ${\rm Id}$ to any matrix $M$, the square of any of its singular values grows by at most $1+\overline{\tau}$ in general and by at least $1+\underline{\tau}$ under mild conditions.
%
Here, $\overline{\tau}$ and $\underline{\tau}$ denote the largest and smallest eigenvalues of $M+M^T$, respectively.
%
A direct application of our perturbation results explains analytically why a ResNet is  easier to optimize than a ConvNet: thanks to its more stable singular values, the local loss surface of a ResNet is smoother, with wider local minima.




We study the singular values of matrices of the form $A=(D_1 W+\PertVar{\rm Id})D$ as they are perturbed by adding a fraction $\PertVar$ of the identity ${\rm Id}$.
%
This scenario is motivated by the need to better understand the impact of architecture on the performance of a deep network.
%
Here, $W$ contains the weights of the network layer of interest; $D_1$ and $D$ capture the nonlinearity of network's activation functions; and $\PertVar$ defines a spectrum between two common architectures, with $\PertVar=0$ corresponding to a convolutional network (ConvNet) and $\PertVar=1$ corresponding to a residual network (ResNet).
%
Our perturbation results enable us to explain what deep learning practitioners have long observed empirically: some deep architectures (e.g., ResNets) are easier to optimize than others (e.g., ConvNets). 
%
Gradient-based optimization depends crucially on the landscape of the loss surface.
%
Building on our earlier work in continuous piecewise-affine deep networks, we show that, for regression tasks that optimize the squared error, the optimization loss surface is piecewise-quadratic, with local shape governed by the singular values of the matrix $A$.
%
\richb{need to connect all the discussion about $A$ above with $M$ below}
%
In both deterministic and random settings, we prove a result that could be of independent interest:  when adding ${\rm Id}$ to any matrix $M$, the square of any of its singular values grows by at most $1+\overline{\tau}$ in general and by at least $1+\underline{\tau}$ under mild conditions.
%
Here, $\overline{\tau}$ and $\underline{\tau}$ denote the largest and smallest eigenvalues of $M+M^T$, respectively.
%
A direct application of our perturbation results analytically explain why a ResNet is  easier to optimize than a ConvNet: thanks to its more stable singular values, the local loss surface of a ResNet is smoother, with wider local minima.



%We study the perturbation of the singular values of a square matrix $W$ when adding a fraction of the Identity ${\rm Id}$ and multiplying  by certain diagonal matrices $D_1$, $D$ as in $A=(D_1W+\PertVar{\rm Id})D$.
%

To be more precise: 
Gradient based optimization depends crucially on the shape of the loss surface.
Building on earlier work \cite{reportRB,balestriero2018spline} we find that 
this shape is continuous, piecewise-quadratic, and is essentially governed by the singular values of the matrix $A$ where
$D_1$ and $D$  capture different types of nonlinear activations used in the DN,
$W$ represents the weights of a layer and where $\PertVar=0$ corresponds to a
Fully Convolutional architecture (CNN) and $\PertVar=1$ to a Residual architecture (ResNet).

When adding Identity to any matrix $M$, we show that the square of any singular value grows at most by $1+\overline{\tau}$; also, they grow at least by $1+\underline{\tau}$ under mild conditions. Here, $\overline{\tau}$  and $\underline{\tau}$ denote the largest and smallest eigenvalue of $M+M^T$. We also show how multiplication with diagonal matrices perturbs the singular values of a matrix. Thereby, we assume bounds on the size of the entries of $W$ and work in both, deterministic and random settings.
Through these perturbation results we are able to explain from an optimization perspective what practitioners have long observed: some DN architectures are simpler to optimize than others. 
\end{comment}

%
% \PrintAll{
%   This is of relevance for  DNs when using the absolute
%   value as activation since this does not alter singular values.
%For $n\times n$ matrices with entries bounded by $1/n$ the lower bound is always positive, yielding bounds on the conditioning of $W+{\rm Id}$. 
%For $n\times n$ matrices $W$ with i.i.d.~entries of
% zero mean and variance proportional to $1/n$
%   the lower bound is positive with high probability.
%   We provide empirical evidence for the fact that the bounds on the growth
%   are surprisingly tight, suggesting that singular
%   values of random matrices $W+{\rm Id}$
%   tend to spread as much as possible, thus,
%   extending a fact due to Wigner for symmetrical zero-mean matrices.
%   In the same setting, our simulations indicate that asymptotically
%   $\overline{\tau}/\|W\|_{\rm Op}$  converges in distribution to
%   $\sqrt{2}$. This suggests that $\|W\|_{\rm Op}$ follows a Tracy-Widom law
%   when properly renormalized, a fact established so far for symmetrical
%   random matrices only --- to the best of our knowledge.
%   This implies that the upper bound of growth we establish is significantly
%   smaller than the trivial $\|W+{\rm Id}\|_{\rm Op}\leq 1 + \|W\|_{\rm Op}$.
%}

==> content/backups/body.tex <==
%\section{Existing and Related Work}
\section{Background}
\label{sec:101}

\subsection{Notation}
\label{subsec:notation}

\if 0
{\bf Any matrix $M$.}
\rolf{approve or disapprove the following}

Throughout the paper, the matrix $M$ is of the form 
(see \equ{M_intro}).
$$
    M=M(\PertVar)
    =
    D_pW_p \cdots D_1W_1+\PertVar{\rm Id}
$$
We often use the shorthand $M_o=M(0)$ and $M=M_o+\PertVar{\rm Id}$.

The term ``any matrix $M$'' means to say that no restrictions are imposed on $D_i$ and $W_i$.
Consequently, $M$ can then indeed be any matrix.
This can be seen by
setting $D_p=...=D_1=W_p=...=W_2=$Id; this leads to 
$M=W_1+\PertVar$Id which may equal any arbitrary given matrix.

In conclusion, the term ``any matrix $M$'' is not ambiguous despite the particular form \equ{M_intro}.

Whenever restrictions on $D_i$ or $W_i$ are enforced, this will be noted explicitly.
\fi{}

{\bf Singular values.}
    Let $\AnyM$ be a $n\times n$-matrix, and let $\|u\|$ denote the $\ell_2$-norm of the vector $u$.
    All products are to be understood as matrix multiplications,
    even if the factors are vectors. Vectors are always column vectors.

    Let $u_i$ denote a unit-eigenvector of $\AnyM^T\AnyM$
    to its  \emph{eigenvalue }
    $\eigval_i=\eigval_i(\AnyM^T\AnyM)$ such that
    the vectors $u_i$ ($i=1\ldots n$) form an orthonormal basis.


    The \emph{singular values} of $\AnyM$ are defined as the square roots of the eigenvalues of ${\AnyM}^T{\AnyM}$
    $$
        \singval_i
        =
        \singval_i(\AnyM)
        =
        \sqrt{\eigval_i({\AnyM}^T{\AnyM})}
        =
        \|{\AnyM}u_i\|.
    $$
    Note that the singular values are always real non-negative valued since
    $$
    0\leq \|{\AnyM}u_i\|^2=u_i^T{\AnyM}^T{\AnyM}u_i=\eigval_i u_i^Tu_i=\eigval_i .
    $$
    %
    For reasons of definiteness, we take the eigenvalues of ${\AnyM}^T{\AnyM}$, and thus the singular values of ${\AnyM}$ to be ordered by size: $\singval_1\geq\ldots\geq\singval_n$.

{\bf Singular vectors.}
The vectors $u_i$ are called \emph{right singular vectors} of ${\AnyM}$.
The \emph{left singular vectors} of ${\AnyM}$ are denoted $v_i$ and are defined as an orthonormal basis with the property that
    \begin{equation}
    \label{EQU:singular_values}
        {\AnyM}u_i=\singval_i v_i
        \qquad\mbox{and}\qquad
        {\AnyM}^Tv_i=\singval_i u_i.
    \end{equation}
    Such a basis of left-singular vectors always exists.
    \iffalse
    \PrintAll{Indeed, assume for a moment that all $\singval_i \neq 0$ and set $v_i=\frac{1}{\singval_i} Mu_i$.
    Note that these vectors obviously satisfy the equations (\ref{EQU:singular_values}),
    first by definition of $v_i$, and second since
    ${\AnyM}^Tv_i=(1/\singval_i){\AnyM}^T{\AnyM}u_i=\singval_iu_i$.
    Also, $\|v_i\|=1$ by definition of $\singval_i$
    and for $i\neq j$ we have $v_i^Tv_j=u_i^T{\AnyM}^T{\AnyM}u_j/(\singval_i\singval_j)
    =\singval_j^2u_i^Tu_j/(\singval_i\singval_j)=0$.

    Now, should there be some $\singval_k=0$ simply choose the corresponding $v_k=u_k$;
    in other words, they form an orthonormal basis of the kernel of ${\AnyM}$.
    Then, the first equation of (\ref{EQU:singular_values}) holds also for these $v_k$
    since $\singval_k=0$.
    Thus, the first part of (\ref{EQU:singular_values}) holds for all $i=1\ldots n$.
    In order to show that ${\AnyM}^Tv_k=0$ note that
    its projection onto all basis vectors $u_i$ is zero:
    $({\AnyM}^Tv_k)^Tu_i=v_k^T{\AnyM}u_i=\singval_i v_k^Tv_i=0$, for $i\neq k$ by orthogonality
    and for $i=k$ since $\singval_k=0$.

    Vice versa, whenever two normed vectors $u_i$ and $v_i$ and a non-negative $\singval_i$
    satisfy (\ref{EQU:singular_values}) they are the left and right singular vectors
    of ${\AnyM}$ and $\singval_i$ is the corresponding singular value.
    To verify this fact, simply note that $u_i$ is indeed the correct eigenvector of ${\AnyM}^T{\AnyM}$:
    ${\AnyM}^T{\AnyM}u_i={\AnyM}^T{\AnyM}u_i=\singval_i{\AnyM}^Tv_i=\singval_i^2u_i$.
    }
\fi


{\bf SVD.} Collecting the right singular vectors $u_i$ as columns into an orthogonal matrix $U$, the left singular vectors $v_i$ into an orthogonal matrix $V$ and the singular values $\singval_i$ into a diagonal matrix $\Sigma$ in corresponding order, we get the Singular Value Decomposition of ${\AnyM}=V\Sigma U^T$. 
\if 0
    The basis vectors $u_i$ are first moved into alignment with the coordinate axes, stretched by the singular values, and finally moved to $v_i$. Consequently, the matrix ${\AnyM}$ can be viewed as mapping the unit sphere to an ellipsoid with semi-axes in directions of the $v_i$ and with lengths $\singval_i$. 
\fi

{\bf Eigenvectors.}
Note that ${\AnyM}$ may have eigenvectors that may  differ from the singular vectors. In particular, eigenvectors are not always orthogonal onto each other. Clearly, if ${\AnyM}$ is symmetric then eigenvectors and right-singular vectors coincide and every \emph{eigenvalue $r_i$ of ${\AnyM}$} corresponds to a
    singular value $\singval_i=|r_i|$.
%
However, to avoid confusion we will refrain from referring to the \emph{eigenvalues} of ${\AnyM}$
    whenever possible.


{\bf Smooth matrix deformations.}
Let us consider a family of $n \times n$  matrices 
${\AnyM}(\PertVar)$ where the variable $\PertVar$ in assumed 
to lie in some interval $I$.
We say that the family ${\AnyM}(\PertVar)$ is $\mathcal{C}^{m}(I)$
if all its entries are, with $m=0$ corresponding to being continuous
and $m=1$ to continuously differentiable.
If ${\AnyM}$ is $\mathcal{C}^{m}(I)$, so is ${\AnyM}^T{\AnyM}$.

We denote the matrix of derivatives of the entries of ${\AnyM}$ by ${\AnyM}'(\PertVar)=\frac{d}{d\PertVar} {\AnyM}(\PertVar)$.
%Note that the associated eigenvectors and eigenvalues also depend on $\PertVar$.


{\bf Multiplicity of singular values}
Denote by
$S_i\subset I$ the set of $\PertVar$ values
%in the domain $I$ of ${\AnyM}(\PertVar)$
for which $\singval_i$ is a \emph{simple} singular value:
\begin{equation}\label{EQU:def_simple}
  S_i
  =
  \{\PertVar\in I
  \,:\,
  \singval_i(\PertVar)\neq\singval_j(\PertVar)
  \mbox{ for all $j\neq i$}\}.
\end{equation}
%and let $S_i^*\subset S_i$ be the set where
%$\singval_i(\PertVar)\neq0$.
\MoreDetails{The singular vectors $u_i$ are uniquely
defined on $S_i$ up to multiplication
by $-1$; the $v_i$ follow from the
$u_i$ according to (\ref{EQU:singular_values}).
When two or more singular values coincide
then the corresponding eigenspace of ${\AnyM}^T{\AnyM}$ is at least $2$-dimensional and
there is a freedom of choice of 
eigenvectors $u_i$ as the basis of that eigenspace.}
For later use let
\begin{equation}\label{EQU:def_nonzero}
  S_i^*
  =
  \{\PertVar\in S_i
  \,:\,
  \singval_i(\PertVar)\neq0\}.
\end{equation}

%\if 0
For completeness
we mention an obvious fact that follows from the SVD:
    \begin{equation}\label{EQU:transpose}
      \singval_i({\AnyM})
      =
      \singval_i({\AnyM}^T).
    \end{equation}
%\fi
%
\subsection{Singular values under additive perturbation}

A classical result that will prove to be key in our study is due to Wielandt and Hoffman \cite{Wielandt_Hoffman}.
It uses the notion 
of the Frobenius norm 
$\|{\AnyM}\|_2$
of the $n\times n$-matrix ${\AnyM}$.
Denoting the entries of ${\AnyM}$ by ${\AnyM}[ij]$
and its singular values by $\singval_i({\AnyM})$,
it is well known that
\begin{equation}\label{EQU:frobenius_norm}
  \|{\AnyM}\|_2^2
  =
  \sum_{i,j=1}^{n} |{\AnyM}[ij]|^2
  =
  \mbox{\rm trace}({\AnyM}^T{\AnyM})
  =
  \sum_{i=1}^{n}\singval_i^2({\AnyM})
  .
\end{equation}
%
\begin{prop}[Wielandt and Hoffman]
  \label{prop:Frobenius_bound}
    Let ${\AnyM}$ and ${\AnyMt}$ be symmetrical $n\times n$-matrices
    with eigenvalues ordered by size.
    Then
    \begin{equation}
    \label{EQU:frobenius_bound}
        \sum_{i=1}^{n}
        \Big|\eigval_i({\AnyM})-\eigval_i({\AnyMt})\Big|^2
    % result not to be trusted, by appears so Chafaï:
    %    \Big|\singval_i({\AnyM})-\singval_i(B)\Big|^2
        \leq
        \|{\AnyM}-{\AnyMt}\|_2^2
    \end{equation}
\end{prop}
%
It can easily be strengthened to read as follows.
\begin{cor}[Wielandt and Hoffman]
  \label{cor:Frobenius_bound}
    Let ${\AnyM}$ and ${\AnyMt}$ be any $n\times n$-matrices
    with singular values ordered by size.
    Then
    \begin{equation}
    \label{EQU:strong_frobenius_bound}
        \sum_{i=1}^{n}
        \Big|\singval_i({\AnyM})-\singval_i({\AnyMt})\Big|^2
        \leq
        \|{\AnyM}-{\AnyMt}\|_2^2
    \end{equation}
\end{cor}
Note that this result, as most others, holds actually also for rectangular matrices
with the usual adjustments.

\begin{proof}
  We establish Corollary~\ref{cor:Frobenius_bound}.
  The $2n$ eigenvalues of the symmetrical matrix
%  \begin{equation}\label{EQU:proof_cor_Frob}
$$
    H_{\AnyM}
    =
    \left[
        \begin{array}{cc}
          0 & {\AnyM}  \\
          {\AnyM}^T & 0
        \end{array}
    \right]
$$
%\end{equation}
  are $\singval_i({\AnyM})$ with eigenvector
%  $\frac{1}{\sqrt 2}(v_i^T u_i^T)^T$
  $\frac{1}{\sqrt 2}{ v_i \choose u_i }$
  and $-\singval_i({\AnyM})$ with eigenvector
%  $\frac{1}{\sqrt 2}(-v_i^T u_i^T)^T$.
  $\frac{1}{\sqrt 2}{ -v_i \choose u_i }$.
  Also, $\|H_\AnyM\|_2^2=2\|{\AnyM}\|_2^2$. 
  Therefore, when applying Proposition~\ref{prop:Frobenius_bound} 
  with $\AnyM$ replaced by 
  $H_\AnyM$ and $\AnyMt$ replaced by $H_\AnyMt$
  we run through the left hand side of (\ref{EQU:strong_frobenius_bound}) twice
  and in turn obtain twice the right hand side.
  \hfill$\Box$
\end{proof}

Corollary~\ref{cor:Frobenius_bound}.
  immediately implies 
  a well known result that will be key:
   the singular values of a matrix depend continuously on its entries, as we state next. 
   \if 0
   This is in essence a consequence of the fact that the complex zeros of a polynomial depend continuously on the coefficients. 
   \fi
   
\begin{lem}
    \label{lem:continuity}
    If ${\AnyM}(\PertVar)$ is $\mathcal{C}^{0}(I)$, then
    all its singular values $\singval_i(\PertVar)$ depend continuously on $\PertVar$.
    Consequently, all $S_i$ \equ{def_simple} and
    $S_i^*$ \equ{def_nonzero} are then open.
\end{lem}

\begin{proof}

To establish continuity,
choose $\PertVar_1$ and
$\PertVar_2$ arbitrary and
apply Corollary~\ref{cor:Frobenius_bound} (in slight abuse of notation) with
${\AnyM}={\AnyM}(\PertVar_1)$ and
${\AnyMt}={\AnyM}(\PertVar_2)$.
\hfill$\Box$
\end{proof}

As will become clear in the sequel,
the main difficulty in establishing
further results on regularities of the singular values
with elementary
arguments and estimates lies
in dealing with multiple zeros, i.e., with
multiple singular values.



Also useful are some facts about the special role of the largest singular value.
\begin{prop}[Operator norm]
  \label{prop:operator_norm}
    Let ${\AnyM}$ be a  $n\times n$-matrix. Then, its largest singular value
    is equal to its operator norm, and we have the following additional inequalities:
    \begin{equation}
    \label{EQU:operator_norm}
        \singval_1({\AnyM})
        =
        \|{\AnyM}\|_{\rm Op}
        :=
        \max_{|x|=1}|\AnyM x|
        \leq
        \|{\AnyM}\|_2
        \leq
        \sqrt{{\rm rank}({\AnyM})}\cdot
        \|{\AnyM}\|_{\rm Op}
        %\singval_1({\AnyM})
    \end{equation}
    In particular, if ${\AnyM}$ is rank 1, then both norms coincide.
    Also, being a norm, the largest singular value
    satisfies for any matrices ${\AnyM}$ and ${\AnyMt}$
    \begin{equation}
    \label{EQU:norm_inequality}
    \singval_1({\AnyM}+{\AnyMt})\leq \singval_1({\AnyM})+\singval_1({\AnyMt})
    .
    \end{equation}
\end{prop}
\begin{proof}
  The first equality follows from the fact that $\singval_1$ is the largest semi-axis of the ellipsoid that is the image of the unit-sphere.
  The first inequality follows from (\ref{EQU:frobenius_norm}).
  The last inequality follows again from considering the aforementioned ellipsoid.
\end{proof}
%
Another proof of the continuity of singular values
is found in the well known interlacing properties of singular values,
which we adapt to our notation and summarize for the convenience of the reader
(see, e.g. \cite[Theorem~6.1.3-5.]{Chafai}):
\begin{prop}[Interlacing]
  \label{prop:interlacing}
    Let ${\AnyM}$ and ${\AnyMt}$ be $n\times n$-matrices
    with singular values ordered by size.
    \begin{itemize}
      \item (Weyl additive perturbation) We have:
    \begin{equation}
    \label{EQU:weyl}
        \singval_{i+j-1}({\AnyM})
        \leq
        \singval_i({\AnyMt})+\singval_j({\AnyM}-{\AnyMt}).
    \end{equation}
\if 0
not needed
\item (Finite rank additive perturbation)
      If ${\rm rank}({\AnyM}-{\AnyMt})\leq k$, then
    \begin{equation}
    \label{EQU:finite_rank}
        \singval_{i-k}({\AnyM})
        \geq
        \singval_i({\AnyMt})
        \geq
        \singval_{i+k}({\AnyM})
    \end{equation}
\fi
\item (Cauchy interlacing by deletion)
      Let ${\AnyMt}$ be obtained from ${\AnyM}$ by deleting $m$ rows or $m$ columns.
      Then
    \begin{equation}
    \label{EQU:deletion}
        \singval_{i}({\AnyM})
        \geq
        \singval_i({\AnyMt})
        \geq
        \singval_{i+m}({\AnyM}).
    \end{equation}
    \end{itemize}
\end{prop}
From (\ref{EQU:weyl}), applied with $j=1$
we note that the singular values are in fact uniformly continuous.
Indeed, we have for any $i$ that
    \begin{equation}
    \label{EQU:uniform_bound}
        |\singval_{i}({\AnyM})
        -
        \singval_i({\AnyMt})
        |
        \leq
        \singval_1({\AnyM}-{\AnyMt})
        \leq
        \|{\AnyM}-{\AnyMt}\|_2
    \end{equation}


\iffalse
\PrintAll{
Locating the eigenvalues without solving the characteristic
polynomial is a hard problem. Apparently, the diagonal
elements play a special role in such an endeavor.
An interesting result, appearing in
the book by Horn and Johnson (see \cite[theorem 6.1.1.]{Horn_Johnson}),
gives a first clue
as to the relation between diagonal elements
and the eigenvalues of ${\AnyM}^T{\AnyM}$:
\begin{prop}[Gersgorin-discs]
  \label{prop:Gersgorin}
Let
$$
    r_i=\sum_{j\neq i} |n_{ij}|
$$
be the $\LayerIndex_1$ norm of the $i$-th row of ${\AnyM}^T{\AnyM}$ with all diagonal elements set to zero.
Then all eigenvalues of ${\AnyM}^T{\AnyM}$ lie in the union of the closed discs
with centers $n_{ii}$ and radii $r_i$:
$$
    \eigval_j({\AnyM}^T{\AnyM})
    \in\bigcup\limits_{i_1}^n
        \{x\in\reals\,:\,|n_{ii}-x|\leq r_i\}
    .
$$
\if 0
    Furthermore, if a union of $k$ such discs forms a connected set that is disjoint from all the remaining $n-k$ discs, then there are precisely $k$ eigenvalues of ${\AnyM}^T{\AnyM}$ in this union.

    Furthermore, if $p_1,...,p_n$ are positive real, then the above
    conclusions hold also when replacing all radii by
    $$
        r_i
        =
        (1/p_i)\sum_{j\neq i}^{} p_j|a|_{ij}|
    $$
    leading potentially to sharper estimates.
\fi
\end{prop}
}

If the matrix ${\AnyM}^T{\AnyM}$ has a dominant diagonal in the sense that the
Gersgorin-discs are mutually disjoint, then the above results pin-points
the location of the individual eigenvalues.
\fi


\subsection{Singular Values Under Smooth Perturbation}

Let us now turn to the study of how singular values of ${\AnyM}(\PertVar)$ change as a function of $\PertVar$, thereby leveraging the concept of differentiability.

This can be done 
in several ways; the following computation is particularly simple
and well known.
Let $N(\PertVar)$ 
denote a family of  symmetrical $\mathcal{C}^{1}(I)$ matrices.
Dropping all indices and variables $\PertVar$ for ease of reading, the eigenvalues and eigenvectors satisfy:
\begin{eqnarray*}
    Nu=\eigval u,
    \qquad
    u^Tu=1.
\end{eqnarray*}
By taking the derivatives w.r.t.\ $\PertVar$,
assuming they exist, we obtain
\begin{eqnarray*}
    N' u+N u'
    =
    \eigval'u+\eigval  u',
    \qquad
    u'^Tu=u^Tu'=0.
\end{eqnarray*}
We then left-multiply the first equality by $u^T$ and use the second equality
to find
\begin{eqnarray*}
    u^T N' u + u^TN u'
    =
    \eigval' u^T u + \eigval u^T u'
    =
    \eigval'.
\end{eqnarray*}
Finally, as $N$ is symmetric we see that  $u^T Nu'=(Nu)^Tu'=\eigval u^T u' = 0$ leading to
$$
\eigval'=u^T N' u
.
$$

In quantum mechanics, the last equation 
is known as the Hellmann-Feynman theorem and
was discovered independently by several authors in the 1930s.
%, as well as by the present author in 2019 and many others.
It is known, though seldom mentioned,
that the formula may fail when eigenvalues coincide. For further studies in this direction we refer the interested reader to works in the field of degenerate perturbation theory.

For a proof of the Hellmann-Feynman Theorem it is natural to 
consider the function $\Psi:\reals^{n+2}\to \reals^{n+1}$
    $$
        \Psi(\PertVar,u,\eigval)
        =
    \left(\begin{array}{c}
        Nu-\eigval u \\
        u^Tu-1
        \end{array}
    \right)
    $$
where $u$ is an $n$-dimensional column vector.
    %with coordinates $u[j]$.
The  Implicit Function Theorem, applied to $\Psi$ then yields the following result.

\begin{thm} [Hellmann-Feynman]
\label{thm:lambda_differentiability}
Assume $N(\PertVar)$ forms a family of symmetrical $\mathcal{C}^{1}(I)$ matrices.
Then, as a function of $\PertVar$
each of its eigenvalues $\eigval_i=\eigval_i(\PertVar)$ is continuously differentiable  where  it is simple. 
%More precisely, $\eigval_i$ is
%$\mathcal{C}^{1}(S_i)$
Its derivative reads as
\begin{equation}
    \label{EQU:derivative_lambda}
        \eigval_i'(\PertVar)
        =
        u_i^T N' u_i
%        =
%        u_i^T({\AnyM}'^T {\AnyM} + {\AnyM}^T {\AnyM}')u_i
%        =
%        2u_i^T{{\AnyM}'}^T {\AnyM} u_i
%        =
%        2\singval_i u_i^T{{\AnyM}'}^T v_i
        .
\end{equation}
Its corresponding right singular vector
$u_i(\PertVar)$ can be chosen such that
it becomes
$\mathcal{C}^{1}(S_i)$
as well.
\end{thm}
%
If in addition to the assumptions of Theorem~\ref{thm:lambda_differentiability}
the family $N$ is actually $\mathcal{C}^{m}(I)$
then $\eigval_i(\PertVar)$ and $u_i(\PertVar)$
are $\mathcal{C}^{m}(S_i)$. 
From Hellmann-Feynmann we may conclude the following:

\begin{cor}
\label{cor:sigma_differentiability}
Let ${\AnyM}(\PertVar)$ be $\mathcal{C}^{1}(I)$.
Assume that $S_i^*$
consists of isolated points only. Then, $\singval_i(\AnyM)$
and its  left singular vector $v_i$
are $\mathcal{C}^{1}(S_i^*)$
with
$$
    \singval'_i(\PertVar)
        =
        u_i(\PertVar)^T{{\AnyM}'(\PertVar)}^T v_i(\PertVar)
    %=\eigval_i'/(2\singval_i)=
    %=u_i^T\AnyM'^Tv_i.
$$
\end{cor}
%
Simple examples show that the above results cannot be improved
without stronger assumptions
(see Example 1 below and Figure~\ref{fig:ex_101}).

\begin{proof}
Apply theorem~\ref{thm:lambda_differentiability}
to the family $N={\AnyM}^T {\AnyM}$. 
Note that
$N'={\AnyM}'^T {\AnyM} + {\AnyM}^T {\AnyM}'$
and apply the chain rule to
$\eigval_i=(\singval_i(\PertVar))^2$
to find the first equality of the following formula:
$$
    \singval'_i
        =
        \frac{1}{2\singval_i}
        u_i^T({\AnyM}'^T {\AnyM} + {\AnyM}^T {\AnyM}')u_i
        =
        \frac{1}{2\singval_i}
        2u_i^T{{\AnyM}'}^T {\AnyM} u_i
        =
        u_i^T{{\AnyM}'}^T v_i
    %=\eigval_i'/(2\singval_i)=
    %=u_i^T\AnyM'^Tv_i.
$$
Also, we have 
$u_i^T{\AnyM}'^T {\AnyM}u_i=(u_i^T{\AnyM}'^T {\AnyM}u_i)^T
=u_i^T{\AnyM}^T {\AnyM}'u_i$ since this is a real-valued number. This implies
the second equality in the formula above. 
Finally note that 
${\AnyM} u_i=\singval_i v_i$ to complete the proof.
\hfill$\Box$
\end{proof}


\if 0
        We have the
        following auxiliary result.
        \begin{lem}
            \label{lem:Jacobi_derivaitve}
            If the family of normal $n \times n$-matrices $N(\PertVar)$
            depends differentiably on $\PertVar$, then
            \begin{equation}
                \label{EQU:Jacobi}
                \frac{d}{d\PertVar} \det (N(\PertVar))
                =
                \sum_{i=1}^n
        %            r_i(\PertVar) u_i(\PertVar) N'(\PertVar) u_i(\PertVar)
                    r_i u_i N' u_i
            \end{equation}{}
            Here,
            $u_i(\PertVar)$ denote the eigenvectors
            with eigenvalues  $\eigval_k(\PertVar)$ of $N(\PertVar)$,
            and  $r_i(\PertVar)=\prod_{k\neq i}\eigval_k(\PertVar)$ .
            For ease of notation, we dropped the variable $\PertVar$
            on the right side on~\ref{EQU:Jacobi} in all quantities.
        \end{lem}

        \begin{proof}
            TODO
        \end{proof}
        \rolf{END of go to the appendix}
\fi

\iffalse
\PrintAll{
\begin{proof}
(i)
    As a first steps towards establishing differentiability of eigenvalues and eigenvectors
    consider the function $\Psi:\reals^{n+2}\to \reals^{n+1}$
    $$
        \Psi(\PertVar,u,\eigval)
        =
    \left(\begin{array}{c}
        Nu-\eigval u \\
        u^Tu-1
        \end{array}
    \right)
    $$
    where $u$ is an $n$-dimensional column vector
    with coordinates $u[j]$.
    Also, let us compute $J$, the matrix of partial derivatives of all $n+1$ coordinates of $\Psi$
    with respect to the $n+1$ variables $u[1],\ldots u[n],\eigval$.
    One finds
    the $(n+1)\times(n+1)$-matrix
    $$
        J(u,\eigval)
        =
    \left(\begin{array}{cc}
        N-\eigval\mbox{\rm Id} & -u \\
        u^T     & 0 \\
        \end{array}
    \right)
    $$

(ii)
    Now fix $i$ and let $\PertVar^*\in S_i$ arbitrary.
    Set $\eigval^*=\eigval_i(\PertVar^*)$
    and $u^*=u_i(\PertVar^*)$.
    Then, obviously $\Psi(\PertVar^*,u^*,\eigval^*)=0$.
    Also, note that $\det(J(u^*,\eigval^*))\neq 0$.

    This is most easily seen when changing into the eigenbasis of $N(\PertVar^*)$.
    Then, $N(\PertVar^*)$ becomes diagonal.
    Also, if we assume for simplicity of notation, that the fixed index $i=1$, then
    $u^*=u_i(\PertVar^*)=(1 0\ldots 0)^T$ becomes a standard basis vector and
    $\eigval_1(\PertVar^*)=\eigval^*$.
    Inserting into the formula for $J$ we get
    $$
    \det(J(u^*,\eigval^*))
        =
    \det
    \left(\begin{array}{cc}
            {\rm diag}(0,(\eigval_2(\PertVar^*)-\eigval^*)\ldots (\eigval_n(\PertVar^*)-\eigval^*))
            & -(1~ 0~ ...~0)^T \\
            (1~ 0~ ... ~0)     & 0
        \end{array}
    \right)
    $$
    When exchanging the first and the last line, this matrix becomes diagonal with non-zero determinant equal to
    $1\cdot \prod_{j\neq1}
    (\eigval_j(\PertVar^*)-\eigval_1(\PertVar^*))\cdot 1$
    which is non-zero because $\PertVar^*\in S_i$.

    Since $J(u^*,\eigval^*)$ is invertible
    the implicit function theorem implies the following:
    There is an open interval $U_i$ containing $\PertVar^*$ and
    a $\mathcal{C}^1(U_i)$ function $g_i:U_i\to \reals^{n+1}$
    which we may write as $g_i=(w_i^T,\zeta_i)$ with
    $w_i:U_i\to \reals^{n}$ and $\zeta_i:U_i\to \reals$
    such that $\Psi(\PertVar,w_i^T(\PertVar),\zeta(\PertVar))=0$ for $\PertVar\in U_i$
    and $g_i(\PertVar^*)=(u^*,\eigval^*)$.
    This means that $w_i$ is eigenvector of $N$ with eigenvalue $\zeta_i$
    for all $\PertVar\in U_i$ which coincide with $u_i$ and $\eigval_i$ at $\PertVar=\PertVar^*$.


(iii)
    Since all eigenvalues vary continuously in $\PertVar$,
    they cannot change their relative ordering in terms of size
    unless they coincide in between. In other words,
    the eigenvalues  will not change relative ordering
    within each connected component of $S_i$.
    As a consequence, and by continuity, the functions $\zeta_i$
    and $\eigval_i$ which coincide at $\PertVar=\PertVar^*$ must coincide
    in $U_i$. This establish differentiability.

(iv)
    The implicit function theorem allows to compute the
    derivatives of $w_i$ and $\zeta_i$ w.r.t $\PertVar$.
    Simpler, however, is to follow the same argument as
    given just before the statement of
    Theorem~\ref{thm:lambda_differentiability}
    to obtain at least
    $\zeta'(\PertVar)$.
    As step (iii) shows, this derivative is
    equal to $\eigval_i'$.
    The derivative of $u_i$ is only somewhat harder.

(v) The chain rule yields the derivative of $\singval_i$.

Note that working with $A_G$ instead of $N$ (cpre. cor.~\ref{cor:Frobenius_bound}) leads to the same
formula and condition for the singular values. Indeed, the eigenvalues
of $A_G$ coincide if either two singular values of $\AnyM}$ coincide or if
one vanishes, since then $\singval_i=0=-\singval_i$.
\end{proof}
}
\fi
%
%{\bf Examples}
%
\iffalse
Example 1:
Set $u_1=(\sin(1/\PertVar)~~ \cos(1/\PertVar))^T$,
$u_2=(-\cos(1/\PertVar) ~~ \sin(1/\PertVar))^T$,
$\singval_1=2\PertVar^4$,
$\singval_2=3\PertVar^4$,
and $v_i=u_i$.
Then, the family $M=V\Sigma U^T$ is $\mathcal{C}^1(\reals)$
with singular values $\singval_i$ that are even $\mathcal{C}^\infty(\reals)$
although $S_i=\reals\setminus\{0\}$.
Note that $u_i$ are $\mathcal{C}^\infty(S_i)$
but possess no limit as $\PertVar\to 0$.
In particular, they are not even continuous there.
\fi

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{./figures/SingValues_Diag+kappaId.jpg}
    \includegraphics[width=0.45\linewidth]{./figures/SingValues_15x15_GaussMatrix_Scale03.pdf}
    \caption{Singular values of two families of matrices of the form
    $M(\PertVar)=M_o+\PertVar{\rm Id}$ for $0\leq\PertVar\leq1$ on the horizontal axis.
    On the left, $M_o={\rm diag}(-0.4~~ -0.2 ~~-0.1)$
    demonstrates that even the largest singular value may not be
    increasing or everywhere differentiable.
    On the right, the entries of the $15\times 15$ matrix $M_o$
    are drawn from a zero-mean Gaussian distribution with $\Std=0.3$. This example
    demonstrates that the singular values may be non-convex
    and may have several extrema even
    without coinciding with others.}
    \label{fig:ex_101}
\end{figure}

Example 1:
The diagonal family $M=$diag$(-4 ~~ -2)+\PertVar${\rm Id} is
$\mathcal{C}^\infty(\reals)$.
When ordered by size,
the eigenvalues of $N=M^TM$
are $\max((\PertVar-4)^2,(\PertVar-2)^2)$
and
$\min((\PertVar-4)^2,(\PertVar-2)^2)$.
They are
not differentiable where they coincide.
In particular, the matrix norm of $N$ is not
differentiable at $\PertVar=3$.
%
The singular values of $M$
%the diagonal family $M=$diag$(-4 -2)+\PertVar${\rm Id}
are
$\singval_1=\max(|\PertVar-4|,|\PertVar-2|)$ and
$\singval_2=\min(|\PertVar-4|,|\PertVar-2|)$; they are
not differentiable
at their respective zeros. Also, the left singular
vectors $v_i$ changes sign at the zero of $\singval_i$
and is not even continuous there
(see  Figure~\ref{fig:ex_101} for a similar example).


\section{Singular Values in Deep Learning}
\label{sec:DeepLearning}


In this section we establish that the loss landscape of a deep network (DN) is governed locally by the singular values of the matrix of weights of a layer and that the difference between certain network architectures can be interpreted as a perturbation of this matrix. Combining this key insight with the perturbation theory of singular values for DNs, which will be developed in the sections to follow, will enable us to characterize the dependence of the loss landscape on the underlying architecture. Doing so, we will ultimately provide analytical insight into numerous phenomena that have been observed only empirically so far, such as the fact that so called ResNets \cite{he2016identity} are easier to optimize than ConvNets \cite{lecun1995convolutional}.

\subsection{The continuous piecewise-affine structure of deep networks}
\label{subsec:structure}

%\rolf{should we clarify in the title or the first par, that this section in on ConvNets? Nov 8}
%\randall{I think the title is ok because it works also for MLP etc, basically any feedforward without skip connection}
%\rolf{true...so I guess we leave it}

The most popular DNs  
contain nonlinearities that are
continuous piecewise affine (CPA), 
such as ReLU, leaky-ReLU, absolute value, and max-pooling nonlinearities \cite{goodfellow2016deep}. 
To be more precise, let $f_{\LayerIndex}$
denote a layer of a DN. 
We will assume that it can be written as an affine map
$
    W_{\LayerIndex}{\inlayeri}+b_{\LayerIndex}
$
followed by a
nonlinearity $\phi_{\LayerIndex}$:
\begin{equation}\label{EQU:layer}
  {\outlayeri}
  =
  f_{\LayerIndex}({\inlayeri})
  =
  \phi_{\LayerIndex}(W_{\LayerIndex}{\inlayeri}+b_{\LayerIndex}).
\end{equation}
The entries of the matrix $W_{\LayerIndex}$ are called \emph{weights},
the constant additive term $b_{\LayerIndex}$ is called the \emph{bias}.
More general settings can easily be employed; however, the above will be sufficient for our purpose. Indeed, 
the mentioned, commonly used nonlinearities can be
written in this form using
\begin{equation}\label{EQU:non_linearities}
  \phi_{\LayerIndex}(t)
  =
  \max(t,\eta t)
\end{equation}
where the max is  taken coordinate by coordinate.
Clearly, any nonlinearity in the form of 
(\ref{EQU:non_linearities}) is continuous and piecewise linear,
rendering the corresponding layer CPA.
The following choices for $\eta$ correspond to
ReLU ($\eta=0$) \cite{glorot2011deep},
leaky-ReLU ($0<\eta<1$) \cite{DBLP:journals/corr/XuWCL15} and
absolute value \cite{bruna2013invariant}
($\eta=-1$)
(see also \cite{reportRB,balestriero2018spline}).
In summary:
\begin{equation}\label{EQU:non_linearities_eta}
  \left\{
    \begin{array}{ll}
     \eta>0  & \mbox{leaky-ReLU} \\
      \eta=0  & \mbox{ReLU} \\
      \eta=-1 & \mbox{absolute value} \\
    \end{array}
    \right.
\end{equation}
For example, in two dimensions we obtain $\phi_{\LayerIndex}^{\rm (Abs)}(t_1,t_2)=(|t_1|,|t_2|)$.
%
We will consider only non-linearities that can be written in the form
\equ{non_linearities}.
Such non-linearities are in fact linear in each hyper-octant of space,
and can be written as
$$
    \phi_{\LayerIndex}(t)
    =
    D_{\LayerIndex}t,
$$
where $D_{\LayerIndex}$ is a diagonal matrix
with entries that depend on the signs
of the coordinates of the input $t=W_{\LayerIndex}{\inlayeri}+b_{\LayerIndex}$.
The diagonal entries of $D_{\LayerIndex}$ equal either $1$ or
 $\eta$ depending on the hyper-octant.

Consequently, the input space of the layer
$f_{\LayerIndex}$ is divided into \emph{regions}
which depend on $W_{\LayerIndex}$ and $b_{\LayerIndex}$
in which $f_{\LayerIndex}$ is affine
and can be rewritten as
\begin{equation}\label{EQU:locally_linear_layer}
  {\outlayeri}
  =
  f_{\LayerIndex}({\inlayeri})
  =
  \phi_{\LayerIndex}(W_{\LayerIndex}{\inlayeri}+b_{\LayerIndex})
  =
  (D_{\LayerIndex}W_{\LayerIndex}){\inlayeri}+D_{\LayerIndex}b_{\LayerIndex}.
\end{equation}
%
By the linear nature of ${\inlayeri}\mapsto W_{\LayerIndex}{\inlayeri}$,
these regions of the input space
(${\inlayeri}$-space) are piecewise linear.
Concatenating several layers into
a multi-layer $F({\inlayerone})=f_p\circ \ldots\circ  f_1({\inlayerone})$ then leads to a
division of its input space into piecewise linear regions, in which $F$
is affine, a result due to
\cite{reportRB,balestriero2018spline}.
In each linear region of linearity this multi-layer
reads as
$$
    {\outlayerp}
    =
    D_pW_p\ldots D_1 W_1 {\inlayerone} +  B_p,
$$
where all constant terms are collected in
$$
    B_p
    =
    D_pW_p\ldots D_2 W_2 b_1
    +
    D_pW_p\ldots D_3 W_3 b_2
    + \ldots +
%    D_pW_pb_{p-1}
%    +
    b_p.
$$
A multi-layer can be considered to be an entire DN or a part of one.

\begin{figure}
    \centering
    \includegraphics[width=0.3\linewidth]{./figures/partitioningalone_0_0.pdf}
    \includegraphics[width=0.3\linewidth]{./figures/partitioningalone_1_0.pdf}
    \includegraphics[width=0.3\linewidth]{./figures/partitioningalone_2_0.pdf}
    \caption{Iterative partitioning of input space by three consecutive layers
    of a toy Deep Network (DN). The first layer maps $\reals^2$ to $\reals^3$ producing three cuts
    and seven regions, one lying outside the visible part.
    }
    \label{fig:partitioning}
\end{figure}





\subsection{From ConvNets to ResNets and DenseNets, and learning}
\label{subsec:Conv_vs_Res}

A DN with an architecture $F({\inlayerone})=f_p\circ \ldots\circ  f_1({\inlayerone})$
as described above is called a \emph{Convolutional Network}
(ConvNet) \cite{lecun1995convolutional} whenever $W_k$ are circulant-block-circulant; otherwise it is called a multi-layer-perceptron. Without loss of generality we will focus on ConvNets. While such architectures have been at the origin of the new wave of deep learning successes, they are known to be intricate to effectively employ when the number of layers $p$ gets large. This motivated an alternative architecture.

When adding the input ${\inlayeri}$ to the output $\phi_{\LayerIndex}(W_{\LayerIndex}{\inlayeri}+b_{\LayerIndex})$
of a convolutional layer one obtains a \emph{residual layer}
which reads in each region of linearity as
\begin{equation}\label{EQU:locally_residual_layer}
  {\outlayeri}
  =
  f_{\LayerIndex}({\inlayeri})
  =
  \phi_{\LayerIndex}(W_{\LayerIndex}{\inlayeri}+b_{\LayerIndex})+{\inlayeri}
  =
  (D_{\LayerIndex}W_{\LayerIndex}+{\rm Id}){\inlayeri}+D_{\LayerIndex}b_{\LayerIndex}
\end{equation}
%
A ConvNet in which all (or most) layers are residual are called
\emph{Residual Networks} (ResNets) \cite{he2016identity}. {\em Densely Connected Networks} (DenseNets) \cite{huang2017densely} is to allow the residual connection to bypass not a single but multiple layers which reads in each of its regions as
\begin{equation}\label{EQU:locally_skip_residual}
  {\outlayerp}
  =
  (D_pW_p\ldots D_1W_1+{\rm Id}){\inlayerone}+B_p
\end{equation}
%
All of the above DN architectures are universal approximators. Learning the per-layer weights of any DN architecture is done ny solving an optimization problem that involves a training set, a differentiable loss function such as the mean-squared-error, and a weight update policy such as gradient descent. Hence, the key benefit of one architecture over another only emerges when considering the optimization problem, and in particular gradient based optimization. 

\subsection{Training}
\label{subsec:learning}

We propose to discuss the training of one specific layer of a network. Describing the optimization landscape of one layer independently of the others is sufficient as will become clear in the next sections, since we will be able to demonstrate that regardless of the other layers, each layer of some architectures benefit from a better conditional loss-landscape compare to other architectures. 

The trained layer is $f_0$; however, for clarity we drop the index $0$ and use the notation 
\begin{equation}
    {\outlayert}=f(\inlayert)=\phi(W\inlayert+b)=DW\inlayert+b
  \qquad\qquad\qquad\qquad\,\mbox{trained layer}
\end{equation}
for clear distinction. 
The layers following $f$ are the only ones relevant
in the study of the training of $f$.
This part of the network will be denoted by
$F=f_p\circ \ldots\circ  f_1$.
In  in each region it takes the form:
\begin{eqnarray}
  \label{EQU:trained_layer}
    {\outDN}
    =
%%%    AW\inlayert+B
    MDW\inlayert+B
  \qquad\qquad\qquad\,\mbox{[trained plus subsequent layers]}
\end{eqnarray}
Here, $B$ collects all the constants, $D$ represents the
nonlinearity of the trained layer in the current region, 
and $M$ collect the action of the subsequent layers $F$. 
We use the parameter $\PertVar$ in order to distinguish ConvNets and ResNets with $\PertVar=0$ corresponding to convolution
layers and $\PertVar=1$ to residual ones. The matrix $M=M(\PertVar)$ representing the subsequent layers $F$
becomes
\begin{eqnarray}
  \label{EQU:training_one_layer}
%%%   A &=&   (D_1W_1+\PertVar{\rm Id})D
   M=M(\PertVar) &=&   D_1W_1+\PertVar{\rm Id}
  \qquad\qquad\qquad\qquad\,\mbox{one layer}
  \\
  \label{EQU:training_multi_layer}
%%%   A &=&   (D_pW_p\cdots D_1W_1+\PertVar{\rm Id})D
   M=M(\PertVar) &=&   D_pW_p\cdots D_1W_1+\PertVar{\rm Id}
  \qquad\qquad\mbox{multi-layer}
%  \\
%  \label{EQU:training_onelayer_residual}
% {\outlayerp} &=&   (D_1W_1+{\rm Id})DWz+\beta_1
%  \qquad\mbox{one residual layer}
%  \\
%  \label{EQU:training_skip_residual}
%  {\outlayerp} &=&   (D_pW_p\ldots D_1W_1+{\rm Id})DWz+\beta_p
%  \qquad\mbox{residual}
\end{eqnarray}
%where $\beta_{\LayerIndex}$ collects the constant terms (bias)
%and where $p=1$ corresponds to one residual layer,
%$p>1$ to a skip residual layer.
%
%
As a shorthand we will often write 
\begin{equation}
    \label{EQU:Mo}
    M_o
    =
    M(0)
    =
    D_pW_p\cdots D_1W_1
\end{equation}
When saying ``let $M_o$ be arbitrary'' we mean that no restrictions on the factors of \equ{Mo} are imposed except for the $D_i$ to be diagonal and the $W_i$ be square. 
When choosing $D_p=\ldots=D_1=W_p=\ldots=W_2=$Id 
and $W_1$ arbitrary, we have $M_o=W_1$ arbitrary. So, there is no ambiguity in our usage of the term ``arbitrary''.


\subsection{Quadratic loss}
\label{subsec:quadr_loss}


We wish to quantify the advantage in training of a ResNet
architecture over a ConvNet one.
We consider a quadratic loss function such as the Mean Squared Error as mentioned in section~\ref{sec:intro} (cpre. (\ref{eq:loss})):
\begin{equation}
    \label{eq:loss_squared_out}
    L^{(\dcounter)} :=
%    \left\| y^{(\dcounter)}-
%    \widehat{y}^{(\dcounter)} \right\|_2^2
    \left\| y-\widehat{y} \right\|_2^2
    =
    (y-\widehat{y})^T(y-\widehat{y})
    =
    \left\| y \right\|_2^2
    -
    2y^T\widehat{y} 
%    -
%    \widehat{y}^Ty
    +  
    \left\|\widehat{y} \right\|_2^2
\end{equation}
Thereby we used that 
$y^T\widehat{y}=(y^T\widehat{y})^T=\widehat{y}^Ty$ since this is a real number.



Recalling that the DN is a continuous piecewise affine operator and fixing all parameters except for $W$ 
we may locally write $\widehat{y}=MD W z +B$ 
for all $W$ in some region $\mathcal{R}$ of $F$.


Writing $    \left\|\widehat{y} \right\|_2^2
=\widehat{y} ^T\widehat{y} $ we find
that the loss can be viewed as an 
affine term $P(W)$ with $P$ some polynomial of degree $1$
plus a quadratic term $\|MD W z \|_2^2$:
\begin{eqnarray}
\label{EQU:quadr_term_MSE}
    L^{(\dcounter)}
    =
    P(W)+\|MD W z \|_2^2
    \qquad
    (W\in\mathcal{R})
%    =
%    z^TW^TD^TM^TMDWz
%%%    \|A W z\|^2
%%%    =
%%%    z^TW^TA^TAWz
    .
\end{eqnarray}
Let us denote by $W_o=W_o(\PertVar,\mathcal{R})$ 
the minimum of the function $h(W)=P(W)+\|MD W z \|_2^2$
($W$ arbitrary)
which may very well lie outside $\mathcal{R}$.
Writing $\Delta W=W-W_o$ and
developing $h$ into its Taylor series at $W_o$
we find 
$h(W)=h(W_o)+\|MD \Delta W z \|_2^2$
since all first order derivatives of $h$ vanish at $W_o$.

It is worthwhile pointing out that the region  $\mathcal{R}$ 
does not change when changing the value 
of $\PertVar$ in $M=M(\PertVar)$ since 
$D\Delta Wz$ does not depend on $\PertVar$.
From this, writing $c=h(W_o)$ for short we get for any $\PertVar$
\begin{eqnarray}
    \label{EQU:loss_centered_at_min}
    L^{(\dcounter)}
    =
    c +\|M(\PertVar)D \Delta W z \|_2^2
    \qquad
    (W\in\mathcal{R})
    .
\end{eqnarray}

This means that the loss surface is in each region
$\mathcal{R}$ of $F$ a part of an exact ellipsoid 
and that its shape determined by the second order expression
$\|M(\PertVar)D \Delta W z \|_2^2$ as a function of $\Delta W$. 
The value $c$ should not be looked at as the 
minimum of the loss function, since $W_o$ may lie outside the 
region $\mathcal{R}$.

Before commenting further on the loss, however, let us untangle
the influence of the data $z$ (which remains unchanged during training). 
from
the weights $W$ in \equ{quadr_term_MSE} (analogous for $\Delta W$
in \equ{loss_centered_at_min}).

When listing these variables $W[ij]$ row by row in a ``flattened''
vector $w$, the term 
\equ{quadr_term_MSE} 
becomes a quadratic form with following matrix $Q$:
\begin{lem}
\label{lem:standard_quadratic_form}
In the quadratic term \equ{quadr_term_MSE} of the MSE 
we have the following matrices:
$W$ is $c\times d$, $(MD)$ is $c\times c$ and $z$ is $d\times 1$.
Denote the flattened version of $W$ by $w$ ($cd \times 1$)
and the singular values of $(MD)$
by $\singval_i$.
Let
$
    Q
    =
    \text{\rm diag}(z) \otimes (MD)
$
meaning
$$
    Q =
    \begin{pmatrix}
        z[1] MD & 0           & \dots & 0\\
        0       & z[2] MD    & \dots &0 \\
               &         &  \ddots    &  \\
         0      &         \dots & 0 & z[d] MD
%        z[1] A & 0           & \dots & 0\\
%       0       & z[2] A    & \dots &0 \\
%               &         &  \ddots    &  \\
%         0      &         \dots & 0 & z[d] A
    \end{pmatrix}.
$$
Then, we have (cpre.\equ{quadr_term_MSE})
\begin{equation}
\label{EQU:flattened_M}
    \|MD W z\|_2^2
%%%    z^TW^T(MD)^T(MD)Wz
    =
    w^TQ^TQw
%    \;\;\text{ with }\;\;
\end{equation}
and the singular values of $Q$ factor as follows 
\begin{equation}
\label{EQU:sing_vals_Q}
\singval_{ij}(Q)
=
\singval_i(MD) \cdot|z[j]| 
\end{equation}
with $1 \leq i \leq c$ and $1 \leq j \leq d$.
\end{lem}


\begin{proof}
    The following notation will be useful:
    Let $\pi_j(a)=[0;\dots;0; a; 0; \dots;0]$ where the $0$ stands for
    a column vector of zeros of the same length as the vector $a$,
    and where $\pi_j$ is
    formed by $j-1$ column vectors $0$
    followed by the column vector $a$, followed by similar $0$
    vectors to make $\pi_j$ of length $cd$.
%
    In other words, setting all of the matrix entries of $W$ to zero
    except for column $j$ which consists of a $c$-dimensional vector $a$,
    and then flattening the resulting matrix will result in $\pi_j(a)$.
    Due to the flexible definition of $\pi_j$ the analogous procedure
    works for $W^T$, setting all its columns to zero, except the $j$th and
    flattening it.


    Let us now proceed to the construction of
    the right singular vectors of $Q$,
    which we denote by $u^*_{ij}$,
    one for each coordinate of $z$, enumerated by $j=1,\dots,d$, and for
    each right singular vector $u_i$ of $(MD)$, enumerated by $i=1,\dots,c$.

    We set $u^*_{ij}=\pi_j(u_i)$.
    Recall this is the flattened version of the matrix of the same dimensions as $W$ with all entries
    zero, except for column $j$, which equals $u_i$.
%
    Note that these vectors $u^*_{ij}$ are orthonormal
for two reasons. For one,
    for fixed $j$ the $u_i$ are orthonormal Second, for fixed $i$
    $u^*_{ij}$ and $u^*_{ik}$ are orthogonal whenever $j\neq k$ by construction
    via $\pi$ since they correspond to different columns in $W$.

    Note that the action of $Q$ on
    vectors of the form $\pi_j(a)$ is
    simply $z_j\pi_j((MD)a)$.
    We obtain
    $$
        Qu^*_{ij}
        =
        Q\pi_j(u_{i})
        =
        z_j\pi_j((MD)u_{i})
        =
        z_j\pi_j(\sigma_i v_i)
        =
        z_j\sigma_i \pi_j(v_i)
        .
    $$
    We set $v^*_{ij}=\pi_j(v_i)$ and show that these are the left singular vectors
    of $Q$.
    Indeed,
    $$
        Q^Tv^*_{ij}
        =
        Q^T\pi_j(v_{i})
        =
        z_j\pi_j((MD)^Tv_{i})
        =
        z_j\pi_j(\sigma_i u_i)
        =
        z_j\sigma_i \pi_j(u_i)
        =
        z_j\sigma_i u^*_{ij}
        .
    $$
\hfill$\Box$
\end{proof}


\subsection{Condition number}
\label{subsec:cond_number}

After this clarification, let us return to the shape of the loss surface.
Lemma~\ref{lem:standard_quadratic_form} implies that characterizing the spectrum of the $Q$ matrix directly characterizes the geometry of the loss landscape of the trained layer $f$. 
The loss surface being exactly equal to a portion of an ellipsoid 
its curvature and higher dimensional eccentricity
has a considerable influence on the numerical behavior of the optimization. This is due to the use of gradient-based optimization, which is highly sensitive to the loss landscape geometry.
The higher dimensional eccentricity 
of this loss landscape
is in essence determined by the singular values of
the  matrix $Q$ due to 
\equ{loss_centered_at_min}. 
In essence, the larger the eccentricity the less accurately does  
the gradient point towards the maximal change of the loss 
when making a non-infinitesimal change in $W$.



The condition number $\CondNb$ of the matrix $Q$ constitutes 
 a measure of its
higher dimensional eccentricity and
indicates the difficulty of optimization by linear least squares.
% See wiki (last sentence before "discussion"): vanishing sing vals are ignored 
% https://en.wikipedia.org/wiki/Numerical_methods_for_linear_least_squares
It is defined as
the ratio of the largest singular value $\singval_1$
to the smallest non-zero singular value. Denoting 
the latter by $\singval_*$ for convenience, the
condition number of
an arbitrary matrix $A$ is given by
\begin{equation}\label{EQU:def_conditioning}
  \CondNb(A)
  :=
  \frac{\singval_1(A)}{
  \min\{\singval_i(A)\,:\,\singval_i(A)>0\}}
  =
  \frac{\singval_1(A)}{\singval_*(A)}.
\end{equation}


In summary, Lemma~\ref{lem:standard_quadratic_form} makes explicit how the data influences said loss landscape.
In particular, from \equ{sing_vals_Q} follows immediately:

\begin{cor}[The data factor]
\label{cor:standard_quadratic_form}
    The condition number of the matrix $Q$ 
    of Lemma~\ref{lem:standard_quadratic_form} 
    factors in the following sense:
    \begin{equation}
        \label{EQU:data_factor}
        \CondNb(Q)
        =
        \CondNb(MD)
        \cdot
        \CondNb(\mbox{\rm diag}(z))
    \end{equation}
 
\end{cor}

Since the data $z$ does not change during training, the performance of linear least squares optimization will be governed by $\CondNb(MD)=\CondNb(M(\PertVar)D)$.

We thus propose to study various perturbation settings in the next sections leading to two types of results: First, we study the evolution of the loss landscape of DNs when their architecture is continuously interpolated from a ConvNet ($\PertVar=0$) to a ResNet ($\PertVar=1$). 
Since the region $\mathcal{R}$ of $F$ does not depend on $\PertVar$ such an analysis is meaningful for understanding the optimization of the loss via 
\equ{loss_centered_at_min}.
Second, we investigate how the diagonal matrix $D$ perturbs the singular values of $M$.



\section{Perturbation of a DN's Loss Landscape When Moving from a ConvNet to a ResNet}
\label{sec:AddingIdentity}

Recall the special form  
$M(\PertVar)=M_o+\PertVar${\rm Id}
\equ{Mo}.
In this section we exploit the differentiability of 
$M(\PertVar)$ in order to study the perturbation of
its singular values when moving from
ConvNets with $\PertVar=0$  to ResNets with $\PertVar=1$    (see Section~\ref{subsec:Conv_vs_Res}).


A first simple but most useful consequence of Weyl's additive perturbation bound reads as follows:
\begin{lem}
    \label{lem:Weyl_bound}
    Let $M_o$ be arbitrary (see \equ{Mo}).
    We have
\begin{equation}
    \label{EQU:Weyl_bound}
    \PertVar-\singval_1(M_o)
    \leq
    \singval_i(M(\PertVar))
    \leq
    \PertVar+\singval_1(M_o)
\end{equation}  
\end{lem}

\begin{proof}
Apply \equ{uniform_bound} 
with $\AnyM=M(\PertVar)=M_o+\PertVar{\rm Id}$
and $\AnyMt=\PertVar{\rm Id}$ to get
$$
    |\singval_i(M(\PertVar))-\PertVar|
    \leq
    \singval_1(\AnyM-\AnyMt)
    =
    \singval_1(M_o)
    .
$$
\hfill$\Box$
\end{proof}

Also, due to the simple form of $M(\PertVar)$, the following fact is obvious:

\begin{lem}[Eigenvector]
  \label{lem:eigenvector}
    Let $M_o$ be arbitrary (see \equ{Mo}).
  Assume that $w=u_i(\PertVar_o)$ is an eigenvector of $M$ for some $\PertVar_o$
  with eigenvalue $t$.
  Then, for all $\PertVar$, the vector $w$ is an eigenvector and right singular vector of $M(\PertVar)$ with eigenvalue $t+\PertVar-\PertVar_o$
  and singular value $|t+\PertVar-\PertVar_o|$.
\end{lem}
Note that the singular value of the fixed vector $w$
may change order, as other singular values may increase or decrease at
a different speed.

Somewhat sharper bounds can be obtained using differentiability. 

\MoreDetails{
        A simple result concerns  with the sum of the eigenvalues
        $\eigval_i$ of $N=M^TM$ or equivalently the sum of squared singular values of $M$:
        \begin{equation}
            \label{EQU:def_sum_eigenvalues}
            \sumSQsing(\PertVar)
            :=
            \sum_{i=1}^n \eigval_i(\PertVar)
            =
            \sum_{i=1}^n \singval^2_i(\PertVar)
            =
            {\rm  tr}(N(\PertVar))
            =
            \|M(\PertVar)\|_2^2
            .
        \end{equation}
        Since the trace is the sum of the diagonal entries of $N$, a simple direct computation yields immediately the following result.
        
        \begin{lem}
            \label{lem:trace}
            Let $M_o$ be arbitrary (see \equ{Mo}).
            Then, $M'=$Id and 
            %$\mathcal{C}^{1}(\reals)$ 
            \begin{equation}
                \label{EQU:derivative_trace}
                \frac{d}{d\PertVar} \sumSQsing(\PertVar)
                =
                \sumSQsing'(\PertVar)
                =
                %\sum_i \eigval_i'(\PertVar)=
                {\rm tr}(N'(\PertVar))
                %={\rm tr}({M'}^T M + M^T M')(\PertVar)
                =
                2{\rm tr}({M'}^T M)
                =
              2{\rm tr}(M_o)+2n\PertVar
                .
            \end{equation}
        %    and
        %$$      
        %    \sumSQsing(\PertVar)=\sumSQsing(0)+2\PertVar{\rm tr}(M_o)+n\PertVar^2.
        %$$
        \end{lem}
}


\begin{lem}[Derivative]
  \label{lem:derivative_lambda_plusId}
    Let $M_o$ be arbitrary (see \equ{Mo}).
Writing  $u_i=u_i(\PertVar)$ for short, the derivative of the  eigenvalue $\eigval_i(\PertVar)$ of $M^TM$ becomes, on $S_i$ (see \equ{def_simple})
\begin{equation}
    \label{EQU:derivative_lambda_plusId}
        \eigval_i'(\PertVar)
        =
        u_i^T(M_o^T+M_o) u_i+2\PertVar
        =
        2u_i(\PertVar)^TM_o u_i(\PertVar)+2\PertVar
\end{equation}
On $S_i^*$ (see \equ{def_nonzero}) we have
\begin{equation}
    \label{EQU:derivative_sigma_plusId}
        \singval_i'(\PertVar)
        =
        \eigval_i'(\PertVar)/(2\singval_i)
        =
        u_i^T v_i
        =
        \cos(\alpha_i(\PertVar))
        ,
\end{equation}
where $\alpha_i(\PertVar)$ denotes the angle between the $i$-th left and right singular vectors.
\end{lem}

Using \equ{derivative_sigma_plusId} it is possible 
to compute the derivative
$\singval_i'(\PertVar)$ numerically.
(In a general  numerical setting, derivatives can only be estimated.)


\begin{proof}
We may apply Theorem~\ref{thm:lambda_differentiability} to the family $N(\PertVar)=M^TM$.
Note that $M'=$Id, whence 
$N'=(M')^TM+M^T(M')=M+M^T=M_o^T+M_o+2$Id.
Using $u_i^Tu_i=1$ we  find
$$
        \eigval_i'(\PertVar)
        =
        u_i^T(M^T+M) u_i
        =
        u_i^T(M_o^T+M_o) u_i+2\PertVar.
$$
Also, we have $u_i^TM_o^Tu_i=(u_i^TM_o^Tu_i)^T
=u_i^TM_ou_i$ since this is a real-valued number. 
This establishes \equ{derivative_lambda_plusId}.

In a similar way we find 
$        \eigval_i'(\PertVar)
        =
u_i^T(M^T+M) u_i=2(u_i^TM u_i)=2\singval_i u_i^Tv_i$. The chain rule implies
\equ{derivative_sigma_plusId}.
Alternatively, \equ{derivative_sigma_plusId}
follows from corollary~\ref{cor:sigma_differentiability}.
\hfill$\Box$ \end{proof}


Let us collect a few direct  consequences for the singular values.
From \equ{derivative_sigma_plusId} 
we have $|\singval_i'(\PertVar)|\leq1$ on $S_i^*$ which is obvious from  geometry
and is also reflected in lemma~\ref{lem:Weyl_bound}.
The eigenvectors of $M_o$, if such exist,
achieve extreme growth or decay.
\begin{lem}[Maximum Growth]
  \label{lem:max_growth}
    Let $M_o$ be arbitrary (see \equ{Mo}).
  Assume that
  %$\alpha_i(\PertVar_o)=0$
  $\singval'_i(\PertVar_o)=1$
  for some $\PertVar_o$.
  Then, $w=u_i(\PertVar_o)$ is eigenvector and right singular vector of $M(\PertVar)$
  with eigenvalue $t+\PertVar-\PertVar_o$ and singular value $|t+\PertVar-\PertVar_o|$
  for some $t>0$.
  % and all $\PertVar$.
%
  Analogous for
%  $\alpha_i(\PertVar_o)=\pi$
  $\singval'_i(\PertVar_o)=-1$
with $t<0$.
\end{lem}
%@@@ double text under PrintAll
Note that the singular value of the fixed vector $w$
may change order, as other singular values may increase or decrease at
a different speed.
Related to this fact is the following.

\begin{lem}[Non-Vanishing Singular Values]
  \label{lem:vanishing_sing_value}
  Let $M=M_o+\PertVar{\rm Id}$.
  Assume that $\singval_i(\PertVar_o)=0$ for some $\PertVar_o$.
  Then, $w=u_i(\PertVar_o)$ is an eigenvector and right singular vector of $M$
  with eigenvalue $\PertVar-\PertVar_o$ and singular value $|\PertVar-\PertVar_o|$.
%
  Consequently, if $M_o$ has no eigenvectors, then $\singval_i(\PertVar)\neq 0$
  for all $\PertVar$ and $i$.
  % and $\min\{\singval_i(\PertVar)\,:\,0\leq\PertVar \leq 1\}>0$,  for all $i$.
\end{lem}


Stronger consequences for the singular values of $M$ emerge from a look at their squares, the eigenvalues of $M^TM$.
In order to bound the derivative $\eigval_i'$ 
we use the following notation  throughout the paper:
\begin{defi}
\label{def:tau}
For a family of matrices of the form $M(\PertVar)=M_o+\PertVar${\rm Id} 
denote the smallest eigenvalue of the symmetrical matrix $M_o^T+M_o$ by $\underline{\tau}$ and
its largest by $\overline{\tau}$.
\end{defi}
Note that due to
$\underline{\tau}\leq \overline{\tau}$
\begin{equation}\label{EQU:OpNorm_MT+M}
  \|M_o^T+M_o\|_{\rm Op}
  =
  \max(
  |\underline{\tau}|,|\overline{\tau}|
    )
  =
  \max(
  -\underline{\tau},\overline{\tau}
    )
  \leq
  2\singval_1(M_o)
  .
\end{equation}
Using \equ{derivative_lambda_plusId} we have the following immediate result.

\begin{lem}
\label{lem:sigma_plusId}
    Let $M_o$ be arbitrary (see \equ{Mo}).
%Writing  $u_i=u_i(\PertVar)$, 
We have on $S_i$ (see \equ{def_simple})
\begin{equation}
    \label{EQU:lambda_prime_bounds}
    \underline\tau+2\PertVar
    \leq
    \eigval_i'(\PertVar)
    \leq
    \overline\tau+2\PertVar.
\end{equation}
\end{lem}

As we state next, 
the bound on $\eigval'_1$ \equ{lambda_prime_bounds} is indeed somewhat sharper
than $\singval'_1(\PertVar) \leq 1$ 
(see \equ{derivative_sigma_plusId}) 
leading to a sharper bound than
the following obvious bound (cpre. lemma~\ref{lem:Weyl_bound}):
  \begin{equation}\label{EQU:max_value}
    \singval_1(\PertVar)
    =
    \|M(\PertVar)\|_{\rm Op}
    \leq
    \PertVar+\singval_1(M_o)
  \end{equation}

\begin{prop}[Largest Singular Value, Sharpness of bound]
  \label{prop:max_value}
    Let $M_o$ be arbitrary (see \equ{Mo}). We have
  \begin{equation}\label{EQU:max_value_stronger}
    \sqrt{\singval_1^2(M_o)
    +
    \PertVar\underline{\tau}  % from derivative, works only for largest sing val=op norm bc convex
    +\PertVar^2}
    \leq
    \singval_1(\PertVar)
    =
    \|M(\PertVar)\|_{\rm Op}
    \leq
    \sqrt{\singval_1^2(M_o)
    +
%    \PertVar  \max(  -\underline{\tau},\overline{\tau}  ) % from operator bound
    \PertVar\overline{\tau}  % from derivative, works only for largest sing val=op norm bc convex
    +\PertVar^2}
  \end{equation}
%
  If equality holds in \equ{max_value} for some $\PertVar_o$
  then it holds for all $\PertVar\geq0$.
\MoreDetails{  
  In fact, 
  equality holds in \equ{max_value} for all $\PertVar\geq0$
  if and only if
  equality holds in \equ{max_value} for some $\PertVar_o$
  if and only if
  $w=u_1(0)$ is actually an eigenvector of $M_o$ with positive eigenvalue equal to $s_1(0)$.}
  Further, then $\overline{\tau}=2\singval_1(0)\geq -\underline{\tau}$
  and the upper bound of \equ{max_value_stronger} coincides with \equ{max_value}.

\MoreDetails{
    Both, $\singval_1(\PertVar)$ and $\eigval_1(\PertVar)$ are convex functions of $\PertVar$
  and differentiable in all but countable many $\PertVar>0$.
 }
  The derivative of $\singval_1(\PertVar)$ is either equal to $1$ for all $\PertVar>0$
  or it is non-decreasing and strictly below $1$ where it exists.
\end{prop}
As we will see, certain random matrices of interest 
tend to achieve the  upper bound 
in form of the deterministic expression 
\equ{max_value_stronger} 
quite closely with high probability.

\if 0
 If
 $w=u_1(0)$ is an eigenvector of $M_o$ with NEGATIVE eigenvalue equal to $-s_1(0)$
 then $\underline{\tau}=-2\singval_1(0)$, $\alpha_1(0)=\pi$,
 $\singval'_1(0)=-1$ and $\singval_1$ decays
 at first,
 not being able to get up to speed and reach $\singval_1(0)+\PertVar$ ever again
 for $\PertVar>0$.
\fi





\begin{proof}
Obviously, $\|M_o+\PertVar{\rm Id}\|_{\rm Op} \leq \|M_o\|_{\rm Op} + \PertVar$, which
implies \equ{max_value}.
\if 0
%The slightly stronger \equ{max_value_stronger} !!!! version "from operator norm"
% follows similarly from %$\singval_1(\PertVar)=\sqrt{\eigval_1(\PertVar)}=\sqrt{\|M^T(\PertVar)M(\PertVar)\|_{\rm Op}}$.
\fi
To show the stronger bound \equ{max_value_stronger}, we establish first convexity.
Let $0<p<1$, $q=1-p$ and $0\leq x\leq y$. Then
\begin{eqnarray*}
    \singval_1(px+qy)
    &=&
    \|M_o+ (px+qy) {\rm Id}\|_{\rm Op}
    =
    \|p(M_o+ x {\rm Id} ) + q(M_o+ y {\rm Id} )\|_{\rm Op}
    \\
    &\leq&
    \|p(M_o+ x {\rm Id} ) \|_{\rm Op} + \| q(M_o+ y {\rm Id} )\|_{\rm Op}
    =
    p\singval_1(x)+q\singval_1(y)
    .
\end{eqnarray*}
Next, convexity of $\eigval_1$ follows since $x\mapsto x^2$ is convex:
$$
    \singval_1^2(px+qy)
    \leq
    \left(    p\singval_1(x)+q\singval_1(y) \right)^2
    \leq
    p\singval_1^2(x)+q\singval_1^2(y)
    .
$$
As a convex function,
$\eigval_1(\PertVar)$ is differentiable at all but countably many points.
We may extend its derivative to all $x$ in the following way,
in slight abuse of notation
$$
    \eigval_1'(x+)
    :=
    \inf\{ \eigval_1'(y)\,:\, y\geq x \mbox{ and $\eigval_1'(y)$ exists} \}
$$
Note that $   \eigval_1'(x+) $ is monotone and bounded by $\overline\tau+2x\leq\overline\tau+2\PertVar$
for $x\in[0,\PertVar]$. Thus, it is even Riemann-integrable on $[0,\PertVar]$. It is easy to check
that any upper Riemann-sum $\overline R$ and any lower Riemann-sum $\underline R$
satisfy $\underline R \leq \eigval(\PertVar)-\eigval(0) \leq \overline R$. Therefore,
\begin{eqnarray}
    \label{EQU:lambda_integral}
    \eigval(\PertVar)-\eigval(0)
    =
    \int_0^\PertVar \eigval_1'(x+) dx
    \leq
    \int_0^\PertVar  \overline\tau+2x dx
    =
    \PertVar    \overline\tau + \PertVar^2
    .
\end{eqnarray}
Similarly
$
\eigval(\PertVar)-\eigval(0)
    \geq
    \PertVar    \underline\tau + \PertVar^2
.$
This implies \equ{max_value_stronger}. Its upper bound is slightly stronger than
\equ{max_value} due to \equ{OpNorm_MT+M}.


Next, if $w$ is an eigenvector with positive eigenvalues
then the equality holds from Lemma~\ref{lem:eigenvector}.
%
Vice versa, we have $|\singval'_1(\PertVar+)|\leq 1$ from \equ{derivative_sigma_plusId}.
Therefore, if equality holds in \equ{max_value}, then
there must be at least one value $\PertVar_o$
where $\singval'_1(\PertVar_o)=1$ and $\alpha_i(\PertVar_o)=0$.
By Lemma~\ref{lem:max_growth} $w=u_i(\PertVar_o)$
is an eigenvector of $M_o$.
\hfill$\Box$ \end{proof}

The growth of the other singular values 
can be bounded in the same way as 
$\singval_1$ in proposition~\ref{prop:absolute_value},
provided that $\eigval_i=\singval_i^2$
is differentiable in all but finite many points of
$[0,\PertVar]$. For this, it is sufficient that it be
piecewise simple, meaning that $[0,\PertVar]\setminus S_i$
consists only of finite many points.

\MoreDetails{
        \begin{thm}
        \label{thm:lambda_bounds}
            Let $M_o$ be arbitrary (see \equ{Mo}).
            Fix $i$
        and let $S_i$ as in \equ{def_simple}.
        %
        Assume that either $i=1$ or
            that $\eigval_i=\singval_i^2$
        is differentiable in all but finite many points of
        $[0,\PertVar]$. For this, it is sufficient that it be
        piecewise simple, meaning that $[0,\PertVar]\setminus S_i$
        consists only of finite many points.
        Then,
        \begin{equation}
            \label{EQU:lambda_increase_bounds}
            \PertVar\underline\tau+\PertVar^2
            \leq
            \eigval_i(\PertVar)-\eigval_i(0)
            \leq
            \PertVar\overline\tau++\PertVar^2.
        \end{equation}
        \end{thm}
        
        \begin{proof}
          For $i=1$ this is established in Proposition~\ref{prop:max_value}.
%          For $n=2$ we conclude from Lemma~\ref{lem:trace}
%          that $\eigval_2'(x+):=      2{\rm tr}(M_o)+2nx  -\eigval_1'(x+)$ 
%          is Riemann-integrable (cpre. \equ{lambda_integral}).
%          The claim follows by integration similar to
%          \equ{lambda_integral}.
          For $i>1$ we proceed similarly to
          \equ{lambda_integral}; however, instead of extending the derivative
          one subdivides $[0,\PertVar]$ into intervals in which the derivatives exist.
        \hfill$\Box$ \end{proof}
}

Combining lemma~\ref{lem:Weyl_bound}, proposition\ref{prop:max_value} and  the above remark
%and recalling \equ{def_conditioning}, 
we obtain the following.

\begin{thm}
\label{thm:chi_bounds}
    Let $M_o$ be arbitrary (see \equ{Mo}).
Assume that
$\singval_1(M_o)< 1$.
Then
\begin{equation}
    \label{EQU:cond_bound_via_OpNorm}
    \CondNb(M_o+{\rm Id})
    \leq
    \frac{\sqrt{1+\overline\tau+\singval_1(M_o)^2}}{1-\singval_1(M_o)}
    \leq
    \frac{1+\singval_1(M_o)}{{1-\singval_1(M_o)}}.
\end{equation}
Alternatively, assume that
$\underline{\tau}\geq -1$ and that
$\singval_n(\PertVar)$ is piecewise simple in $[0,1]$.
Then
\begin{equation}
    \label{EQU:cond_bound_via_Tau}
    \CondNb(M_o+{\rm Id})
    \leq
    \sqrt{\frac{1+\overline\tau+\singval_1(M_o)^2}{1+\underline\tau+\singval_n(M_o)^2}}
    \leq
    \frac{1+\singval_1(M_o)}{\sqrt{1+\underline\tau}}.
\end{equation}
\end{thm}
We list all four bounds due to their different advantages.
Due to \equ{OpNorm_MT+M} the first bounds in both,
\equ{cond_bound_via_OpNorm} as well as \equ{cond_bound_via_Tau}
are in general sharper than the second. 
Indeed, for random  matrices as used in Section~\ref{sec:probabilities}
we have typically 
$\overline\tau\simeq\sqrt{2}\singval_1(0)<2\singval_1(0)$.
The second bounds are simpler and  sufficient in certain
deterministic settings.

The first bound of \equ{cond_bound_via_Tau} is the tightest
of all four bounds for the mentioned random matrices. Also,
it paves the way for the next result.
It's drawback lies in the technical assumption on the piecewise simplicity of the smallest singular value.

\MoreDetails{
        More detailed information on the ratio of singular values is provided by
        the next result.
        \begin{lem}
        \label{lem:conditioning}
            Let $M_o$ be arbitrary (see \equ{Mo}).
        Let $0<\gamma<1$ be arbitrary.
        Assume that (\ref{EQU:lambda_increase_bounds}) holds.
        %and that $\underline{\tau}\geq -1$.
        Let $i$ and $j$ be such that
        $0<\singval_i(0)\leq\singval_j(0)$.
        If $n>2$ assume that $\eigval_i=\singval_i^2$
        is piecewise simple.
        If $j>2$ assume the same for $\eigval_j$.
        Provided
        \begin{equation}
            \label{EQU:conditioning_condition}
            \underline\tau+1
            \geq
            \eigval_i(0)\frac{1-\gamma}{\gamma}
            +
            \frac{\overline\tau+1}{\gamma}\cdot\frac{\eigval_i(0)}{\eigval_j(0)}
            \geq 0
            ,
        \end{equation}
        the ratio $\singval_j/\singval_i$
        decreases at least by a factor $\sqrt\gamma$ when adding Identity to $M_o$.
        In other words:
        \begin{equation}
            \label{EQU:conditioning_bound}
            \frac{\eigval_j(1)}{\eigval_i(1)}
            \leq
            \gamma\frac{\eigval_j(0)}{\eigval_i(0)}
        \end{equation}
        In particular,
        if
        $
            {\eigval_j(0)}/{\eigval_i(0)}
            \geq
            (\overline\tau+1)/(\underline\tau+1)
        %    \underline\tau+1
        %    \geq
        %    (\overline\tau+1)\frac{\eigval_i(0)}{\eigval_j(0)}
            \geq 0
            ,
        $
        then
        the ratio $\singval_j/\singval_i$
        does not increase when adding Identity to $M_o$.\end{lem}
}

\MoreDetails{
            Of particular interest in our context is the question, whether adding the residual link, thus passing from a ConvNet to a ResNet, of from $M(0)$ to $M(1)$. To this end, we establish the following:
            \begin{thm}
            \label{thm:conditioning}
            Let $M_o$ be arbitrary (see \equ{Mo}).
            Assume that the smallest singular value $\singval_n(\PertVar)$ of $M(\PertVar)=M_o+\PertVar$Id 
            is piecewise simple and non-zero ($\singval_{*}=\singval_n$) for $0\leq \PertVar \leq 1$.
            Then, we have:
            
            If $\CondNb(M_o)^2\geq    (\overline\tau+1)/(\underline\tau+1)$ then 
            \begin{equation}
            \label{EQU:ResNet_beats_ConvNet}
                \CondNb(M_o)\geq    
                \CondNb(M_o+{\rm Id})
            \end{equation}
            \end{thm}
}

\begin{proof}
From proposition~\ref{prop:max_value} and lemma~\ref{lem:Weyl_bound}
we get the first inequality of \equ{cond_bound_via_OpNorm};
the second part follows from 
$\overline\tau\leq 2\singval_1(0)$.

Using the same type of argument as for 
proposition~\ref{prop:max_value}, especially
\equ{lambda_prime_bounds} and \equ{lambda_integral},
and writing
for short $\singval_i(\PertVar)=\singval_i(M(\PertVar))$
we get
$
\singval_n^2(0)
    +
    \underline{\tau}  
    +1
\leq
\singval_n^2(1)
$
and the first inequality of \equ{cond_bound_via_Tau};
the second part follows again from 
$\overline\tau\leq 2\singval_1(0)$.
%
\MoreDetails{
            Simple algebra yields
            $$
                \singval_n^2(0)
                +
                \underline{\tau}  
                +1
                \geq
                \singval_n^2(0)
                +
                (\overline\tau+1)/\CondNb(M_o)^2
                =
                \left[\singval_1^2(0)
                +
                (\overline\tau+1)\right]
                /\CondNb(M_o)^2
            $$
            The first inequality of \equ{cond_bound_via_Tau} completes the proof.
            %
}
\hfill$\Box$ \end{proof}

\section{Influence of the Activation Nonlinearity on a Deep Network's Loss Landscape }
\label{sec:PerturbationDiagonal}

As put forward in section~\ref{sec:DeepLearning}, each layer of a DN can be represented locally as a product of matrices $D_iW_i$ where 
$W_i$ contains the weights of the layer while 
$D_i$ captures the effect of the non-linearity, 
being diagonal with entries equal to $\eta$ or $1$ (cpre.\equ{non_linearities_eta} and \equ{locally_linear_layer}).

In the last section we explored how the singular values of a matrix $M_o$
change when adding identity, i.e., when
moving from a ConvNet to a ResNet.
In this section we explore the effect of the non-linearities on the singular values.
\if 0
%%%@ old notation for diagonal nonlinearity matrices
    Some notation: let $M$ be a $n \times n$-matrix.
    Let $\boldk$ denote a vector of length $m$ with $0\leq m\leq n$
    and who's entries are strictly increasing:
    $k_1<k_2<\ldots<k_m$.
    Let
    \begin{equation}\label{EQU:Dk(eta)}
        D^{(\sboldk)}
        =
        D^{(\sboldk)}(\eta)
        =
        {\rm diag}(\underbrace{1\ldots 1}_{k_1-1}~ \eta ~ \underbrace{1\ldots 1}_{k_2-k_1-1}~\eta~\ldots)
    \end{equation}
    denote the diagonal matrix of the same size as $M$
    with diagonal entries $1$ except for the positions indicated by
    %the vector $k=(k_1,\ldots,k_m)$ (with $k_1>\ldots>k_m$)
    %which are set to $\eta$.
    $\boldk$ which are set to $\eta$.
    If \boldk~is empty ($m=0$) we set $D^{(\sboldk)}=\rm Id$.
\fi
To this end, let $\mathcal D(m,n,\eta)$ denote the set of all $n \times n$ diagonal matrices
with exactly $m$ diagonal entries $\eta$ and $n-m$ entries $1$:
    \begin{eqnarray}\label{EQU:Dk(eta)}
        \!\!\!\!\!
        \mathcal{D}(m,n,\eta)=
        \{D={\rm diag}(\eigval_1,\ldots,\eigval_n)
        :
        \eigval_i\in\{\eta,1\},
        {\rm trace}(D)=m\eta+n-m
        \}.
    \end{eqnarray}
We will always assume that $0\leq m \leq n$.
Note that
$\mathcal D(0,n,\eta)=\{{\rm Id}\}$
and
$\mathcal D(n,n,\eta)=\{\eta{\rm Id}\}$


\subsection{Absolute value}

Intuitively, if most of the diagonal entries of $D$
equal $1$ or $-1$ then the singular values of $DM$ and $M$ should not
differ by too much. This is trivially the case for $\eta=-1$, corresponding
to the absolute value (see (\ref{EQU:non_linearities_eta})).

\begin{prop}[Absolute Value]
  \label{prop:absolute_value}
  \sloppy
    Let $M_o$ be arbitrary (see \equ{Mo}).
  For any $D\in\mathcal{D}(m,n,-1)$ we have
  \begin{equation}
    \label{EQU:absolute_value}
    \singval_i(M)
    =
    \singval_i(MD)
    =
    \singval_i(DM).
  \end{equation}
\end{prop}
\begin{proof}
  This is a simple consequence of the SVD.
  Since $D$ is orthogonal due to $\eta=-1$,
  $DV$ and $DU$ are orthogonal as well.
  Multiplication by $D$ only changes the singular vectors,
  not the singular values: $DM=D(V\Sigma U^T)=(DV)\Sigma U^T$
  and $MD=(V\Sigma U^T)D=V\Sigma (DU)^T$.
\hfill$\Box$ \end{proof}

\subsection{ReLU}
The next simple case is the ReLU activation, corresponding to $\eta=0$ in (\ref{EQU:non_linearities_eta}). As we state next, the singular values of a linear map $M$ decrease when the map is combined with a ReLU activation, from left or right:

\begin{lem}[ReLU Decreases Singular Values]
  \label{lem:ReLU_decrease}
  ~\\
    Let $M_o$ be arbitrary (see \equ{Mo}).
  For any $D\in\mathcal{D}(m,n,0)$ we have
  \begin{equation}
    \label{EQU:ReLU_decreases}
    \singval_i(M)
    \geq
    \singval_i(MD)
    \qquad\mbox{and}\qquad
    \singval_i(M)
    \geq
    \singval_i(DM)
  \end{equation}
\end{lem}
Note that a similar result holds for leaky ReLU ($\eta\neq0$), however only for $i=1$.
This follows from the fact that $\singval_1(MD)\leq \singval_1(M)\singval_1(D)$ for any two matrices $M$ and $D$.

\begin{proof}
  Lemma~\ref{lem:ReLU_decrease}
  is a simple consequence of the Cauchy interlacing property by deletion (see (\ref{EQU:deletion})).
\hfill$\Box$ \end{proof}

As a consequence we have for ReLU's that
$
    |
    \singval_i(M)
    -
    \singval_i(DM)
    |
    =
    \singval_i(M)
    -
    \singval_i(DM)
$
and analogous for $MD$.
\if 0
    $
        |
        \singval_i(M)
        -
        \singval_i(MD)
        |
        =
        \singval_i(M)
        -
        \singval_i(MD)
    $
\fi
This motivates the  computation of the difference
of traces which equals the sum of squares of singular values
(recall (\ref{EQU:frobenius_norm})).
\begin{prop}[ReLU]
  \label{prop:ReLU_output}
  %Let $0\leq\eta\leq1$.
\if 0
      %%%@
      Let $D=D^{(k)}(0)$
      with integer $k$, setting only one diagonal entry to zero.
      Let $\tilde M=MD$.
      Denote by ${\singval_i}$ the singular values of $M$ and
      by $\tilde{\singval_i}$ those of
      $\tilde M$,
      %$\tilde M=D^{(k)}(\eta)M$,
      both ordered by size.
      In analogous fashion denote by $\sumSQsing$ and $\tilde\sumSQsing$
      the sum of squares of the corresponding singular values.
      Then,
      \begin{equation}
        \label{EQU:ReLU_trace_output}
        \sumSQsing-\tilde\sumSQsing
        =
        \sum_{i=1}^n
            \singval_i^2-\tilde\singval_i^2
    %        \singval_i^2(M) - \singval_i^2(\tilde M)
        =
    % only for ReLU, not for leaky ReLU:
        \sum_{i=1}^n
            |\singval_i^2-\tilde\singval_i^2|
    %       |\singval_i^2(M) - \singval_i^2(\tilde M)|
        =
    %    (1-\eta^2)\sum_{i =1}^{m} \sum_{j=1}^{n} M[k_i j]^2
    %    (1-\eta^2) \sum_{j=1}^{n} M[k j]^2
        \sum_{j=1}^{n} M[j k]^2
      \end{equation}
    More generally,
    let
    $D=D^{(\sboldk)}$
\fi
  \label{prop:ReLU_multiple_output}
  ~\\
    Let $M_o$ be arbitrary (see \equ{Mo})
    Let $\PertVar$ be arbitrary and write $M$ instead of $M(\PertVar)$ for short.
  For any $D\in\mathcal{D}(m,n,0)$ the following holds:
  Let $k_i$ ($i=1\ldots m$) be such that
    $D[k_ik_i]=0$.
%    With the notation of prop.~\ref{prop:ReLU_output}
      Denote by ${\singval_i}$ the singular values of $M$ and
      by $\tilde{\singval_i}$ those of
      $MD$,
  Then,
  \begin{eqnarray}
    \label{EQU:ReLU_multiple_trace_output}
    \sum_{i=1}^n \singval_i^2
    -
    \sum_{i=1}^n \tilde\singval_i^2
    =
    \sum_{i=1}^n
        |\singval_i^2-\tilde\singval_i^2|
    &=&
    \|M\|_2^2-\|MD\|_2^2
    =
    \sum_{i=1}^m
    \sum_{j=1}^{n} M[j k_i]^2
%%%    ~~\geq~~
%%%    |\singval_i-\tilde\singval_i|^2
    \\
    \label{EQU:ReLU_multiple_singval_output}
    \sum_{i=1}^n
    |\singval_i-\tilde\singval_i|^2
    &\leq&
    \sum_{i=1}^m
    \sum_{j=1}^{n} M[j k_i]^2.
%%\if 0
%%   %moved to later
%%    \\
%%    \label{EQU:ReLU_multiple_frobenius}
%%    \sum_{i=1}^{n}
%%        \Big|
%%            \singval_i^2-\tilde\singval_i^2
%%        \Big|^2
%%    &\leq&
%%    \sum_{i,j=1}^{n} \left(\sum_{i=1}^m M[k_i i]M[k_p j] \right)^2
%%\fi
  \end{eqnarray}
\end{prop}

\begin{proof}
\if 0
    %%%@ proof one ReLU
    Let us first establish the result for one active ReLU,
    meaning $D=D^{(k)}(0)$.
    The equality (\ref{EQU:ReLU_trace_output})
    %of the first formula
    follows from
    $
    %    \sumSQsing(M)-\sumSQsing(\tilde M)
        \sumSQsing-\tilde\sumSQsing
        =
        \|M\|_2^2-\|\tilde M\|_2^2
    $
    .
    %and writing the squared Frobenius norm $\|M\|_2^2$ of a matrix $M$
    %as the sum of the squared $\LayerIndex_2$-norms of its lines.

    The inequality (\ref{EQU:ReLU_singval_output})  follows from (\ref{EQU:uniform_bound}) and
    $
        \singval_1^2(M-\tilde M)
        =
        \|M-\tilde M\|_2^2.
    $
    which holds due to $M-\tilde M$ being of rank $1$.

    Interestingly, $\|M\|_2^2-\|\tilde M\|_2^2=\|M-\tilde M\|_2^2$ in this special setting.

    Clearly, it is enough to establish the result for arbitrary $m$.
\fi%
%
Write $\tilde M=MD$ for short.
The following equality simplifies computation and holds in this special setting
because $D$ amounts to an orthogonal projection allowing to apply Pythagoras:
$ \|M\|_2^2
    =
    \|\tilde M\|_2^2
    +
    \|M-\tilde M\|_2^2
.
$
This can also be verified by direct computation.
Lemma~\ref{lem:ReLU_decrease} implies
$$
%    \sumSQsing(M)-\sumSQsing(\tilde M)
%%%@    \sumSQsing-\tilde\sumSQsing
    \sum_{i=1}^n
        |\singval_i^2-\tilde\singval_i^2|
    =
    \sum_{i=1}^n \singval_i^2
    -
    \sum_{i=1}^n \tilde\singval_i^2
    =
    \|M\|_2^2-\|\tilde M\|_2^2
    =
    \|M-\tilde M\|_2^2
    =
    \sum_{i=1}^m
    \sum_{j=1}^{n} M[jk_i]^2,
$$
yielding \equ{ReLU_multiple_trace_output}.
Using Corollary~\ref{cor:Frobenius_bound}
with ${\AnyM}=M$ and ${\AnyMt}=\tilde M$ we get \equ{ReLU_multiple_singval_output}.
\if 0

    In this context recall  $a^2-b^2=(a-b)(a+b)$ and
    observe that in our applications
    $|\singval_i-\tilde\singval_i|^2$ is rather small.
    Thus, we should expect \equ{ReLU_multiple_trace_output}
    to be stronger than \equ{ReLU_multiple_singval_output}
    in our application.
\fi
\hfill$\Box$ \end{proof}

Bounds on the effect of non-linearities at the input can be obtained easily from
bounds at the output using the following fact.
\begin{prop}[Input-Output via Transposition]
  \label{prop:input-output}
  Let $D$ be diagonal, then
  \begin{equation}\label{EQU:input-output}
    \singval_i(MD)
    =
    \singval_i(DM^T).
  \end{equation}
\end{prop}

\begin{proof}
This follows from the fact that matrix transposition does not alter singular values.
%combined with $D=D^T$.
\end{proof}



\section{Bounding  the Weights of a ResNet Bounds its Condition Number}
\label{sec:Identity_withDiagonal}


In this section, we combine the results of the preceding two sections in order to quantify 
how bounds
on the entries of the matrix $W_i$
translate into bounds on the condition number. 
As we have seen, this is of relevance in the context of optimizing
DNs, especially when comparing ConvNets to ResNets (recall
Section~\ref{subsec:Conv_vs_Res}).

To this end, we will proceed in three steps:
\begin{enumerate}
    \item Bounds on the weights $W_i[jk]$ translate into bounds of $M(0)$ (ConvNet)
    \item Perturbation when adding a residual link, moving from  $M(0)$ (ConvNet) to  $M(1)$ (ResNet)
    \item Perturbation by the nonlinearity of the trained layer (passing from $M(1)$ to $M(1)D$)
\end{enumerate}

Also, we treat the two cases of deterministic weights (hard bounds)  and random weights (high probability bounds) separately.


\subsection{Hard bounds}
\label{sec:hard_bounds}

We start with a few facts on how hard bounds on the entries
are inherited by the entries and singular values of
perturbed versions of the matrix.
We use the term ``hard bounds'' to distinguish the following results for a deterministic setting 
from ``high probability bounds'' for a random setting 
some of which are in terms of random variables themselves
and which apply only with a certain probability as indicated.

\begin{lem}
  \label{lem:op_norm_hard_bound}
  Assume that all entries of the $n\times n$ matrix $W_i$
  are bounded by the same constant: $|W_i[jk]|\leq c$.
  Then
  \begin{equation}\label{EQU:sigma1_hard_bound}
    \singval_1(W_i)
    \leq
    cn,
  \end{equation}
  with equality, e.g., for the matrix $W_i$ with all entries equal to $c$.
\end{lem}

\begin{proof}
  The bound is a simple consequence of (\ref{EQU:operator_norm}):
    $\singval_1(W_i) \leq \|W_i\|_2 \leq cn$.
%
  If all entries of $W_i$ are equal to $c$, then the unit vector
  $u_1=1/\sqrt n (1,\ldots,1)$ achieves $W_i\cdot u_1=cn\cdot u_1$.
\hfill$\Box$ \end{proof}

\begin{lem}
  \label{lem:product_hard_bound}
  Let $W_i$ ($i=1,\ldots, p$) be
  matrices as in Lemma~\ref{lem:op_norm_hard_bound}.
  Assume that $c\leq 1/n$.
  Let $D_i$ ($i=1\ldots p$) be diagonal matrices with entries
  bounded by $1$.
  Then all
  the entries of $M_o=M(0)=D_pW_p\cdots D_1W_1$ are bounded by $c$
  as well.
\end{lem}

\begin{proof}
  Each entry of $D_iW_i$ is bounded by $c$
  and each entry of $(D_2W_2)(D_1W_1)$ is bounded by
  $nc^2=(nc)c\leq c$. Iterating the argument establishes
  the second claim.
\hfill$\Box$ \end{proof}

Recall that $M(0)=M_o$ corresponds to a multi-layer $F=f_p\ldots f_1$
with arbitrary non-linearities.
Let us add a skip-residual link by choosing $\PertVar=1$ in \equ{training_multi_layer} 

\begin{lem}
  \label{lem:increase_singval_hard_bound}
  Let $W_i$ be as in Lemma~\ref{lem:product_hard_bound}
  and recall \equ{training_multi_layer}.
  Assume that $c<1/n$.
  Then
  \begin{equation}
  \label{EQU:increase_singval_hard_bound}
    0
    <
    1-cn
    \leq
    \singval_n(M(1))
    \leq
    \singval_1(M(1))
    \leq
    1+cn
    <
    2
  \end{equation}
  and
  \begin{equation}
  \label{EQU:conditioning_hard_bound}
    \CondNb(M(1))
    \leq
    \frac{1+cn}{1-cn}
    .
  \end{equation}
\end{lem}

\begin{proof}
To establish (\ref{EQU:increase_singval_hard_bound}) apply
lemma~\ref{lem:Weyl_bound} with $i=1$ and $i=n$ and 
$\PertVar=1$, and note
that $\singval_1(M_o)\leq cn$ by Lemmata~\ref{lem:op_norm_hard_bound} and~\ref{lem:product_hard_bound}.
\MoreDetails{
    Alternatively, apply
    (\ref{EQU:uniform_bound}) with ${\AnyM}=M(1)$ and ${\AnyMt}={\rm Id}$.
    Note that $\singval_i({\AnyMt})=1$ and ${\AnyM}-{\AnyMt}=M(1)-{\rm Id}=M(0)$ which yields
    $\singval_i({\AnyM})-\singval_i({\AnyMt})=\singval_i(M(1))-1\leq\|{\AnyM}-{\AnyMt}\|_2
    =\singval_1(M(0))$.
}
The bound (\ref{EQU:conditioning_hard_bound}) follows immediately.
\hfill$\Box$ \end{proof}

Proposition~\ref{prop:absolute_value} implies the following bound for non-linearities of the type ``absolute value.''

\begin{thm}[Hard Bound, Absolute Value]
  \label{thm:increase_singval_hard_bound}
    Under the assumptions of 
    Lemma~\ref{lem:increase_singval_hard_bound}
    and for 
    $D\in\mathcal{D}(m,n,-1)$
    we have
    \begin{equation}\label{EQU:hard_abs}
%%%@        \CondNb((M(1))D^{(\sboldk)}(-1))
        \CondNb(M(1)D)
        \leq
        \frac{1+cn}{1-cn}.
    \end{equation}
\end{thm}


For a residual multi-layer \equ{training_multi_layer}
with ReLU non-linearities we find:


\begin{thm}[Hard Bound, ReLU]
  \label{thm:conditioning_ReLU_hard_bound}
    Under the assumptions of 
    Lemma~\ref{lem:increase_singval_hard_bound}
    and for 
    $D\in\mathcal{D}(m,n,0)$ the following statements hold:
  
  Provided $2cn<1/(1+n)$,
  we have
  \begin{equation}
  \label{EQU:conditioning_ReLU_hard_bound}
    \CondNb(M(1)D)
    \leq
    \frac{1+cn}{\sqrt{1-2cn(1+n)}}
  \end{equation}
  Provided $m\leq n(1-cn)^2$, we have
  \begin{equation}
  \label{EQU:conditioning_ReLU_hard_bound_small_m}
    \CondNb(M(1)D)
    \leq
    \frac{1+cn}{1-cn-\sqrt{m/n}}
    .
  \end{equation}
  Provided $2cn<1/(1+2m)$,
  we have
  \begin{equation}
  \label{EQU:conditioning_ReLU_hard_bound_alt}
    \CondNb(M(1)D)
    \leq
    \frac{1+cn}{\sqrt{1-2cn(1 +2m)}}
    .
  \end{equation}

\end{thm}



\begin{proof}
Applying Prop.~\ref{prop:ReLU_multiple_output} with $\PertVar=1$, i.e. $M=M(1)$ we have by
(\ref{EQU:ReLU_multiple_trace_output}) that
$$
    \sum_{i=1}^{n}
        |\singval_i^2 - \tilde\singval_i^2 |
%    =
%    \|M\|_2^2-\|\tilde M\|_2^2
    =
    \|M(1)- M(1)D\|_2^2
    \leq
    m\cdot (c^2n+2c+1)
    .
$$
Note that this bound
cannot be made arbitrarily small
by choosing $c$ small and
that it amounts to at least $m$.
However, the bulk of the sum of deviations
stems from some $m$ singular values of $M$
being changed to zero by $D$,
compensating the constant term $m$ in the above bound.
More precisely,
$\singval_i\geq 1-cn$ by (\ref{EQU:increase_singval_hard_bound})
for all $i$
while
$\tilde\singval_i=0$ for $i=n-m+1,\ldots, n$.
Thus,
$$
    \sum_{i=n-m+1}^{n}
        |\singval_i^2 - \tilde\singval_i^2 |
    =
    \sum_{i=n-m+1}^{n}
        \singval_i^2
    \geq
    m\cdot (1-cn)^2
    ,
$$
implying for any $1\leq j \leq n-m$
$$
    |\singval_j^2 - \tilde\singval_j^2 |
    \leq
    \sum_{i=1}^{n-m}
        |\singval_i^2 - \tilde\singval_i^2 |
    \leq
    m\cdot (c^2n+2c+1)
    -
    m\cdot (1-cn)^2
%    =
%    mc(cn+2+2n-cn^2)
%%    =
%%    mc(2+n(2+c-cn))
    \leq
    2mc(1+n)
    ,
$$
(using $cn-cn^2<0$).
Therefore,
$$
    \tilde\singval_j^2
    \geq
    \singval_j^2 - 2mc(1+n)
    \geq
    (1-cn)^2 - 2mc(1+n)
    =
    1-c(2n+ 2m(1+n)-cn^2)
%    \geq
%    1-c(2n^2 + 2n)
    \geq
    1-2c(n^2+n)
    .
$$
(using $m(1+n) \leq n^2-1\leq n^2$).
As this bound holds for all non-zero singular values of $\tilde M$,
we get
$$
    \tilde\singval_*
    \geq
    \sqrt{1-2c(n^2+n)}
%    \geq
%    {1-2c(n^2+n)}
    .
$$
%
Finally, we have $\tilde\singval_1\leq\singval_1\leq 1+cn$
by Lemma~\ref{lem:ReLU_decrease} and (\ref{EQU:increase_singval_hard_bound}).
This proves (\ref{EQU:conditioning_ReLU_hard_bound}).
%
Alternatively, we may estimate as follows:
$$
    \tilde\singval_j^2
    \geq
    1-c(2n+ 2m(1+n)-cn^2)
    \geq
    1-cn(2 +2m(1+1/n)-cn)
    \geq
    1-2cn(1 +2m)
$$
using $1/n\leq 1$ which proves \equ{conditioning_ReLU_hard_bound_alt}
%
At last, we may use \equ{ReLU_multiple_singval_output}
instead of (\ref{EQU:ReLU_multiple_trace_output}). Similar as before we find
$$
    \sum_{i=1}^{n}
        |\singval_i - \tilde\singval_i |^2
    \leq
    \|M(1)-M(1)D\|_2^2
    \leq
    m\cdot (c^2n+2c+1),
$$
implying for any $1\leq j \leq n-m$ that
$
    |\singval_j - \tilde\singval_j |^2
    \leq
    2mc(1+n)
    .
$
Therefore, provided $2cn<1/(1+n)$, or  $2c(1+n)<1/n$, we get
\equ{conditioning_ReLU_hard_bound_small_m} by observing
$$
    \tilde\singval_j
    \geq
    \singval_j - \sqrt{2mc(1+n)}
    \geq
    (1-cn) - \sqrt{2mc(1+n)}
    \geq
    1-cn -\sqrt{m/n}
    .
$$
\hfill$\Box$ \end{proof}

For leaky-ReLU the situation is more intricate.

\begin{thm}[Hard Bound, Leaky-ReLU]
  \label{thm:conditioning_Leaky_ReLU_hard_bound}
  Let $W_i$ be as in Lemma~\ref{lem:product_hard_bound}
  and recall \equ{training_multi_layer}.
  Assume that $c<1/n$.
  Let $D\in\mathcal{D}(m,n,\eta)$ with $0\leq \eta\leq1$.
%%%@  Let $D=D^{(\sboldk)}(0)$
  %which  corresponds to a
  %nonlinearity of the type ReLU
%%%@  with $\boldk=(k_1\ldots k_m)$ and $0\leq m\leq n-1$.
  Provided $n\geq5$ and $\eta<1$ large enough to ensure
    $(1-cn)^2
        >
    4(1-\eta)\sqrt{m}
    $
  we have
  \begin{equation}
  \label{EQU:conditioning_Leaky_ReLU_hard_bound}
    \CondNb(M(1)D)
    \leq
    \frac{1+cn}{
        \sqrt{
        (1-cn)^2
        -
        4(1-\eta)\sqrt{m}
        }}.
  \end{equation}
  Alternatively, if $\eta<1$ is such that
  $1-cn>(1-\eta)m(3c+1)$
  we have
  \begin{equation}
  \label{EQU:conditioning_Leaky_ReLU_hard_bound_alt}
    \CondNb(M(1)D)
    \leq
    \frac{1+cn}{{1-cn-(1-\eta)m(3c+1)}}
    .
  \end{equation}

\end{thm}

This situation corresponds to a ResNet \equ{training_multi_layer}
with leaky-ReLU non-linearities.


\begin{proof}
  We would like to proceed along the lines of the arguments of
  Theorem~\ref{thm:conditioning_ReLU_hard_bound}.
  To this end, we need to generalize the results of
  Proposition~\ref{prop:ReLU_multiple_output}.

  In order to replace \equ{ReLU_multiple_trace_output} we
  write for short 
  $M=M(1)=M_o+$Id with singular values $\singval_i$
  and $\tilde M=M(1)D$ 
  with singular values $\tilde\singval_i$.
  Apply Proposition~\ref{prop:Frobenius_bound} with
  ${\AnyM}=M^TM$ and ${\AnyMt}= \tilde M^T\tilde M=
  (MD)^TMD=D{\AnyM}D$ to get
  $$
  \sum_{i=1}^n
  |\singval_i^2-\tilde\singval_i^2 |^2
  \leq
          \|{\AnyM}-{\AnyMt}\|_2^2
  .
  $$
  Since all entries of $M_o$ are bounded by $c$ due to
  Lemma~\ref{lem:product_hard_bound} and using $cn<1$
   it follows
  that the entries of ${\AnyM}$ are bounded as
  follows
  $$
    |{\AnyM}[ij]|
    \leq
    \twocases{
        (n-2)c^2+2(1+c)c\leq3c}{if $i\neq j$}{
        (n-1)c^2+(1+c)^2\leq3c+1~~~}{if $i= j$
        .}
  $$
  Using these bounds, 
  direct computation shows that
  $
      {\AnyM}-{\AnyMt}={\AnyM}-D{\AnyM}D
  $ contains $2m(n-m)$ terms off the diagonal bounded by $3c(1-\eta)$,
  $m$ terms in the diagonal bounded by $(3c+1)(1-\eta^2)$,
  further $m^2-m$ terms off the diagonal bounded by $3c(1-\eta^2)$,
  and the remaining $(n-m)^2$ terms equal to zero.
  Using $cn<1$ whenever apparent
  as well as $(1-\eta^2)\leq 2(1-\eta)$ we may estimate as follows:
  \begin{eqnarray*}
    \|{\AnyM}-{\AnyMt}\|_2^2
    &\leq&
    (1-\eta)^2 18c^2 m(n-m)
        +
    (1-\eta^2)^2\left(
                9c^2 (m^2-m)+(3c+1)^2 m
                \right)
    \\
    &\leq&
    (1-\eta)^2
        18c^2 m(n-m)
        +
    4(1-\eta)^2\left(
                9c^2 m^2+6cm+ m
                \right)
    \\
    &\leq&
    (1-\eta)^2(42cm+18c^2m^2+4m)
    \leq
    4(1-\eta)^2m(15/n+1)
    .
  \end{eqnarray*}
  We conclude that
  for $n\geq5$ we have
  $|\singval_j^2-\tilde\singval_j^2 |\leq (1-\eta)4\sqrt{m}$.
  Together with $\singval_j\geq (1-cn)$
  we obtain
   \equ{conditioning_Leaky_ReLU_hard_bound}.
\if 0
  $$
    \tilde{\singval}_j^2
    \geq
    \singval_j^2
        -
    4(1-\eta)\sqrt m
    \geq
    (1-cn)^2
        -
    4(1-\eta)\sqrt{m}
  $$
\fi

Alternatively, we may strive at adapting
\equ{ReLU_multiple_singval_output} (which is based on
Corollary~\ref{cor:Frobenius_bound})
for $\eta\neq0$.
Recomputing
\equ{ReLU_multiple_singval_output} using
\equ{strong_frobenius_bound}
with ${\AnyM}=M$ and ${\AnyMt}=\tilde M$  for non-zero $\eta$
we get
$$    \sum_{i=1}^n
    |\singval_i-\tilde\singval_i|^2
    \leq
        \|M-\tilde M\|_2^2
    \leq
%%%@
%    (1-\eta)^2
%    \sum_{i=1}^m
%    \sum_{j=1}^{n} M[j k_i]^2
%    \leq
    (1-\eta)^2
    m(c^2n+2c+1).
$$
We obtain
$|\singval_j-\tilde\singval_j |
\leq (1-\eta)\sqrt{m(c^2n+2c+1)}
\leq (1-\eta)\sqrt{m(3c+1)}
$
and \equ{conditioning_Leaky_ReLU_hard_bound_alt}.
\hfill$\Box$ \end{proof}


We mention that the earlier Theorem~\ref{thm:chi_bounds}
will not lead to strong results in this context.
As we will see it will prove effective 
 effective in the random setting of the
next section.

\if 0
% not needed, just some comment
In fact, thm.~\ref{thm:lambda_bounds} will result in a
bound that is slightly less tight.
Indeed, for $M_o$ as in Lemma~\ref{lem:op_norm_hard_bound}
we would get
  \begin{equation}\label{EQU:tau_hard_bound}
    -2cn
    \leq
    \underline\tau
    \leq
    \overline{\tau}
    \leq
    2cn
  \end{equation}
  leading to slightly weaker bounds, and hinging on the
  technical assumption of piecewise simple eigenvalues.
%  with equality, e.g., for the matrix $M_o$ with all entries equal to $c$.

  While the upper bound is obvious,
  recall that $\eigval_i(-A)=-\eigval_i(A)$
  and the lower bound follows by symmetry.
\fi



\if 0
%  comment that without restriction on the entries, there is no general guarantee.

    For a ReLU nonlinearity, no guarantees on the improvement
    of condition number for all singular values
    can be given under such general assumptions.
    Indeed, as a special case consider a diagonal matrix $M_o$ with
    singular values equal to the absolute values to its diagonal
    elements, thus, $\singval_i=|M_o[ii]|<c$ (un-ordered).
    Adding identity will change the singular values to
    $|M_o[ii]+1|\geq 1-c$  (un-ordered).
    With $c$ being small, this amounts to
    a substantial increase and improvement of condition number.
    However, a ReLU active on line $k$ will set the corresponding
    singular value to $0$ with catastrophic consequences for condition number.
\fi



\subsection{Bounds with high probability for random matrices}
\label{sec:probabilities}

While the results of the last section provide absolute guarantees,
they are quite restrictive on the matrix $M_o$ since they cover the worst cases.
%
Working with the average behavior of a randomly initialized matrix $M_o$
allows the relax the restrictions.

\if 0
        We set up some notation for the case
        where the matrix $M_o$
        is initialized with zero-mean
        iid random variables.
        It is easy to extend our results to non-zero mean.
        It is well known that a random  variable $X$
        with zero mean $\mu=\expect[X]=0$ has variance
        equal to its second moment:
        \begin{eqnarray*}
        \nonumber
        %  \mu &=& \expect[X]
        %    \quad\mbox{(mean)}\\
        %  \mu_2 &=& \expect[X^2]
        %    \quad\mbox{(second moment)}\\
           \Var = \var(X) = \expect[X^2]
           %=\mu_2-\mu^2
        %    \quad\mbox{(variance)}\\
        %  \mu_4 &=& \expect[X^4]
        %    \quad\mbox{(forth moment)}\\
        \end{eqnarray*}
        \if 0
                which we extend as follows:
                \begin{eqnarray}
                  \mu(\PertVar) &=& \expect[X+\PertVar]
                    \quad\mbox{(mean)}\\
                  \mu_2(\PertVar) &=& \expect[(X+\PertVar)^2] = \mu_2+2\PertVar\mu+\PertVar^2
                    \quad\mbox{(second moment)}\\
                  \var(\PertVar) &=& \var(X+\PertVar) = \Var
                    \quad\mbox{(variance)}\\
                  \mu_4(\PertVar) &=& \expect[(X+\PertVar)^4]
                    \quad\mbox{(forth moment)}\\
                \end{eqnarray}
        \fi
        It is customary to denote the Gaussian case by $X\simeq\mathcal{N}(\mu,\Var)$.

        For a uniform $X\simeq U[-c,c]$
        the hard bounds of the last section
        such as Lemma~\ref{lem:op_norm_hard_bound}
        and Theorem~\ref{thm:conditioning_ReLU_hard_bound}
        apply since all entries must lie in $[-c,c]$.
\fi

The strongest results in this context concern the operator norm
and exploit cancellations in the entries of $M_o$
(see \cite[Proposition 3.1]{BAL}, \cite{Tracy_Widom,Tracy_Widom2}).
\if 0
    \begin{prop}[Benhamou-Atif-Laraki]
    \label{prop:Benhamou-Atif-Laraki}
      Let $M$ be a squared matrix with iid sub-Gaussian entries (such as Bernoulli, Uniform, Gaussian)
      of $\var=1$.
      Then there exist non-negative real constants $C,c >0$
      such that for all $A\geq C$ we have
      \begin{equation}\label{EQU:BAL_operator_bound}
        P[\|M\|_{\rm Op}>A\sqrt n]
        \leq
        C\exp(-cAn)
      \end{equation}
    \end{prop}
\fi
Most useful for this study is the well-known
result due to Tracy and Widom \cite{Tracy_Widom,Tracy_Widom2}.
Translated into our setting, it reads as follows.



\if 0

Info online:

https://terrytao.wordpress.com/2010/01/09/254a-notes-3-the-operator-norm-of-a-random-matrix/

Symmetric Wigner matrix ensembles, in which the upper triangular coefficients {\xi_{ij}}, {j \geq i} are jointly independent and real, but the lower triangular coefficients {\xi_{ij}}, {j<i} are constrained to equal their transposes: {\xi_{ij}=\xi_{ji}}. Thus {M} by construction is always a real symmetric matrix. Typically, the strictly upper triangular coefficients will be iid, as will the diagonal coefficients, but the two classes of coefficients may have a different distribution.

An {n \times n} matrix consisting entirely of {1}s has an operator norm of exactly {n}, as can for instance be seen from the Cauchy-Schwarz inequality. More generally, any matrix whose entries are all uniformly {O(1)} will have an operator norm of {O(n)} (which can again be seen from Cauchy-Schwarz, or alternatively from Schurs test, or from a computation of the Frobenius norm). However, this argument does not take advantage of possible cancellations in {M}. Indeed, from analogy with concentration of measure, when the entries of the matrix {M} are independent, bounded and have mean zero, we expect the operator norm to be of size {O(\sqrt{n})} rather than {O(n)}. We shall see shortly that this intuition is indeed correct. (One can see, though, that the mean zero hypothesis is important; from the triangle inequality we see that if we add the all-ones matrix (for instance) to a random matrix with mean zero, to obtain a random matrix whose coefficients all have mean {1}, then at least one of the two random matrices necessarily has operator norm at least {n/2}.)

The most advanced knowledge we have on the operator norm is given by the Tracy-Widom law, which not only tells us where the operator norm is concentrated in (it turns out, for instance, that for a Wigner matrix (with some additional technical assumptions), it is concentrated in the range {[2\sqrt{n} - O(n^{-1/6}), 2\sqrt{n} + O(n^{-1/6})]}), but what its distribution in that range is.

Theorem 37 (Strong Bai-Yin theorem, upper bound)
    Let {\xi} be a real random variable with mean zero, variance {1}, and finite fourth moment, and for all {1 \leq i \leq j}, let {\xi_{ij}} be an iid sequence with distribution {\xi}, and set {\xi_{ji} := \xi_{ij}}. Let {M_n := (\xi_{ij})_{1 \leq i,j \leq n}} be the random matrix formed by the top left {n \times n} block.

    Then almost surely one has {\limsup_{n \stackrel{\rm distr}{\rightarrow} \infty} \|M_n\|_{op}/\sqrt{n} \leq 2}.

By using these methods, it is in fact possible to show that under various hypotheses, {\|M\|_{op}} is concentrated in the range {[2\sqrt{n}-O(n^{-1/6}), 2\sqrt{n}+O(n^{-1/6})]}, and even to get a universal distribution for the normalised expression {(\|M\|_{op}-2\sqrt{n}) n^{1/6}}, known as the Tracy-Widom law. See this paper of Soshnikov for details. There has also been a number of subsequent variants and refinements of this result (as well as counterexamples when not enough moment hypotheses are assumed); see for instance these papers of Soshnikov, Soshnikov-Fyodorov, Ruzmaikina, Péché, Vu, Soshnikov-Péché, Péché, Khorunzhiy and Tao-Vu for an (incomplete) sample of the work in this area. (Similar results for some non-independent distributions are also available, see e.g. this paper of Deift and Gioev, which (like many of the other references just cited) builds upon the original work of Tracy and Widom that handled special ensembles such as GOE and GUE.)


not publically available:

Soshnikov, A. Universality at the Edge of the Spectrum¶in Wigner Random Matrices. Comm Math Phys 207, 697733 (1999). https://doi.org/10.1007/s002200050743


out of Benhamou p2 top

Other impor-
tant contribution have been the Tracy Widom law, which says that for Wigner
matrix, the operator norm is concentrated in the range of

2 sqrt n - O (n^-1/6)
2 sqrt n + O (n^-1/6)
(see Tracy and Widom (1994)),





\fi


\if 0
 the Tracy-Widom law, which says that for Wignermatrix,
 the operator norm is concentrated in the range of
 $[2 \sqrt n - O(n^{-1/6}),2 \sqrt n + O(n^{-1/6})]$
 (see  Tracy  and  Widom  (1994),
\fi


\begin{thm}[Tracy-Widom]
  \label{thm:op_norm_edge_bound}
    Let $X_{ij}$ ($1\leq i,j$) be an infinite family of
    iid copies of a random variable $X$
    which is Gaussian or Uniform, has zero mean  and variance $1$.
    %%%$\Std^2$.
    Let $K_n$ be a sequence of $n\times n$ matrices with entries
    $K_n[i,j]=X_{i,j}$ ($1\leq i,j\leq n$).


    Let $\overline{t_n}$ denote the largest eigenvalue of
    $K_n^T+K_n$ and let $\underline{t_n}$ denote its smallest.

  Then, as $n\to\infty$, both $\overline{t_n}$ and $-\underline{t_n}$
  lie  with high probability in the interval
  \begin{equation}\label{EQU:tau_edge_bounds}
    %%%\Std\cdot
    [ \sqrt{8n}- O(n^{-1/6}),\sqrt{8n}+O(n^{-1/6})]
    .
  \end{equation}
  
  More precisely, the distributions of
\begin{eqnarray}
    \label{EQU:TAU_edge_bound_sharper}
   Z_n
   &:=&
   (\overline{t_n}%%%/\Std
        -\sqrt{8n})\cdot n^{1/6}
   \\
    \label{EQU:tau_edge_bound_sharper}
   \tilde Z_n
   &:=&
   (-\underline{t_n}%%%/\Std
        -\sqrt{8n})\cdot n^{1/6}
\end{eqnarray}
   converge both (individually) to a Tracy-Widom law $P_{TW}$. 
   The Tracy-Widom law is well concentrated
   at values close to $0$.
\end{thm}

The random variables $Z_n$ and $\tilde Z_n$
are equal in distribution due to the
symmetry of the random variable~$X$. However,
they are not independent.


It is easy to verify that the theory of Wigner matrices and the
law of Tracy-Widom apply, and to establish the theorem.
In particular, $K_n^T+K_n$ is symmetric with iid\ entries above the diagonal
and iid\ entries in the diagonal, all with finite non-zero second moment.
The normalization of $\overline{t_n}$ leading to $Z_n$ (see \equ{TAU_edge_bound_sharper}) is quite
sharp, meaning that the distributions of $Z_n$ are close to their limit starting at
values as low as $n=5$ (see Figure~\ref{fig:tracy-widom}).

The Tracy-Widom distributions
are well studied and documented, with a right tail that
decays exponentially fast \cite{TW_Tail}.
Moreover, they are well concentrated at values close to $0$.
Combined with the fast convergence this implies that $\overline{t_n}$ is close to
$\Std \sqrt{8n}$ with high probability even for modest $n$.

A related useful result reads as follows
(see \cite[Thm.~2,6]{Chafai} and refs.~there)
\begin{thm}
  \label{thm:Op_norm_Gauss}
  Let $K_n$ be as in theorem~\ref{thm:op_norm_edge_bound}, but Gaussian. Then, as $n\to\infty$
  \begin{equation}
      \label{EQU:Op_norm_Gauss_limit}
      \frac {\singval_1(K_n)}{\sqrt{n}}
    \stackrel{\rm a.s.}{\rightarrow}
      2 
  \end{equation}
  Moreover, letting $\mu_n=(\sqrt{n-1}+\sqrt{n})^2$
  and $q_n=\sqrt{\mu_n}(1/\sqrt{n-1}+1/\sqrt{n})^{1/3}$, 
  the distribution of 
\begin{equation}
      \label{EQU:Yn_def}
      Y_n
      :=
      ({\singval_1(K_n)^2-\mu_n})/{q_n}
  \end{equation}
    converges narrowly to a Tracy-Widom law.
\end{thm}
Comparing with theorem~\ref{thm:op_norm_edge_bound}
we should expect $\singval_1(K_n)\simeq 2\sqrt{n}\simeq \overline t_n/\sqrt{2}$
(compare figure~\ref{fig:Yn_convergence}).

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{./figures/Tracy_Widom_50k_Gauss.jpg}
    \includegraphics[width=0.45\linewidth]{./figures/Tracy_Widom_50k_Uniform.jpg}
    \caption{
    Empirical demonstration of the Tracy-Widom law.
    Note the collapsing histograms of
    $Z_n=(\overline{t_n}%%%/\Std
    -\sqrt{8n})\cdot n^{1/6}$
    for $n=5, 10, 25, 50, 100$
    where $\overline{t_n}$ denotes the largest eigenvalue of the
    $n\times n$ matrix of the form $K_n+K_n^T$ 
    and where the entries of $K_n$ are drawn from
    a Gaussian (left) or uniform (right) distribution with zero mean and
    variance $1$.
    %%%$\Std^2$.
    Note that the right-side tails $P[Z_n>x]$ decay very quickly,
    leading to negligible probabilities at moderate values of $x$.}
    \label{fig:tracy-widom}
\end{figure}



\if 0

Paper on TAIL  unknown o(1)
*************


    The right tail exponent of the Tracy-Widom \beta distribution
    Dumaz, Laure ; Virág, Bálint
    Annales de l'I.H.P. Probabilités et statistiques, Tome 49 (2013) no. 4, pp. 915-933.

P[TW_\beta > r) = a^{-3/4 \beta+ o(1)} \exp (-2/3  \beta a^3/2)



MATLAB on TAIL
*************

GAUSS
    using 50'000 matrices $M+M^T$ 	of sizes [5 10 25 50 100]

    99 Percentiles of empir. Tracy Widom
    meaning the $r$ value with $P_{TW}(Z\leq r]=99\%$

    r   2.3092    2.4009    2.5417    2.6248    2.6906

    99.9 Percentiles of empir. Tracy Widom
        3.8686    4.1165    4.2776    4.2793    4.4687


    compare quantiles to threshold for TAU<2*target (instead of TAU=target) target =\Std \sqrt{8n}
        8.2704   13.1284   24.1827   38.3877   60.9366

    compare quantiles to threshold for TAU<1.1*target (instead of TAU=target)
        0.8270    1.3128    2.4183    3.8388    6.0937

    compare quantiles to threshold for TAU<1.25*target (instead of TAU=target)
        2.0676    3.2821    6.0457    9.5969   15.2342



    proba of TAU<= 2 sigma sqrt(8n)
         1     1     1     1     1
    compare with formula via P[ Z<= sqrt(8)*n^(2/3) ]
         1     1     1     1     1

    proba of TAU<= 1.1 sigma sqrt(8n)
        0.9456    0.9662    0.9885    0.9983    0.9999
    compare with formula via P[ Z<= 0.1*sqrt(8)*n^(2/3) ]
        0.9456    0.9662    0.9885    0.9983    0.9999

    proba of TAU<= 1.25 sigma sqrt(8n)
        0.9867    0.9968    0.9999    1.0000    1.0000
    compare with formula via P[ Z<= 0.25*sqrt(8)*n^(2/3) ]
        0.9867    0.9968    0.9999    1.0000    1.0000



    $Z_n\leq s\sqrt{8} n^{2/3}$ means $\overline{t\leq (1+s) \Std\sqrt{8n}}$


UNIFORM

statistics for all simulated sizes of matrix from 50000 samples
sizes of matrix
     5    10    25    50   100

99 Percentiles of empir. Tracy Widom
    1.4445    1.7170    2.0741    2.3009    2.4424

99.9 Percentiles of empir. Tracy Widom
    2.7010    3.0667    3.6704    3.9584    4.0884

compare quantiles to threshold for TAU<2*target (instead of TAU=target)
    8.2704   13.1284   24.1827   38.3877   60.9366

compare quantiles to threshold for TAU<1.1*target (instead of TAU=target)
    0.8270    1.3128    2.4183    3.8388    6.0937

compare quantiles to threshold for TAU<1.25*target (instead of TAU=target)
    2.0676    3.2821    6.0457    9.5969   15.2342

proba of TAU<= 2 sigma sqrt(8n)
     1     1     1     1     1

compare with formula via P[ Z<= sqrt(8)*n^(2/3) ]
     1     1     1     1     1

proba of TAU<= 1.1 sigma sqrt(8n)
    0.9726    0.9819    0.9934    0.9988    1.0000

compare with formula via P[ Z<= 0.1*sqrt(8)*n^(2/3) ]
    0.9726    0.9819    0.9934    0.9988    1.0000

proba of TAU<= 1.25 sigma sqrt(8n)
    0.9963    0.9993    1.0000    1.0000    1.0000

compare with formula via P[ Z<= 0.25*sqrt(8)*n^(2/3) ]
    0.9963    0.9993    1.0000    1.0000    1.0000


Lecture notes on TAIL ... unknown c
*************

    % from Kemp_247A_Notes p 27
    $$
        P[
        \overline{t_n}
        >
        (2+\delta n^{-1/6+\eps})\Std\sqrt{2n}
        ]
        \leq
        2n\left(
        1+\frac \delta 2 n^{-1/6+\eps}
            \right)^{-2cn^{1/6}}
        \simeq
        2n\exp(-c\delta n^\eps)
    $$
    for some $c>0$.

    choose $\delta n^\eps=n^{1/12}$
\fi

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{./figures/Histo_Yn_Gauss_50k_r2_kap1.jpg}
    \includegraphics[width=0.45\linewidth]{./figures/Histo_Tau_by_sq2s1_Gauss_50k_r3_kap1.jpg}
    %\includegraphics[width=0.45\linewidth]{./figures/Histo_Yn_Gauss_50k_r3_kap1.jpg}
    \caption{
    Left: Empirical demonstration of the convergence of $Y_n$
    \equ{Yn_def},
to a Tracy-Widom law.
Note that the right-side tails $P[Y_n>x]$ decay very quickly,
    leading to negligible probabilities at moderate values of $x$ and for $n$
    as small as $5$
    similar to $Z_n$ from figure~\ref{fig:tracy-widom}.
    \\
    Right: Empirical demonstration of the convergence of $\overline{\tau}/(\sqrt{2}\singval_1)$
    to $1$: the ratio lies indeed with high probability between $0.8$ and $1.2$ for 
    $n$ as small as $10$.}
    \label{fig:Yn_convergence}
\end{figure}



Combining
%Proposition~\ref{prop:max_value} as well as
Theorem~\ref{thm:chi_bounds} (with $M_0=W_1$)
%, i.e., $D_1=$Id), 
and Theorem~\ref{thm:op_norm_edge_bound},
and using (for $n\geq2$) that
$\mu_n\leq 4n$ and
$q_n
\leq 
\sqrt{(4n)}2^{1/3}(n-1)^{-1/6}
\leq 
\sqrt{(4n)}2^{1/3}(n/2)^{-1/6}
\leq 
2^{3/2}n^{1/3}
$,
we get:

\begin{lem}[High Probability Bound]
  \label{lem:Abs_Value_average_bound}
  In the notation of Theorem~\ref{thm:op_norm_edge_bound}
  let $r>1$ and $n\geq 2$, set
  \begin{equation}
  \label{EQU:Sigma_n_Abs_Value}
    \Std_n
    =
    \frac{1}{r\cdot \sqrt{8n}}
  \end{equation}
  and let
  $
    W_1 %M_n
    =
    \Std_n K_n
    .
    $
  Denote the largest and smallest eigenvalues of $W_1^T+W_1$ % M_n^T+M_n$
  by $\overline{\tau}_n=\overline{\tau}_n(r)$ and $\underline{\tau}_n=\underline{\tau}_n(r)$
  (compare with \equ{OpNorm_MT+M}).
  \\
  (1) We have
  \begin{eqnarray}
  \label{EQU:TAU=renormZn}
    % proof:
    % \overline{\tau} &=& \Std_n\cdot t_n =  \Std_n\cdot (\sqrt{8n}+Z_n n^{-1/6}\\
    \overline{\tau}_n(r) 
    &=& \frac 1 r \cdot (1 +
            Z_n \frac {1}{\sqrt{8}\cdot n^{2/3}})
    \qquad
    -\underline{\tau}_n(r)
    = \frac 1 r \cdot (1 +
        \tilde   Z_n \frac {1}{\sqrt{8}\cdot n^{2/3}})
  \end{eqnarray}
  and
  $$
    P[\underline{\tau}_n(r)>-1]
    =
    P[\tilde Z_n\leq (r-1)\sqrt{8} n^{2/3}]
    .
  $$
  (2) We have 
  $
    \singval_1(W_1)
    {\rightarrow}
%    \stackrel{\rm a.s.}{\rightarrow}
    1/(\sqrt{2}r)
$
with probability $1$, i.e. almost surely, 
and
  \begin{equation}
      \label{EQU:renorm_s1(W1)}
      \singval_1(W_1)^2
      =
      \frac{1}{2r^2}
      \left( 
      \frac{\mu_n}{4n}
      +
      n^{-2/3}\frac{q_n}{4n^{1/3}}
      Y_n
      \right)
      \leq
      \frac{1}{2r^2}
      \left( 
      1
      +
      n^{-2/3}\frac{1}{\sqrt{2}}
      Y_n
      \right)
  \end{equation}

  (3)
  For any realization of $W_1$
  for which 
  $\singval_1(W_1)<1$ we have
  \begin{equation}
  \label{EQU:conditioning_average_bound_via_s1}
    \CondNb(W_1+{\rm Id})
    \leq
    \frac{\sqrt{\singval_1^2(W_1)+\overline\tau_n+1
        }}{1-\singval_1(W_1)}
    \leq
    \frac{1+\singval_1(W_1)}{1-\singval_1(W_1)}
    .
  \end{equation}

  (4)
  For any realization of $W_1$
  for which 
  $\underline{\tau}_n>-1$ and for which 
  %the smallest singular value 
  $\singval_n(\PertVar)=
  \singval_n(W_1+\PertVar {\rm Id})$
  is piecewise simple in $[0,1]$ we have
  the slightly tighter bounds 
  \begin{equation}
  \label{EQU:increase_singval_average_bound}
    0
    <
    \singval_n^2(W_1)+\underline{\tau}_n+1
    %1-\Std\sqrt{8n}
    \leq
    \singval_n^2(W_1+{\rm Id})
    \leq
    \singval_1^2(W_1+{\rm Id})
    \leq
    \singval_1^2(W_1)+\overline{\tau}_n+1
%    \singval_n^2(M_n+{\rm Id})
%    \leq
%    \singval_1^2(M_n+{\rm Id})
%    \leq
%    \singval_1^2(M_n)+\overline{\tau}+1
%    %\Std\sqrt{8n}
%    \leq
%    (1+\singval_1(M_n))^2
    .
  \end{equation}
  and  the condition number of
  %$M_n+{\rm Id}$
  $W_1+{\rm Id}$
  is bounded as follows:
%\if 0
  \begin{equation}
  \label{EQU:conditioning_average_bound}
  \CondNb_n
  :=
    \CondNb(W_1+{\rm Id})
    \leq
    \sqrt{\frac{\singval_1^2(W_1)+\overline\tau_n+1
%%%        }{\singval_n^2(W_1)+\underline\tau_n+1}}
        }{\underline\tau_n+1}}
    \leq
    \frac{\singval_1(W_1)+1}{\sqrt{\underline\tau_n+1}}
    .
  \end{equation}
%\fi
\if 0
  \begin{equation}
  \label{EQU:conditioning_average_bound_kappa}
    \CondNb(W_1+\PertVar{\rm Id})
    \leq
    \sqrt{\frac{\singval_1^2(W_1)+\PertVar\overline\tau+\PertVar^2
            }{\singval_n^2(W_1)+\PertVar\underline\tau+\PertVar^2}}
    \leq
    \frac{\singval_1(W_1)+\PertVar}{\sqrt{\PertVar\underline\tau+\PertVar^2}}
    .
  \end{equation}
\fi
\end{lem}


\begin{figure}
    \centering
    \includegraphics[width=0.3\linewidth]{./figures/Histo_Ratio_LargeEigen_Gauss_50k_r2_kap1.jpg}
    \includegraphics[width=0.33\linewidth]{./figures/Histo_Ratio_SmallEigen_Gauss_50k_r2_kap1.jpg}
    \includegraphics[width=0.33\linewidth]{./figures/Histo_Ratio_Chi2_Gauss_50k_r2_kap1_fixed.jpg}
    \caption{
    Empirical demonstration of the efficiency of the bounds
    \equ{increase_singval_average_bound} and \equ{conditioning_average_bound}
    using $r=2$.
    The figures show histograms of the fractions
    $
    [\singval_n^2(W_1+{\rm Id})]/
    [\singval_n(0)+\underline{\tau}+1]
,
$
$
    [\singval_1^2(W_1)+\overline{\tau}+1]
    /
    [\singval_1^2(W_1+{\rm Id})]
$
and
$
    \sqrt{\frac{\singval_1^2(W_1)+\overline\tau_n+1
%%%        }{\singval_n^2(W_1)+\underline\tau_n+1}}
        }{\underline\tau_n+1}}
    /
        \CondNb(W_1+{\rm Id})
$
.
    Note that all values are above $1$ and actually quite close to $1$.}
    \label{fig:efficient_bounds}
\end{figure}

We make the statement (4) despite its hinging on the technical assumption of $\singval_n$ being piecewise simple because its
bounds are somewhat sharper than those in (2).

For a a single residual layer \equ{training_one_layer}
with weights $W_1$
and a ResNet with 
non-linearities of the type ``absolute value''
we get:

\begin{cor}[High Probability Bound, Absolute Value]
  \label{cor:Abs_Value_average_bound}
  Let $W_1$ be as in Lemma~\ref{lem:Abs_Value_average_bound}.
  Let $D,D_1\in\mathcal{D}(m,n,-1)$ for some fixed $m$.
  Set $M_o=D_1W_1$ and recall Definition~\ref{def:tau}.
\\
  (1)
  We have 
  $
    \singval_1(M_o)
    {\rightarrow}
%    \stackrel{\rm a.s.}{\rightarrow}
    1/(\sqrt{2}r)
$
with probability $1$.
  For any realization of $M_o$
  for which 
  $\singval_1(M_o)<1$ we have
  \begin{equation}
  \label{EQU:conditioning_average_bound_AbsValue_via_s1}
    \CondNb((M_o+{\rm Id})D)
    \leq
    \frac{\sqrt{\singval_1^2(M_o)+\overline\tau+1
        }}{1-\singval_1(M_o)}
    \leq
    \frac{1+\singval_1(M_o)}{1-\singval_1(M_o)}
    .
  \end{equation}
\\
    (2)
    For any realization of $W_1$
  for which 
  $\underline{\tau}>-1$ and for which 
  %the smallest singular value 
  $ \singval_n(M_o+\PertVar {\rm Id})$
  is piecewise simple for $\PertVar$ in $[0,1]$,
  the following bound holds
  \begin{equation}
  \label{EQU:conditioning_average_bound_AbsValue}
    \CondNb((M_o+{\rm Id})D)
    \leq
    \sqrt{\frac{\singval_1^2(M_o)+\overline\tau+1
%%%        }{\singval_n^2(M_o)+\underline\tau_n+1}}
        }{\underline\tau+1}}
    \leq
    \frac{\singval_1(M_o)+1}{\sqrt{\underline\tau+1}}
    .
  \end{equation}
\end{cor}

\begin{proof}
    Note that $M_0=D_1W_1$ is a random matrix with the same properties as $W_1$ itself, since $D_1$ is deterministic and changes only the sign of some of the entries of $W_1$. We may, therefore,
    apply Lemma~\ref{lem:Abs_Value_average_bound} to $M_o$ (replacing $W_1$). 
    % we get the bound on $\CondNb(D_1W_1+{\rm Id})$ in terms of $s_1(D_1W_1)$ and $\overline{\tau}(D_1W_1)$ etc.
    %Problem: $\overline{\tau}(D_1W_1)$ is the  largest eigenvalue of $(D_1W_1)^T(D_1W_1)=D_1(W_1^T+W_1)$ which may change...only its singvals remain unchanged, but the eigenvals may change!
    Also, $D$ does not alter the singular values:
    $\singval_i((M_o+{\rm Id})D)=\singval_i(M_o+{\rm Id})$.
    For the same reason we have $\singval_1(M_o)=\singval_1(W_1)$.
\hfill$\Box$
\end{proof}

{\bf Probabilities of exceptional events}
\begin{itemize}
  \item{Clarification regarding $\underline{\tau}$ vs. $\underline{\tau}_n$ in the setting of 
  Corollary~\ref{cor:Abs_Value_average_bound}} 
  
  While $\singval_1(M_o)=\singval_1(W_1)$, one should note that $\overline\tau$
  (largest eigenvalue of $M_o^T+M_o$)
  may differ from $\overline\tau_n$
  (largest eigenvalue of $W_1^T+W_1$)
  for any particular realization. 
  
  However, since $M_o$ and $W_1$ are equal in distribution due to the special form of $D_1$,
  we have that
  $\overline\tau$ and $\overline\tau_n$, as well as 
  $-\underline{\tau}$ and $-\underline{\tau}_n$
  are all equal in distribution with distribution well concentrated around $1/r$.


  \item{Exceptions 
  $
  E_{\singval_1(W_1)}
  =
  \{\singval_1(W_1)\geq 1\}$ and
  $
  E_{\singval_1(M_o)}
  =
  \{\singval_1(M_o)\geq 1\}$}:
  
  According to \equ{renorm_s1(W1)}, we have
 $       
    P[\singval_1(W_1)^2\geq 1]
      \leq
     P[
      Y_n
      \geq
      \sqrt{2}({2r^2}-1)
    n^{2/3}
    ]
$
which converges to $0$ since $Y_n$ converges to a Tracy-Widom law
and is small for $r\geq 2$ and modest $n$.
Similarly for the second event listed.
  
  \item{Exception 
  $
  E_{\underline{\tau}_n}
  =
  E_{\underline{\tau}_n(r)}
  =
  \{\underline{\tau}_n(r)
  \leq-1\}$}:
  
  We claim that
  $P[E_{\underline{\tau}_n}]\approx0$ 
  for values as small as
  $r\geq 2$ and $n\geq 5$. We are able to support this claim through computations as well as simulations:

  From Figure~\ref{fig:tracy-widom} it appears, that 
  $P[Z_n<8]=1$ for $n\geq 5 $
  for all practical purposes.
  On the other hand, for $r\geq2$ and 
  $n\geq 5$, we have $(r-1)\sqrt{8} n^{2/3}>8$
  and may estimate
  $P[\underline{\tau}_n>-1]
      =
    P[\tilde Z_n < (r-1)\sqrt{8} n^{2/3}]
    \geq
    P[\tilde Z_n < 8]
    =
    P[ Z_n < 8]
  $ 
  to be equal to $1$ for all practical purposes.
  This was confirmed by our simulations 
  in the following sense:
  Every single one of the 500,000 random matrices simulated
  with $r=2$ satisfied $\underline{\tau}_n>-1$.


  \item{Exception $E_{\rm{p.w.}}=\{\singval_n(\PertVar)
  \mbox{ is not piecewise simple}\}$}:
  
The smallest singular value 
$\singval_n(\PertVar)$ of
$W_1+\PertVar {\rm Id}$
%$M_n+\PertVar {\rm Id}$
is almost surely simple for all rational $\PertVar$ in $[0,1]$.
In other words, $S_n$ is a.s.~dense and open in $[0,1]$.
This does not imply, however, that $\singval_n(\PertVar)$ is  almost surely piecewise
simple since $[0,1]\setminus S_n$ could still be a fractal set of non-zero
measure.

However, we believe that such a fractal situation is the exception in our context
and that the mentioned assumption is purely technical and typically satisfied.
Confirming this point of view numerically, however, is an impossible task, due
to the nature of fractal sets.

\item{Exception $E_{\singval_n(W_1)}=\{
  \mbox{at least one of the inequalities of 
  \equ{increase_singval_average_bound} 
  %bounding the growth of singular values 
  fails}\}$}:

  We claim that
  $P[E_{\singval_n(W_1)}]\approx0$ for all 
  practical purposes. 
  
According to
Lemma~\ref{lem:Abs_Value_average_bound}
we have
$
    P[E_{\singval_n(W_1)}]
    \leq
    P[E_{\rm{p.w.}} \cup E_{\underline{\tau}_n}]
    \leq
    P[E_{\rm{p.w.}}]+P[E_{\underline{\tau}_n}]
.$
With reference to the points made above we should expect that this exceptional event is so unlikely that it will  not be observed in applications. 

Such an argument hinges, however, on the alluded ``fractal situation'' to not occur in our setting.
More convincing is a direct confirmation of 
\equ{increase_singval_average_bound} and \equ{conditioning_average_bound} by simulation.
Indeed, not only are the fractions of right side by left side of all relevant
inequalities in
\equ{increase_singval_average_bound} and \equ{conditioning_average_bound}
greater or equal to $1$ in \emph{all} our simulations,
they are actually surprisingly close to $1$.

In summary, for all practical purposes we have
$P[E_{\singval_n(W_1)}]\approx 0$.
Also, 
in \equ{increase_singval_average_bound} 
the first two inequalities are the only ones that may fail.

Moreover, the bounds
\equ{increase_singval_average_bound} and \equ{conditioning_average_bound}
are surprisingly efficient.
The first upper bound of \equ{conditioning_average_bound}, e.g.
amounts to only about $10\%$ larger than $\CondNb(W_1+{\rm Id})$ for large $n$
(see Figure~\ref{fig:efficient_bounds}).

We see an explanation for this efficiency of the bounds to be rooted
in the fact that the singular values of random matrices tend to be
as widely spread as possible, meaning that the largest singular values
grow as fast as possible, the smallest ones as slowly as possible.
While this maximal spreading is well known for symmetrical
random matrices called ``Wigner-matrices'', we are not aware of any
reports to this fact for non-symmetrical matrices such as $W_1$.




\end{itemize}




\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{./figures/Histo_Chi_Gauss_50k_r2_kap1.jpg}
    \includegraphics[width=0.45\linewidth]{./figures/Histo_Chi_Gauss_50k_r3_kap1.jpg}
    \caption{
    Empirical demonstration of the asymptotic bound \equ{conditioning_average_bound_asymptotics}.
    The figures show histograms of the $\CondNb(W_1+{\rm Id})$ for $r=2$ and $r=3$
    together with the upper bound in form of a deterministic expression 
    from \equ{conditioning_average_bound_asymptotics} in black.
    Note that the values of $\CondNb(W_1+{\rm Id})$ lie asymptotically below the deterministic expression as indicated in
    \equ{conditioning_average_bound_asymptotics}.}
    \label{fig:asymptotic_bounds}
\end{figure}

For design purposes, a deterministic expression bounding
 the condition number $\CondNb(W_1+{\rm Id})$
might be useful.

\begin{thm}[High Probability Bound in the limit]
  \label{thm:chi_asymptotics}
  With the notations and assumptions of Theorem~\ref{thm:op_norm_edge_bound}
  and Lemma~\ref{lem:Abs_Value_average_bound},
  the upper bounds given there
  converge in distribution to constants as follows:
  \begin{equation}
  \label{EQU:conditioning_average_bound_asymptotics}
    \sqrt{\frac{\singval_1^2(W_1)+\overline\tau_n+1
        }{\underline\tau_n+1}}
    \stackrel{\rm distr}{\rightarrow}
    \sqrt{
        \frac{r^2+r+1/2}{r^2-r}
    }.
  \end{equation}
  and
  \begin{equation}
  \label{EQU:conditioning_average_bound_asymptotics_via_s1}
    \frac{\sqrt{\singval_1^2(W_1)+\overline\tau_n+1
        }}{1-\singval_1(W_1)}
    \stackrel{\rm distr}{\rightarrow}
    \frac{\sqrt{r^2+r+1/2}}{r-1/\sqrt{2}}
    .
  \end{equation}
\end{thm}

For a demonstration of the deterministic expression bounding
the condition number as in 
\equ{conditioning_average_bound_asymptotics}, see
Figure~\ref{fig:asymptotic_bounds}.



\begin{proof}
  Since $Z_n$ converges in distribution to a real-valued random variable $Z$,
  %%%following a Tracy-Widom law $P_{TW}$
  we may conclude that $Z_n/n^{2/3}$ converges in distribution to $0$.
  Indeed, for any $\eps>0$ and any $n_o\geq 1$ we have for $n\geq n_o$ that
  $$
    P\left[|Z_n/n^{2/3}|\geq \eps\right]
    \leq
    P\left[|Z_n|\geq \eps n_o^{2/3}\right]
    \stackrel{n\to\infty}{\to}
%%%    P_{TW}[Z\geq \eps n_o^{2/3}]
    P\left[|Z|\geq \eps n_o^{2/3}\right]
    .
  $$
  From this we obtain for any $n_o\geq 1$ that
  $$
    \limsup_{n\to\infty} P\left[|Z_n/n^{2/3}|\geq \eps\right]
    \leq
    P_{TW}\left[|Z|\geq \eps n_o^{2/3}\right]
  $$
  and letting $n_o\to \infty$ we conclude that
  $
  P[|Z_n/n^{2/3}|\geq \eps]
  \to
  0
  .
  $

  This establishes that $Z_n/n^{2/3}\stackrel{\rm distr}{\rightarrow} 0$.
  Similarly, we obtain $\tilde Z_n/n^{2/3}\stackrel{\rm distr}{\rightarrow} 0$.

  By the continuous mapping theorem, and since $r>1$ we obtain 
  $$
    \sqrt{\frac{\singval_1^2(W_1)+\overline\tau_n+1
        }{\underline\tau_n+1}}
    \stackrel{\rm distr}{\rightarrow}
    \sqrt{
        \frac {1/(2r^2)+1/r+1
                }{-1/r+1}
                }.
    $$
Similarly,$$
    \frac{\sqrt{\singval_1^2(W_1)+\overline\tau_n+1
        }}{1-\singval_1(W_1)}
    \stackrel{\rm distr}{\rightarrow}
    \frac {\sqrt{1/(2r^2)+1/r+1}
                }{1-1/\sqrt{2}r}.
    $$
Simple algebra completes the proof.
  \hfill$\Box$ \end{proof}


Our simulations suggest that actually  
$\overline{\tau}_n / \singval_1(W_1)$ converges in distribution to $\sqrt{2}$ as $n\to\infty$, implying that we should see 
$\overline{\tau}_n \simeq \sqrt{2} \singval_1(W_1)$
for most matrices in real world applications.
            

\if 0
OLD
{\bf Remarks: Convergence of $Y_n$ and $\singval_1(W_1)$}
\begin{itemize}
    \item 
For $Y_n/n^{2/3}$ to converge in distribution to $0$
it is sufficient
%that there is a $\delta>0$ and a random variable
%$\overline{Y}$ such that $P[Y_n/n^{2/3-\delta}>a]\leq P[\overline{Y}>a]$.
%For this it is sufficient
that $Y_n$ itself converges in distribution to some random variable~$Y$.

\item 
        Putting these empirical findings together, we conjecture the following:
        \begin{conjecture}
        \rolf{}  With the notations and assumptions of theorem~\ref{thm:op_norm_edge_bound}
          and Lemma~\ref{lem:Abs_Value_average_bound}
          the following are conjectured to hold
          \begin{itemize}
            \item 
            $\overline{\tau}_n / \singval_1(W_1)$ converges in distribution to $\sqrt{2}$ as $n\to\infty$.
            \item The renormalization $Y_n$ \equ{Yn_def} of the largest singular value
            $\singval_1(W_1)$ converges in distribution (cpre. Figure~\ref{fig:Yn_convergence}).
        \if 0
            \item There are non-negative random variables $C_n$
            which are bounded independently of $n$
            by a constant $c<1$, such that with high probability (in fact as close to $1$
            as desired by increasing $c$)
            \begin{eqnarray*}
                \singval_1^2(1)
                &=&
                \|W_1+{\rm Id}\|_{\rm Op}^2
                \\
                &=&
                (1-C_n)
                \left(
                    \frac 1 {2r^2}\cdot(1+Y_n/(\sqrt{8}n^{2/3}))^2
                    +
                    \frac 1 r \cdot(1+Z_n/(\sqrt{8}n^{2/3}))
                    +1
                \right)
                \end{eqnarray*}
        \fi
          \end{itemize}
        \end{conjecture}
\fi





\if 0

    In concrete terms, the $99$-percentiles of $Z_n$
    (see \equ{TAU_edge_bound_sharper})
    as measured in our simulation are below $2.70$ (normal entries) and  below $2.45$ (uniform entries)
    for all $n$ simulated, the $99.9$-percentiles below $4.5$ (normal) and $4.1$ (uniform).
    This allows to draw conclusion on  the difference $\overline{t_n}-\Std \sqrt{8n}$.

    For the relative error, we point out that
    $\overline{t_n}\leq 2\Std \sqrt{8n}$ for each and every realization of the
    500'000 simulated matrices of Figure~\ref{fig:tracy-widom}.
    More generally, note that
    \begin{equation}\label{EQU:tau_rel_error}
        P[\overline{t_n} \leq r \Std\sqrt{8n}]
        =
        P[Z_n\leq (r-1)\sqrt{8} n^{2/3}]
    \end{equation}
    As mentioned we estimated these probabilities for $r=2$ to be $1.0000$ for $n=5, 10, 25, 50, 100$.
    For $r=5/4$ we estimated them for the same $n$ to be
    $0.9867, 0.9968, 0.9999, 1.0000, 1.0000$ (normal entries) and
    $0.9963, 0.9993, 1.0000, 1.0000, 1.0000 $ (uniform entries)
    up to small fluctuations depending on the realisations.

\end{itemize}

\fi



We turn now to the condition number of the relevant matrix $(D_1W_1+{\rm Id})D$
for a ResNet with ReLU activations
which are represented by
$D_1\in\mathcal{D}(\tilde m,n,0)$
and
$D\in\mathcal{D}(m,n,0)$.
We address the case of a single  residual layer
following the trained layer (cpre.~\equ{training_one_layer} with $p=1$).

To this end, we let
  \begin{equation}\label{EQU:def_nu}
    \nu
%    =
%    \frac k n
    =
    m+\tilde m-\frac{m\cdot\tilde m}n
  \end{equation}
  which can be considered as a measure of
  the extent to which these two
  non-linearities affect the output in combination.

\begin{thm}[High Probability Bound, ReLU]
  \label{thm:ReLU_average_bound}
~\\
  Let
  $D_1\in\mathcal{D}(\tilde m,n,0)$
  and
      $D\in\mathcal{D}(m,n,0)$
  with %$0\leq m,\tilde m  \leq n-1$ and
  $1 \leq m + \tilde m $.
    Then, $1\leq \nu \leq n$.
\\
%  As mentioned, $D_1$ and $D$
%  may be interpreted as local non-linearities of the type ReLU.
  %
    Choose $\theta$ such that $4<\theta\leq 2 \sqrt n$,
     let ${\rr}>1$,
     and let $r>({\rr}+{\rr}\nu+\theta)$.
\if 0
    {\tiny
    and $\tilde\Std_n$ such that
      \begin{equation}\label{EQU:Sigma_n_ReLU}
        \tilde\Std_n
        <
        \frac{1}{({\rr}+{\rr}\nu+\theta) \sqrt{8n}}
        .
      \end{equation}
      let $K_n$ be as in Theorem~\ref{thm:op_norm_edge_bound} 
      but with Gaussian entries $X_{ij}$,
      and let $W_1=\tilde\Std_nK_n$.
      }
\fi
\\
Let $\Std_n$ and $W_1$ be as in 
  Lemma~\ref{lem:Abs_Value_average_bound}
  but with Gaussian entries for $W_1$.
%denote the smallest eigenvalue of $W_1^T+W_1$
  
  Then,
  with probability
  of at least
  $1-2\exp(-\theta^2/2)
  - P[E_{\underline{\tau}_n(\rr)}]
  - P[E_{\rm \singval_n(W_1)}]
  $ 
%\rolf{replace with the s+(W1) version}  
we have
  \begin{equation}
  \label{EQU:conditioning_ReLU_average_bound}
    \CondNb((D_1W_1+{\rm Id})D))
    \leq
        2\frac{
            1+\singval_1(W_1)
            }{
            \left(
%            {1-\Std_n\sqrt{8n}({\rr}+{\rr}\nu+\theta)}
            {1-({\rr}+{\rr}\nu+\theta)/r}
            \right)
            }
    .
  \end{equation}
\end{thm}

We recall that according to our simulations
$
  P[E_{\rm \singval_n(W_1)}]
$
as well as 
$
    P[E_{\underline{\tau}_n(\rr)}]
    =
    P[Z_n > ({\rr}-1)\sqrt{8} n^{2/3}]
$
are negligible for ${\rr}\geq 2$.


%Several remarks are in order.
\if 0
    When choosing $s=1$, we may safely say:
    assuming $\Std\sqrt{8n}(2+2\nu+\theta)<1$ and $n\geq5$
    we have
    with probability of at least $1-2\exp(-2n)$
    that
      \begin{equation}
      \label{EQU:conditioning_ReLU_average_bound_simple}
        \CondNb((D_1W_1+{\rm Id})D))
        \leq
            2\frac{
                1+\singval_1(W_1)
                    }{
                \left(
                {1-\Std\sqrt{8n}(2+2\nu+\theta)}
                \right)}
        .
      \end{equation}
\fi


We mention further that the restriction $4\leq \theta\leq 2 \sqrt n$
is solely for simplicity of the representation
and can be dropped at the cost of more complicated formulas (see proof).
In the given form, useful bounds on the probability are obtained
even with modest $n$ as low as $n=7$.

Also, the condition number $\CondNb$ can actually be forced arbitrarily close to $1$
by choosing $\Std_n$ sufficiently small, as becomes
apparent from (\ref{EQU:stronger_bound_Gauss}) in the proof.





\begin{proof}
Let ${\AnyM}=W_1+{\rm Id}$ with singular values $\singval_i$
and ${\AnyMt}=(D_1W_1+{\rm Id})D$  with singular values $\tilde\singval_i$.
Clearly, ${r}>{\rr}>1$.

We proceed in several steps

\emph{(i) Sure bound on the sum of perturbations}
We cannot apply Proposition~\ref{prop:ReLU_multiple_output}
as we did in Theorem~\ref{thm:conditioning_ReLU_hard_bound}
since we need to take into account also the effect of the
left-factor $D_1$.
Due to Corollary~\ref{cor:Frobenius_bound} we have
$$
    \sum_{i=1}^{n}
        |\singval_i - \tilde\singval_i |^2
    \leq
    \|{\AnyMt}-{\AnyM}\|^2_2
    =
    \|(D_1W_1D-W_1)+(D-{\rm Id})\|^2_2.
$$
We find $k=n(m+\tilde m)-m\tilde m$
non-zero terms in the first matrix $(D_1W_1D-W_1)$
which are of the form $W_1[ij]$.
The second matrix $(D-{\rm Id})$
is diagonal
with exactly $m$ non-zero terms in the diagonal
which are all equal to $-1$.
%
Thus, the Frobenius norm $\|{\AnyMt}-{\AnyM}\|^2_2$
%the sum of squared entries of ${\AnyMt}-{\AnyM}$
consists of exactly $k$ terms of the form $W_1[ij]^2$
which we collect into a variable denoted by $V_1$,
further several terms of the form $2W_1[ij]$ which
we collect into a variable called $V_2$
and finally $m$ terms $1$.
Note that $V_2$ consists of at most $m$
terms, depending on how many diagonal positions are non-zero
in both, $(D_1W_1D-W_1)$ and $(D-{\rm Id})$.
%
We obtain
$$
    \sum_{i=1}^{n}
        |\singval_i - \tilde\singval_i |^2
    \leq
    \|{\AnyMt}-{\AnyM}\|^2_2
    =
    V_1+V_2+m
$$

By elementary calculus we have
$n\leq k\leq n^2$.
Together with 
$m,\tilde m \leq n$ and $m+\tilde m\geq 1$
this implies $1\leq \nu\leq n$.

\emph{(ii) Concentration of the values of $V_1$, $V_2$ and $\underline{\tau}_n$.}
The variable $V_2$ is zero-mean Gaussian with a variance of
at most $4m\Std_n^2$.
To formulate where the values of $V_2$ concentrate, we will use
a parameter $\theta$.
A standard result says that
\begin{equation}\label{EQU:GaussTail}
  P[V_2>\theta \cdot 2\Std_n\sqrt{m}]
  \leq
  P[X>\theta \cdot \Std_n]
  \leq
  \exp(-\theta^2/2)
  .
\end{equation}

Since $W_1[ij]/\Std_n$ are independent standard normal variables,
the variable $Y=V_1/\Std_n^2$ follows a Chi-square distribution with
$k$ degrees of freedom.
One of the sharpest bounds known for the tail
of a Chi-squared distribution
is that of Massart and Laurent \cite[Lemma 1 p1325]{Laurent-Massart}.
A Corollary of their bound yields
$$
    P[Y\geq k + 2 \sqrt{kq} +2q]
    \leq \exp(-q).
$$
%$$
%    P[X\leq k - 2 \sqrt{kq}]
%    \leq \exp(-q)
%$$
Choosing $q=\theta^2/2$ for symmetry with $V_2$, we obtain
\begin{equation}\label{EQU:ChiTail}
  P[V_1>\Std_n^2(k+2\theta\sqrt{k/2}+ \theta^2)]
  \leq
  \exp(-\theta^2/2)
  .
\end{equation}

Finally, since $-\underline{\tau}_n$ and $\overline{\tau}_n $
are equal in distribution, we get
\begin{equation}\label{EQU:tauTail}
\mbox{\small
$
    P[-\underline{\tau}_n > {\rr} \Std_n\sqrt{8n}]
    =
    P[-\underline{\tau}_n > {\rr} /  r]
    =
    P[Z_n > ({\rr}-1)\sqrt{8} n^{2/3}]
    =
    P[E_{\underline{\tau}_n(\rr)}]
    .
$}
\end{equation}
which is negligibly small for ${\rr}\geq 2$.
%\rolf{replace with the s1(W1) version ... (74) 
%could be tons of changes}  

In summary, 
using 
(\ref{EQU:GaussTail}), (\ref{EQU:ChiTail})
and \equ{tauTail}
we find, that with probability at least 
$
1
-2\exp(-\theta^2/2)
-P[E_{\underline{\tau}_n(\rr)}]
%-P[Z_n > ({\rr}-1)\sqrt{8} n^{2/3}]
-P[E_{\rm \singval_n(W_1)}]
$
%\rolf{replace with the s+(W1) version ... (74) }  
we have  simultaneously  (\ref{EQU:increase_singval_average_bound})
as well as:
\begin{eqnarray}
    \label{EQU:concentration}
    V_2&\leq&\theta \cdot 2\Std_n\sqrt{m}
    \\
    \nonumber
    V_1&\leq&\Std_n^2(k+2\theta\sqrt{k/2}+ \theta^2)
    \\
    \nonumber
    -\underline{\tau}_n &\leq& {\rr} \Std_n\sqrt{8n}=\rr/r
\end{eqnarray}

\emph{(iii) Sure bound on individual perturbations}
As in earlier proofs, we note that the bulk
of the sum of deviations
$|\singval_i - \tilde\singval_i |^2$
stems from some $m$ singular values of ${\AnyM}$
being changed to zero by $D$,
compensating the constant term $m$
on the right.
%in the bound (\ref{EQU:bound-GaussCase}).
More precisely,
%\rolf{replace with the s+(W1) version ... (74) 
%$\singval_i^2\geq \singval_n^2\geq 1-s1(W1)$
%}  
$\singval_i^2\geq \singval_n^2\geq 1+\underline{\tau}_n$
%%$\singval_i^2\geq 1-\Std_n\sqrt{8n}$
by (\ref{EQU:increase_singval_average_bound})
while
$\tilde\singval_i=0$ for $i=n-m+1,\ldots, n$.
Thus,
$$
    \sum_{i=n-m+1}^{n}
        |\singval_i - \tilde\singval_i |^2
    \geq
    m\cdot (1+\underline{\tau}_n)
%%    m\cdot (1-\Std_n\sqrt{8n})
    ,
$$
implying for any $1\leq j \leq n-m$
\begin{eqnarray*}
    |\singval_j - \tilde\singval_j |^2
    &\leq&
    \sum_{i=1}^{n-m}
        |\singval_i - \tilde\singval_i |^2
    \leq
    V_1+V_2+m
    -
    m\cdot (1+\underline{\tau}_n)
%%    m\cdot (1-\Std_n\sqrt{8n})
    \\
    &=&
    V_1+V_2 - m\underline{\tau}_n.
%%    V_1+V_2+m\Std_n\sqrt{8n}
\end{eqnarray*}
%$$
%    \leq
%    ((m+\tilde m)n\Std_n^2 + \theta \Std_n^2\sqrt{2(m+\tilde m)n})
%    +
%    2  \theta \Std_n\sqrt{m}
%    +
%    m
%    -
%    m\cdot (1-\Std_n\sqrt{8n})
%$$



{\em (iv) Probabilistic bound on the perturbation}
Combining the three bounds \equ{concentration}
which hold simultaneously with the indicated probability 
we have
\begin{eqnarray*}
    |\singval_j - \tilde\singval_j |^2
    &\leq&
    \Std_n^2(k+2\theta\sqrt{k/2} + \theta^2)
    +
    \theta \cdot 2\Std_n\sqrt{m}
    +m{\rr}\Std_n\sqrt{8n}
    \\
    &=&
    \Std_n\sqrt{8n}
    \left[
        \Std_n\sqrt{8n}
        \frac{k+\sqrt{2k}\theta+\theta^2}{8n}
        +
        2\theta \sqrt{\frac{m}{8n}}
        +
        m {\rr}
    \right]
\end{eqnarray*}
Here, we factored $\Std_n\sqrt{8n}$
in light of Theorem~\ref{thm:op_norm_edge_bound}.


{\em (v) Simplifications for convenience}
There are many ways to simplify this bound,
just for convenience of presentation.
Here is one. Assuming that $\theta\leq 2\sqrt n$
we have $\theta\leq 2\sqrt k$ and
$$
        \frac{k+\sqrt{2k}\theta+\theta^2}{8n}
        \leq
        \frac{k+\sqrt{8}k+4k}{8n}
        \leq
        \frac{8k}{8n}
        =
        \nu
        .
$$
Using $\Std_n\sqrt{8n}\cdot \nu\leq 1$,
$m /n \leq 1$
as well as
$\nu=m+\tilde m(1-m/n)\geq m$
and
%$1/4+1/\sqrt{2}\leq 1$,
$1+\theta/\sqrt 2\leq \theta$,
we get,
\begin{eqnarray*}
    |\singval_j - \tilde\singval_j |^2
   &\leq&
    \Std_n\sqrt{8n}
    \left[
    1+\theta/\sqrt 2 + {\rr}\nu
    \right]
   \leq
    \Std_n\sqrt{8n}
    \left[
    {\rr}\nu +\theta
    \right]
   .
\end{eqnarray*}
Noting that $\sqrt a-\sqrt b=(a-b)/(\sqrt a + \sqrt b)
\geq (a-b)/(1+\sqrt b)
\geq (a-b)/2$
whenever $0<a,b<1$ and using
(\ref{EQU:increase_singval_average_bound}), $s_j\geq s_n$
and \equ{tauTail}, this implies
\begin{eqnarray}
    \nonumber
    \tilde\singval_j
    &\geq&
    \singval_j
    -
    |\singval_j - \tilde\singval_j |
    \geq
    \sqrt{1-{\rr}\Std_n\sqrt{8n}}
    -
    \sqrt{  \Std_n\sqrt{8n}({\rr}\nu+\theta)}
    \\&\geq&
%    \nonumber
    \label{EQU:stronger_bound_Gauss}
        \frac {1-\Std_n\sqrt{8n}({\rr}+{\rr}\nu+\theta)}
            {
                1
                +
                \sqrt{ \Std_n\sqrt{8n} ({\rr}\nu+\theta)}
            }
            \geq
        \frac 1 2
            \left(
            {1-\Std_n\sqrt{8n}({\rr}+{\rr}\nu+\theta)}
            \right)
    .
\end{eqnarray}
Replacing $\Std_n\sqrt{8n}$ by $1/r$
this becomes
\begin{eqnarray*}
    \tilde\singval_j
    &\geq&
\if 0
    \nonumber
    \singval_j
    -
    |\singval_j - \tilde\singval_j |
    \geq
    \sqrt{1-{\rr}/r}
    -
    \sqrt{  ({\rr}\nu+\theta)/r}
    \\&\geq&
%    \nonumber
\fi
%    \label{EQU:stronger_bound_Gauss}
        \frac {1-({\rr}+{\rr}\nu+\theta)/r}
            {
                1
                +
                \sqrt{ ({\rr}\nu+\theta)/r}
            }
            \geq
        \frac 1 2
            \left(
            {1-({\rr}+{\rr}\nu+\theta)/r}
            \right)
    .
\end{eqnarray*}


This simple form is for convenience. Tighter bounds can be chosen along the lines above.
This takes care of the denominator of $\CondNb$.
For the enumerator we estimate using well-known
rules of operator norms (or alternatively
Lemma~\ref{lem:ReLU_decrease} and \equ{max_value})
$$
    \tilde\singval_1
    \leq
    (\|D_1\|\cdot\|W_1\|+\|{\rm Id}\|)\|D\|
    \leq
    \|W_1\|+1
    =
    \singval_1(W_1)+1
    .
$$
This completes the proof.
\hfill$\Box$
\end{proof}

A similar argument can be given for Uniform random entries instead of Gaussian ones
using the Central Limit Theorem and the Berry--Esseen Theorem instead of the
tail behavior of Gaussian and Chi-Square variables.
The statements and arguments will be more involved.

Also, similarly to the hard bounds it is possible to find bounds on the condition number
for leaky-ReLU, implying again that choosing $\eta$ close to $1$ allows to bound
the condition number.

\subsection{Advantages of Residual Links}
\label{subsec:advantages}

\rolf{changed title}
{\bf Volatility of the piecewise quadratic loss-surface.}~
The preceding sections provide results on the condition number $\CondNb$ of the relevant matrix $M(1)D$ for ResNets
(cpre. Corollary~\ref{cor:standard_quadratic_form}). They establish conditions under which $\CondNb(M(1)D)$ can be bounded. To be more specific, let us provide some concrete examples.

% CONCRETE EXAMPLE
To give a few concrete examples let us consider just one 
subsequent layer after the trained one, i.e., set $p=1$ in \equ{training_multi_layer}.
Consider first a deterministic setting.
Assume that the entries of the $n \times n$ matrix of weights $W_1$ are bounded by $1/(3n)$.
Then the condition number of the relevant matrix $\CondNb(M(1)D)$ amounts to at most $2$
% (1+1/3)/(1-1/3)=4/3 / (2/3) = 2
for an activation of type ``absolute value'' according to (\ref{EQU:conditioning_hard_bound}). 
If in addition not more than $1/4$ of the outputs of the trained layer are affected by the activation,  then the condition number $\CondNb(M(1)D)$ is bounded by $8$
% (1+1/3)/(1-1/3-1/2)=4/3 / (1/6) = 8
for a ReLU activation according to (\ref{EQU:conditioning_ReLU_hard_bound_small_m}).
Under more technical assumptions, bounds on the condition number are available for activation of the type leaky-ReLU.
Further bounds are available without restrictions on the outputs but more severe restrictions on the entries.

Consider now a random weight setting and assume that the standard deviation of the entries of the matrix of weights $W_1$ are bounden in the order of $1/\sqrt n$, then the condition number $\CondNb(M(1)D)$  can be bound for the absolute value activation with known probability using (\ref{EQU:conditioning_average_bound}).
For the ReLU activation,  similar bounds are available as for the absolute value.
Again, as in the deterministic case, the restrictions on the standard deviation of the weights become more severe the more outputs are affected by the ReLU (see (\ref{EQU:conditioning_ReLU_average_bound})).

Such bounds are not available to the best of our knowledge for the relevant matrix $M(0)D$ of ConvNets.
\rolf{added one sentence:}
Rather, the relevant condition number increases with $n$
as we put forward in the proof of the next result.
%\rolf{please verify the following claim:}
Notably, the loss surface is piecewise quadratic, meaning that close to the optimal values $W$ regions with quite different activities of the nonlinearites and thus with different $D$ and $D_k$ may exist. The guarantees provided for the relevant matrix for ResNets assure that the resulting piecewise quadratic loss-surface may not change shape too drastically. No such guarantees are available for ConvNets. 

{\bf Eccentricity of the loss landscape.}~
Intuition says that the loss landscape for ResNets should be less eccentric than that for ConvNets. We provide a theoretical result as well as numerical simulations to support this point of view.

\begin{lem}
  \label{lem:Adding_Id_improves_CondNb}
  Let $W_1$ be as in Lemma~\ref{lem:Abs_Value_average_bound}
  and let $D_1\in\mathcal{D}(m,n,-1)$ for some $m$.
  Let $M_o=D_1W_1$.
Then, asymptotically as $n\to\infty$:
\begin{equation}
\label{EQU:Adding_Id_improves_CondNb}
    P[
\CondNb(M_o)
\geq    
(1+\singval_1(M_o))/(1-\singval_1(M_o)) 
>0
    ]
    \to 1
\end{equation}
\end{lem}

Recalling that non-linearites of the type ``absolute value'' do not change singular values:

\begin{thm}[Residual link improves condition number]
  \label{thm:Adding_Id_improves_CondNb}
  Let $W_1$ be as in Lemma~\ref{lem:Abs_Value_average_bound}
  and let $D,D_1\in\mathcal{D}(m,n,-1)$ 
  for some $m$.
Consider a realization of $W_1$ such  that \equ{Adding_Id_improves_CondNb} holds.
Then,  adding a residual link improves the condition number of the matrix relevant for training:
\begin{equation}
\label{EQU:Res_beats_Conv_AbsValue}    
    \CondNb(D_1W_1D)\geq    
    \CondNb((D_1W_1+{\rm Id})D)
.
\end{equation}
\end{thm}
By Lemma~\ref{lem:Adding_Id_improves_CondNb}, the condition on $W_1$ is satisfied with probability asymptotically equal to $1$.

\begin{proof}
To establish  Lemma~\ref{lem:Adding_Id_improves_CondNb}
it suffices to observe that 
$\singval_1(M_o)$ converges almost surely to $1/(\sqrt{2}r<1$, as well as
\equ{conditioning_average_bound_AbsValue_via_s1}
and that $\CondNb=\CondNb(D_1W_1)$ is asymptotically of the order
$n$.

To give a rigorous argument 
note that $D_1W_1$ is a Gaussian random matrix just like 
$W_1$ itself, since $D_1$ only changes some of the signs of $W_1$ entries. Write $\CondNb=\CondNb(D_1W_1)$ for short.

Applying  a result due to Edelman \cite[Thm. 6.1]{Edelman} to the matrix $D_1W_1$ (multiplying a matrix by a constant does not change its condition number) we find that
$\CondNb/n$ converges in distribution to a random variable $K$ with density (for $x>0$)
$$
    f_K(x)
    =
    \frac{2x+4}{x^3}\exp(-2/x-2/x^2
$$
Note that $f_K$ is $\mathcal{C}^{1}(\reals^+)$ and $f_K(x)\to 0$ as $x\to0$. It follows that $P[K<\eps]\to 0$
as $\eps\to 0$.
We conclude that
$$
    P[\CondNb<n\eps]
    =
    P[\CondNb/n<\eps]
    \to
    P[K<\eps]
$$
as $n\to\infty.$


Now let $\delta>0$ be arbitrary. Choose $\eps>0$ small enough such that 
$    P[K<\eps]<\delta/2
$ and choose $n$ large enough such that 
$P[\CondNb<n\eps]<\delta$. Increase $n$ if necessary and choose $r'<r$ close enough to $1$ such that 
$n\eps=(1+1/r')/(1-1/r')$.


Since $D_1W_1$ has the same properties as $W_1$, it follows that
$\singval_1(M_o)$
is equal in distribution to 
$\singval_1(W_1)$ from  \equ{renorm_s1(W1)}.
Then, since $Y_n$ converges in distribution 
\begin{eqnarray*}
    P[\singval_1(M_o)>1/r']
    &=&
    P[\singval_1(M_o)^2>(1/r')^2]
    \leq
    P[1+Y_n\frac{1}{\sqrt{2}\cdot n^{2/3}}>2(r/r')^2]
    \\
    &=&
    P[Y_n>(2(r/r')^2-1){\sqrt{2}\cdot n^{2/3}}]
    \to 0
\end{eqnarray*}
as $n\to\infty$.
Note: if $\singval_1(M_o)\leq 1/r' $ 
then 
$ (1+\singval_1(M_o))/(1-\singval_1(M_o)) 
\leq (1+1/r')/(1-1/r')$. 
As we just showed  the probability of this happening tends to $1$ as $n\to\infty$.

    
Similarly as in other proofs we note that
$
P[\CondNb<n\eps
\mbox{ or } 
(1+\singval_1(M_o))/(1-\singval_1(M_o)) 
 >(1+1/r')/(1-1/r')
]
$
is at most equal to the sum of both probabilities, and thus at most $2\delta$ as $n\to\infty$. 
We conclude that 
$$
P[\CondNb\geq n\eps
\mbox{ and } 
(1+\singval_1(M_o))/(1-\singval_1(M_o)) < n\eps]
$$
is asymptotically at least $1-2\delta$. 
With $\delta>0$ arbitrary, this establishes Lemma~\ref{lem:Adding_Id_improves_CondNb}.

The theorem follows now from \equ{conditioning_average_bound_AbsValue_via_s1}.
\hfill$\Box$
\end{proof}

\if 0
With reference to the proof above we mention that
$P[K> 0.5]
\geq 0.9985
$
and thus 
$P[\CondNb>(\overline\tau+1)/(\underline\tau+1) ]
\geq 0.998
$
for $n$ sufficiently large.)

\rolf{this does not really say anything.}
\fi



We perform the following experiments. We build a network with the following layers: dense $\to$LeakyReLU$\to$dense$\to$LeakyReLU$\to$residual$(\rho)\to$dense. 
We recall that $dense$ performs the affine transformation of its input as in $Wx+b$, LeakyReLU performs the usual $\max(x,\eta x)$ coordinate-wise using $\eta=0.01$ (usual value), and lastly, residual$(\rho)$ performs the same operation that dense$\to$LeakyReLU and then adds the input of the layer's output.


So the $\rho$ parameter affects the residual connection of the residual layer that is before the last linear layer. Given that model, we study the loss landscape of the second layer $W$ matrix i.e. the one right before the controllable residual layer. The task at hand is a $6$-dimensional regression task. The input data is also $6$-dimensional, as well as all the hidden layers width. We visualize the singular values of the Hessian matrix of the loss landscape as $\rho$ evolves in Fig.~\ref{fig:evolution}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure_1.png}
    \begin{minipage}{0.24\linewidth}
    \centering
    $\rho$
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
    \centering
    $\rho$
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
    \centering
    $\rho$
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
    \centering
    $k$
    \end{minipage}
    \caption{Properties of the Hessian matrix
    $Q$ (see lemma~\ref{lem:standard_quadratic_form}
    and \equ{flattened_M})
    \richb{please point to an equation where this matrix appears explicitly}
    \rolf{added refs}
    of the loss as the coefficient $\rho$ is increased in a DN where the penultimate layer is the controlled residual layer, and the Hessian is taken w.r.t. to its directly preceding layer slope matrix $W$. For the left three figures multiple runs are computed with different initializations, each value is reported, on the right, the average and standard deviation over those runs are reported. We observe that (i) as the residual link is made active as the quadratic form of the loss landscape sees wider and less eccentric loss surface i.e., a more friendly geometry for gradient-based optimization.
    \richb{edit caption}
    \rolf{there is no (ii)}
    }
    \label{fig:evolution}
\end{figure}

%https://math.mit.edu/~edelman/publications/eigenvalues_and_condition.pdf



==> content/backups/introduction.tex <==
\section{Introduction}
\label{sec:intro}

% DEEP LEARNING
Deep learning has significantly advanced our ability to address a wide range of difficult inference and approximation problems. 
Today's machine learning landscape is dominated by deep (neural) networks (DNs) \cite{lecun2015deep}, which are compositions of a large number of simple parameterized linear and nonlinear operators, known as layers. 
An all-too-familiar story of late is that of plugging a DN into an application as a black box, learning its parameter values using gradient descent optimization with copious training data, and then significantly improving performance over classical task-specific approaches.

% LOTS OF MODELS, WHAT MAKES THEM DIFFERENT?
Over the past decade, a menagerie of DN architectures has emerged, including Convolutional Neural Networks (ConvNets) that feature affine convolution operations \cite{lecun1995convolutional}, Residual Networks (ResNets) that extend ConvNets with skip connections that jump over some layers \cite{he2016deep}, Dense Networks (DenseNets) with several parallel skip connections \cite{huang2017densely}, and beyond.
A natural question for the practitioners is: Which architecture should be preferred for a given task?
Approximation capability does not offer a point of differentiation, because, as their size (number of parameters) grows, these and most other DN models attain universal approximation capability \cite{daubechies2021neural}. 


% DIFFERENCE IS IN LEARNING
DN practitioners know that ResNets and DenseNets are much preferred over ConvNets, because empirically their gradient descent learning converges faster and more stably to a better solution.
In other words, it is not {\em what} a DN can approximate that matters, but rather {\em how it learns} to approximate. 
Empirical studies \cite{li2018visualizing} have indicated that this is because the so-called {\em loss landscape} of the objective function navigated by gradient descent as it optimizes the DN parameters is much smoother for ResNets and DenseNets as compared to ConvNets (see Figure~\ref{fig:loss_surface}).
However, to date there has been no analytical work in the direction.
%of analytically characterizing the properties of the loss landscape.


% THE CRUX 
In this paper, we provide the first analytical characterization of the local properties of the DN loss landscape that enables us to quantitatively compare different DN architectures.
The key is that, since the layers of all modern DNs (ConvNets, ResNets, and DenseNets included) are continuous piecewise-affine (CPA) spline mappings \cite{reportRB,balestriero2018spline}, {\em the loss landscape is a continuous piecewise function of the DN parameters}.
In particular, for regression problems where the DN approximates a function by minimizing the $\ell_2$-norm squared error, we show that the loss landscape is a continuous piecewise quadratic function of the DN parameters.
\richb{my attempt to be more precise per Section 6.3}
The local eccentricity of this landscape and width of each local minimum basin is governed by the {\em singular values} of a matrix that is a function of not only the DN parameters but also the DN architecture.
%\rolf{we should be more precise. It is not the smoothness but some sort of volatility when changing from region to region (and thus changing from matrix to matrix! not just one matrix), as well as the width (yes, numerically we see that) as well as condition number (close or far from spherical). }
%\rolf{HOW TO FIX THIS: use verbage from new section 6.3}
This enables us to quantitatively compare different DN architectures in terms of their singular values.
%Our analysis technique for the singular values of these kinds of matrices is new, and so we dedicate most of the paper to the development, which is potentially of independent interest.

% DIG DEEPER
Let us introduce some notation to elaborate on the above program.
We study state-of-the-art DNs whose layers $f_k$ comprise a continuous piecewise-linear activation function $\phi$ that is applied element-wise to the output of an affine transformation.
We focus on the ubiquitous class of activations $\phi(t) = \max(\eta t,t)$, which yields the so-called rectified linear unit (ReLU) for $\eta=0$, leaky-ReLU for small $\eta\geq 0$, and absolute value for $\eta=-1$ \cite{goodfellow2016deep}.
In an abuse of notation that is standard in the machine learning community, $\phi$ can also operate on vector inputs by applying the above activation function to each coordinate of the vector input separately.
%
Focusing for this introduction on ConvNets and ResNets (we deal with DenseNets in Section \ref{sec:DeepLearning}), denote the input to layer $k$ by $z_k$ and the output by $z_{k+1}$.
Then we can write 
\begin{equation}
	z_{k+1} = f_k(z_k) := \phi(W_k z_k+b_k) + \PertVar z_k,
		\label{eq:layer}
\end{equation}
where $W_k$ is called the weight matrix and $b_k$ is a vector of offsets.
Typically $W_k$ is a circulent convolution matrix.
The choice $\PertVar=0$ corresponds to a ConvNet, while $\PertVar=1$ corresponds to a ResNet.


\begin{figure}[t!]
    \centering
\begin{minipage}{1\linewidth}
\centering
\begin{minipage}{0.45\linewidth}
\centering
ConvNet\\
\includegraphics[width=\linewidth]{figures/loca3.png}
\end{minipage}
\hfill
\begin{minipage}{0.45\linewidth}
\centering
ResNet\\[1.6cm]
\includegraphics[width=\linewidth]{figures/loca.png}
\end{minipage}
\end{minipage}
\begin{minipage}{1\linewidth}
    \caption{\small
    Optimization landscape of two deep networks (DNs) along a 2D slice of their parameter space \cite{li2018visualizing}.
    (left) Convolutional neural network (ConvNet) with no residual connections. 
    (right) Residual network (ResNet) with residual connections.    
    {\em This paper develops new matrix perturbation theory tools to understand these landscapes and in particular explain why residual connections produce smoother loss landscapes with wider basins of attraction.} 
    Used with permission. }
    \label{fig:loss_surface}
\end{minipage}
    \vspace*{-3mm}
\end{figure}

% CPA SPLINES
Previous work \cite{reportRB,balestriero2018spline} has demonstrated the operator $f_k$ is collection of continuous piecewise-affine (CPA) splines that partitions the layer's input space into polytopal regions and fits a different affine transformation on each region with the constraint that the overall mapping is continuous.
This means that locally around the input $z_k$ and the DN parameters $W_k, b_k$, (\ref{eq:layer}) can be written as 
\begin{equation}
    z_{k+1} = D_k W_k z_k+ D_k b_k + \PertVar z_k,
\label{eq:linear}
\end{equation}
where the diagonal matrix $D_k$ contains 1s at the positions where the corresponding entries of $W_k z_k+b_k$ are positive and $\eta$ where they are negative.

% LEARNING
\sloppy
In supervised learning, we are given a set of $G$ labeled training data pairs $\{x^{(\dcounter)}, y^{(\dcounter)}\}_{\dcounter=1}^G$, and we tune the DN parameters $W_k, b_k$ such that when datum $x^{(\dcounter)}$ is input to the DN, the output $\widehat{y}^{(\dcounter)}$ is close to the true label $y^{(\dcounter)}$ as measured by some {\em loss function} $L$.
For concreteness, in this paper, we will focus on the {\em regression} task, where $y^{(\dcounter)}$ is real-valued and where the loss function is the standard $\ell_2$-norm ``squared error'' distance averaged over some subset of the training data.
%$L:=\sum_{(\dcounter)} \| y^{(\dcounter)}-\widehat{y}^{(\dcounter)}| \|_2^2$.
Standard practice is to use some flavor of gradient descent to iteratively reduce $L$ by differentiating with respect to $W_k, b_k$.
In this paper we focus on {\em fully stochastic gradient descent} that involves only a single data point per gradient step, meaning that we iteratively minimize  
\begin{equation}
    L^{(\dcounter)} :=
    \left\| y^{(\dcounter)}-
    \widehat{y}^{(\dcounter)} \right\|_2^2
    \label{eq:loss}
\end{equation}
for different choices of $\dcounter$.
Let $z_k^{(\dcounter)}$ denote the input to the $k$-th layer corresponding when the DN input is $x^{(\dcounter)}$.
Using the CPA spline formulation (\ref{eq:linear}), 
it is easy to  show (see (\ref{eq:loss_squared_out}))
%in Section~\ref{sec:DeepLearning} 
that, for fixed $y^{(\dcounter)}$, 
%and $z_k^{(\dcounter)}$, 
the loss function 
$L^{(\dcounter)}$ is piecewise-quadratic in 
$W_k, b_k$.


%PIECEWISE QUADRATIC LOSS LANDSCAPE
We can characterize the local geometric properties of this piecewise-quadratic loss surface as follows.
First, without loss of generality, we simplify our notation.
For the rest of the paper, we suppress the superscript ${(\dcounter)}$ that enumerates the training data; we label the layer of interest by $k=0$ and suppress the subscript $0$ (i.e., $W_0 \rightarrow W$); and we assume that there are $p$ subsequent layers ($1,\dots,p$) between layer 0 and the output $\widehat{y}$.
Optimizing the weights $W$ of layer $f$ with training data $x$ and layer input $z$ requires the analysis of the DN output $\widehat{y}$, due to the chain rule calculation of the gradient of $L$ with respect to $W$.
(As we discuss below, there is no need to analyze the optimization of $b$.)
We write the DN output as
\if 0
\begin{equation}
    \widehat{y} = AWz+B
\end{equation}
where
\begin{equation}
    A=(D_pW_p \cdots D_1W_1+\PertVar{\rm Id})D
    \label{eq:A}
\end{equation}
\fi
\begin{equation}
    \widehat{y} = M(\PertVar)DWz+B
\end{equation}
where 
\begin{equation}
    M(\PertVar)=D_pW_p \cdots D_1W_1+\PertVar{\rm Id}
    \label{EQU:M_intro}
\end{equation}
collects the combined effect of applying $W_k$ in subsequent layers $f_k$, $k=1,\dots,p$, and $B$ collects the combined offsets.

Using this notation and fixing the $b_k$ as well as the input $z$, the piecewise-quadratic loss function $L$ can locally be written as a linear term in $W$ plus a quadratic term in $W$, which can be written as a quadratic form featuring matrix $Q$ as follows
(see Lemma~\ref{lem:standard_quadratic_form}):
\begin{equation}
%%%    z^TW^TA^TAWz.
    z^TW^TD^TM(\PertVar)^TM(\PertVar)DWz
    =
    w^TQ^TQw.
    \label{eq:quad}
\end{equation}
Here, $w$ denotes the columnized vector version of the matrix $W$.

% SHAPE OF LOCAL LOSS SURFACE
The semi-axes of the ellipsoidal level sets of the local quadratic loss are determined by the {\em singular values} of the matrix $Q$, which we can write as $s_i \cdot z[j]$ according to Corollary~\ref{cor:standard_quadratic_form}, with $\singval_i=\singval_i(MD)$ the $i$-th singular value of the linear mapping $MD$ and $z[j]$ the $j$-th entry in the vector $z$.
%
The eccentricity of the ellipsoidal level sets is governed by the {\em condition number} of $Q$, which factors as follows:
\begin{equation}
\label{EQU:data_factor:intro}
\CondNb(Q) =
    \frac{\max_i s_i}{\min_i s_i}  \, \cdot \,
    \frac{\max_j z[j]}{\min_j z[j]}
    =
    \CondNb(MD)\cdot \CondNb(\mbox{\rm diag}(z)).
\end{equation}
In this paper we focus on the effect of the DN architecture on the condition number of the matrix $MD$ representing the action of the subsequent layers, which is   
\begin{equation}
    \CondNb(MD)
    =
    \frac{\max_i s_i(MD)}{\min_i s_i(MD)}.
\end{equation}
However, the factorization in \equ{data_factor:intro} 
(see Corollary~\ref{cor:standard_quadratic_form}) provides insights into the role played by the training datum $z[j]$.
%\rolf{In my view, we ignore since the z are the same in each step of training and independently of region. They are relevant because of the ``Data factor'' (see ): if data has a large condition number, we are already in bad shape whether we use ConvNet or ResNet. So this is an insight in addition to our comparison COnv vs Res. We focus in the paper on si and ignore z, because looking at z would be an entire new paper: how can you choose data z so that you improve condition..... Still we mention the ``data factor'' since it is relevant and leave it for someone else to study, or for our future work... whowever is faster:-) }
(We note at this point that the optimization of the offset vector $b$ has no effect on the shape of the loss function.)
\richb{is it $b$ or $B$ or both?}
\rolf{small $b$ is the offset par of the trained layer... so I guess that is what you mean here. Big $B$ is the total constant of all the following layers...this is not trained. the shape does nto depend on either}

% DIFFERENCE BETWEEN CONVNET AND RESNET
For a fixed set of training data (i.e., fixed $z$), the difference between the loss landscapes of a ConvNet and a ResNet is determined soley by $\PertVar$ in \equ{M_intro}.
Therefore, we can make a fair, quantitative comparison between the loss landscapes of the ConvNet and ResNet architectures by studying how singular values evolve as we move infinitesimally from a ConvNet ($\PertVar=0$) towards a ResNet ($\PertVar>0$).

% NEW MATH
Addressing how the singular values and condition number of the linear mapping mapping $M(\PertVar)D$ (and hence the DN optimization landscape) change when passing from $\PertVar=0$ towards $\PertVar=1$ requires a nontrivial extension of {\em matrix perturbation theory}.
Our focus and main contributions in this paper lie in exploring this under-explored territory.\footnote{A closely related situation occurs in Tikhonov regularization, where Id is added to $M^TM$ in order to regularize the ill-posed problem $Mx=b$.}
Our analysis technique is new, and so we dedicate most of the paper to its development, which is potentially of independent interest.


We briefly summarize our key theoretical findings from Sections~\ref{sec:101}--\ref{sec:Identity_withDiagonal} and our penultimate result in Theorem~\ref{thm:chi_bounds} \richb{the former Lemma 6}\rolf{the former lemma 6 clarifed the data-factor ... I believe here you talk about the perturbation via rho, so it is the thm quoted above}.
We provide concrete bounds on the growth or decay of the singular values of any square matrix $M_o=M(0)$ when it is perturbed to $M(\PertVar) = M_o + \PertVar{\rm Id}$ by adding a multiple of the identity $\PertVar{\rm Id}$ for $0\leq \PertVar \leq 1$.
The bounds are in terms of the largest and smallest eigenvalues of the symmetrized matrix $M_o^T+ M_o$.
\richb{is this correct or do we need $(M(\PertVar) D)^T M(\PertVar) D$?}
\rolf{these are overtau and undertau as defined in def 15. I  corrected above}
The behavior of the largest singular value under this perturbation can be controlled quite accurately in the sense that random matrices tend to follow the upper bound we provide quite closely with high probability.
%\richb{explain what you mean by ``hard'' upper bound}
%\rolf{hard=non-probabilistic. the term ``hard'' attempts to express the fact, that this bound hold for any matrix. But it is an upper bound on the norm of the matrix. just a bound. the statement means to say the bound is ``efficient, quite tight (=good)'' in the sense that random matrices have a norm that is quite close to the bound with high probability. in other words, the probability, that the upper bound completely overestimates the norm (=poor bound) is quite small. The term ``tend'' means that this is not an exact statement, and was observed in simulations. only in simulations, I know, but with overwhelming evidence. Short: the ``hard'' upper bound can not be improved without further assumptions. it is a ``good bound''}
For all other singular values, we require that they be non-degenerate, meaning that they have multiplicity $1$
for all but finite many $\PertVar$, a property that holds for most matrices in a generic sense.
%\richb{KEY: we need to state in this paragraph the key fact that the condition number is smaller when $\PertVar=1$ than when $\PertVar=0$!}\randall{yes this is key!}
%\rolf{just so we are all clear on this point:you cannot make this statement in all generality. There are exceptional cases...see Email Nov 7: \"Conv vs Res: kappa(0)>kappa(1) ?" Short: We need to be careful what we say. I see the following: 1) or Resent we have guarantees on condNb while for ConvNet all bets are off. 2) Sims that Randall is doing now (first weekend of Nov) show that in random settings this is what we observe in sims. }


Our new perturbation results enable to make three conclusions regarding the optimization landscape of a DN.  
First, guarantees on the piecewise quadratic optimization landscape's condition number are not available for ConvNets; in particular, $\CondNb (M(0))$ can take any value, even if entries of $M(0)$ are bounded.
Second, as we move from ConvNets ($\PertVar=0$) towards Resnets ($\PertVar>0$), bounds on $\CondNb(M(\PertVar))$ become available.
Third, for the particular case of deep networks employing absolute value activation functions, we rigorously show that the condition number of $M(1)$ (ResNet) is smaller than that of $M(0)$ ConvNet with probability asymptotically equal to $1$ for matrices with a smallest singular value $\singval_n(\PertVar)$ of multiplicity $1$.


% APPLY TO DNs
In the context of DN optimization, these results demonstrate that the local loss landscape of a ResNet is better conditioned than that of a ConvNet and thus both \richb{make sure we can say this:  less locally eccentric and smoother,}
\rolf{see new section 6.3}
%and hence smoother and easier to optimize \richb{is this obvious or do we need to back this point up?}.
%Applying Theorem XXX to DNs, we see that ResNet, conditioning of $s_i$ is better than ConvNet, or at least controllable under certain assumptions on the WEIGHTS W, irrespective of the data zj. Since ConvNet and ResNet use --- of course --- the same data, things can only be better for ResNet.
particularly when the weights in $W$ are small. 
This is typically the case at the initialization of the optimization \cite{glorot2011deep} and often remains true throughout training \cite{gal2016dropout}. 
Our results provide also provide new insights into the best magnitude to randomly initialize the weights at the beginning of learning in order to reap the maximum benefit from a ResNet architecture.
%
\richb{richb will overview Empirical validation in Figure~\ref{fig:evolution}.}


This paper is organized as follows.
%
Section~\ref{sec:101} introduces our notation and provides a review of existing useful results on the perturbation of singular values. 
%
Section~\ref{sec:DeepLearning} overviews our prior work establishing that continuous piecewise-affine (CPA) DNs can be viewed as locally linear and leverages this essential property to identify the singular values relevant for understanding the shape of the quadratic loss surface used in gradient based optimization. 
Section 4 develops the perturbation results needed to capture the influence on the singular values when adding a residual link, i.e., when passing from $M_o$ to $M_o+\PertVar{\rm Id}$. 
\richb{rolf - i added in $\PertVar$ here; is that OK?}
\rolf{we look at arbitrary rho to get the penu result thm~\ref{thm:chi_bounds}. but if you say that you add a res link, you have to pose rho=1}
In particular, bounds on the condition number of $M_o+\PertVar{\rm Id}$ are provided in terms of the largest singular value of $M_o$
and the largest eigenvalue of $M_o^T+M_o$.
Section 5 combines the findings of Sections 3 and 4 
in a deterministic setting elaborating how 
bounds on the weights of a ResNets can be used to 
bound the condition number.
Section 6 is dedicated to the random setting where
the weights of the layer to be trained are initialized 
as iid random values of a given standard deviation, establishing various bounds on the condition number of the corresponding ResNet along the lines of Sections 4 and 5. 
A result of particular interest concerns the fact that, asymptotically, i.e., for very wide DNs, the condition number of a ResNet using the absolute value as the non-linearity is smaller than that of the corresponding ConvNet with probability $1$.
We conclude in Section~\ref{sec:conclusions} with a synthesis of our results and perspectives on future research directions.
All proofs are provided within the main paper.
Various empirical experiments sprinkled throughout the paper support our theoretical results.
